Adaptive Data-Resilient Multi-Modal Hierarchical Multi-Label Book Genre Identification

Identifying fine-grained book genres is essential for enhancing user experience through efficient discovery, personalized recommendations, and improved reader engagement. At the same time, it provides publishers and marketers with valuable insights into consumer preferences and emerging market trends. While traditional genre classification methods predominantly rely on textual reviews or content analysis, the integration of additional modalities, such as book covers, blurbs, and metadata, offers richer contextual cues. However, the effectiveness of such multi-modal systems is often hindered by incomplete, noisy, or missing data across modalities. To address this, we propose IMAGINE (Intelligent Multi-modal Adaptive Genre Identification NEtwork), a framework designed to leverage multi-modal data while remaining robust to missing or unreliable information. IMAGINE learns modality-specific feature representations and adaptively prioritizes the most informative sources available at inference time. It further employs a hierarchical classification strategy, grounded in a curated taxonomy of book genres, to capture inter-genre relationships and support multi-label assignments reflective of real-world literary diversity. A key strength of IMAGINE is its adaptability: it maintains high predictive performance even when one modality, such as text or image, is unavailable. We also curated a large-scale hierarchical dataset that structures book genres into multiple levels of granularity, allowing for a more comprehensive evaluation. Experimental results demonstrate that IMAGINE outperformed strong baselines in various settings, with significant gains in scenarios involving incomplete modality-specific data.

==> 2challenge.tex <==
\section{Dataset Collection \& Design}
\label{app:dataset_creation}

\noindent 
This section discusses on the collected book data, e.g., coverpage, blurb, metadata, followed by genre labeling.



\iffalse 
We first discuss data collection followed by tag creation for level-2 classification, and imbalance in the dataset.  

\subsection{Data Collection}
\noindent 
We developed a dataset from the scratch due to unavailability of pre-existing public dataset. This process involved creating a web scraping script to extract data from the Goodreads platform. Furthermore, we leveraged the Kaggle book dataset as our foundational dataset.

\subsection{Tags Creation for Level-2}
\noindent 
We found more than 1000 genres in collected data. We needed to identify the appropriate genres for this task, since there is significant overlap between various genres and categories. For instance: 
    
\begin{itemize}[---]

    \item The book \textit{The Back Room} (ISBN-13: \textit{9780872863712}) classified under \textit{Classics}, \textit{Plays}, \textit{Fiction}, \textit{School}, \textit{Drama}, \textit{Read For School}, and \textit{Literature}. Rather than assigning each genre its own category, we combined them into the broader \textit{Literature} and \textit{Teen \& Young Adult} categories.
    
    \item The book \textit{Earth Abides} (ISBN-13: \textit{9780449232521}) classified as \textit{Science Fiction}, \textit{Fiction}, \textit{Post Apocalyptic}, \textit{Apocalyptic}, \textit{Dystopia}, \textit{Classics}, and \textit{Science Fiction Fantasy}. Instead of creating separate categories for each, we opted to consolidate them under the broader \textit{Humanities}, \textit{Literature}, and \textit{Science Fiction \& Fantasy} category. 
\end{itemize}
    
\noindent 
This approach reduced the complexity of managing multiple interrelated categories by grouping them into a larger, more inclusive category.
    
\subsection{Imbalance in the Dataset}
\noindent 
We conducted a manual review of the dataset and identified a significant imbalance in it. Several Level-2 genres within both fiction and non-fiction categories had a relatively low number of entries. Although these genres did not have enough data to be eliminated, the limited data made it difficult to train models effectively. To address this challenge, we employed data augmentation techniques to synthesize additional samples, thereby enhancing the dataset's balance and ensuring better model performance.



A subset of books was independently labeled by multiple annotators. Inter-annotator agreement metrics (such as Cohen’s Kappa or simple label overlap ratios) were used to quantify labeling consistency. Cases with low agreement were reviewed and reconciled through discussion.

\fi 

==> 3proposed_feature_extraction.tex <==

\subsection{Feature Extractor} 
\label{subsubsec:feature_extraction}

\noindent 
We utilize dedicated feature extractors for each modality in multi-modal book data and discuss them below.
% To extract features from multi-modal book data, we employed the feature extractor for each modality. We now discuss the feature extractor for each modality.

% \emph{(a)  Visual Feature Extraction Module:} 
%===============================================================
\subsubsection{Visual Feature Extractor from Cover Image}
This module extracts visual feature $g_i^{\prime V}$ from a given book cover image ${\cal{I}}_i$. 
For feature extraction, we here opt for visual transformers over CNNs since they effectively capture global context by modeling relationships across all image patches simultaneously \cite{vit_survey}, making them particularly suitable for our task, which requires a holistic understanding of book covers. 
Specifically, we utilize the Swin Transformer, which provides enhanced multiscale feature representation, capturing both fine details and high-level information \cite{SwinT}, 
as discussed below. 
% Now we discuss modules of the Swin Transformer:
%The Swin-B variant is employed due to its efficiency, offering computational complexity comparable to ViT-B/16 \cite{SwinT}. 
%In the Swin Transformer, the input image is first fed into the patch embedding module to create patches followed by a linear embedding layer to get the embedded features. These embedded features are parallelly fed into several Swin Transformer blocks to get deep features of each patch. These deep features go through the patch merging module and then multiple Swin Transformer blocks many times. Here, the patch merging module combines deep features of neighbor patches. Finally, we get deep features with cross patches information.

% \emph{(i) Patch Embedding:} 
\paragraph{Patch Embedding}
Similar to ViT \cite{ViT}, Swin Transformer takes a resized book cover image  ${\cal{I}}_i \in \mathbb{R}^{w_z \times w_z \times c_p}$ and split it into non-overlapping patches ${\cal{I}}^{<p>}_i \in \mathbb{R}^{w_p \times w_p \times c_p}$ for $p = 1, 2, \ldots, n_p$.  
%A linear embedding layer is employed on patch ${\cal{I}}^{<p>}_i$ to project it to $D_s$ dimensional features.
Each patch ${\cal{I}}^{<p>}_i$ is viewed as token, and projected into $D_s$ dimensional vector $z_0$ through embedding layer by the following linear projection.
\begin{equation}
\small
    z_0 = \left[ {\cal{I}}^{class}_i~;~ {\cal{I}}^{<1>}_i\E~;~ {\cal{I}}^{<2>}_i\E~;~ \ldots~;~ {\cal{I}}^{<n_p>}_i\E \right] +\E_{pos}
\end{equation}
%
where, $\E \in \mathbb{R}^{w_p \times w_p \times c_p \times D_s}$ is the patch embedding projection,  
$\E_{pos} \in \mathbb{R}^{(n_p + 1) \times D_s}$ is the positional embedding that contains the patches' position information \cite{attention}, and  
${\cal{I}}^{class}_i = z_0^0$ is a learnable embedding \cite{ViT}. 

% \emph{(ii) Swin Transformer Block ($ST$):} 
\paragraph{Swin Transformer Block ($ST$)}
We here compute self-attention within the window region. 
Instead of standard multi-head self attention ($MSA$) \cite{ViT}, $ST$ utilizes $WMSA$ and $SWMSA$, i.e., 
regular-window and shifted window-based multi-head self attention, respectively \cite{SwinT}.   
%
It contains $(S)WMSA$, followed by 2-layer $MLP$ with GELU activation fuction \cite{Deep_learning}. Layer normalization ($LN$) is applied before each $(S)WMSA$ and $MLP$ module. After each $(S)WMSA$/ $MLP$ module residual connection is used. 
% This module also uses a shifted window partitioning approach that alternates between two partitioning configurations in successive $ST$s, allowing for cross-window connections while maintaining computational efficiency. successive Swin Transformer blocks are computed as follows:
Here, a shifted window partitioning strategy alternates between two configurations in consecutive $ST$ blocks, enabling cross-window connections while maintaining computational efficiency, as computed below:
%
\begin{equation} \scriptsize
    \begin{split}
        \hat{z}_l = WMSA \left( LN \left( z_{l-1}\right) \right) + z_{l-1}~;~ 
        z_l = MLP \left( LN \left( \hat{z}_l\right) \right) + \hat{z}_l~; \\
        \hat{z}_{l+1} = SWMSA \left( LN \left( z_{l}\right) \right) + z_{l}~;~ 
        z_{l+1} = MLP \left( LN \left( \hat{z}_{l+1}\right) \right) + \hat{z}_{l+1} 
    \end{split}
\end{equation}
%
where, $\hat{z_l}$ and $z_l$ denote the output features of the $(S)WMSA$ module and the $MLP$ module for $l^{\text{th}}$ block, respectively.


\paragraph{Patch Merging}
As the network deepens, the patch merging layers reduce the number of patch tokens, forming a hierarchical representation. Each patch token, represented as a $D_s$-dimensional vector, is combined with features from its neighboring $2 \times 2$ patches and processed through a linear layer with $2D_s$ neurons.
% As the network gets deeper, the patch merging layers reduce the number of patch tokens to produce a hierarchical representation. Let each patch token be $D_s$ dimensional vector then the patch merging layer concatenates the features of $ 2 \times 2$ neighboring patches and employed a linear layer of $2D_s$ neurons.

% Here, the Swin-B variant is employed due to its efficiency, offering computational complexity comparable to ViT-B/16 \cite{SwinT}. 
% It utilizes patch embedding, followed by $2 \times ST$ blocks with 4 head, patch merging, $2 \times ST$ blocks with 8 head, patch merging, $18 \times ST$ blocks with 16 head, patch merging, and $2 \times ST$ block with 32 head to get $8D_s$-dimensional feature vector $g^V_i$. This $g_i^{V}$ is now fed to four different feed-forward neural networks (FNNs), each of which contain a learnable layer with $D$ neurons $ g_{ij}^{\prime V} = FNN_j^V (g_i^V); \text{~for~} j=1,2,\ldots, 4  $.
% The $D$ sized feature vector $g_{ij}^{\prime V}$'s are used in subsequent stages. Empirically, we set $w_z = 224$, $c_p = 3$, $w_p = 4$, $D_s = 128$ and window size = $ 7 \times 7$ for all $ST$ block as same \cite{SwinT}.

The Swin-B variant is employed here due to its efficiency, offering computational complexity comparable to ViT-B/16 \cite{SwinT}. 
It consists of patch embedding, followed by $2 \times ST$ blocks with 4 heads, patch merging, $2 \times ST$ blocks with 8 heads, another patch merging, $18 \times ST$ blocks with 16 heads, further patch merging, and finally, $2 \times ST$ blocks with 32 heads, producing 
% an $8D_s$-dimensional feature vector $g^V_i$. 
a feature vector $g^V_i \in \mathbb{R}^{8D_s}$. 
This feature vector, $g_i^{V}$, is then passed through $4$ separate $FNN$s, each containing a learnable layer with $D$ neurons, represented as $g_{ij}^{\prime V} = FNN_j^V (g_i^V)$; for $j=1,2,\ldots, 4$. 
The resulting 
% $D$-dimensional feature vectors $g_{ij}^{\prime V}$ 
feature vectors $g_{ij}^{\prime V} \in \mathbb{R}^D$ 
are utilized in subsequent processing stages. 
%
Empirically, we set $w_z = 224$, $c_p = 3$, $w_p = 4$, $D_s = 128$, and the window size to $ 7 \times 7$ for all $ST$s \cite{SwinT}.



% \emph{(b) Blurb Text Feature Extraction Module:} 
%===============================================================
\subsubsection{Textual Feature Extractor from Blurb}
We extract textual features $g_i^{\prime T}$ from the book blurb ${\cal{T}}_i$. Nowadays, pre-trained transformers are widely used to obtain textual features as they effectively capture rich semantic representations. While language models typically predict the next word based on preceding words, BERT employs masked token prediction \cite{BERT}, and XLNet enhances bidirectional context modeling by maximizing the expected likelihood across all possible factorization order permutations, leading to a more comprehensive text understanding \cite{XLNet}. In XLNet, the permutation language modeling objective is formulated as:
%
$    \max_{\theta}~ \mathbb{E}_{z\sim {\cal{Z}}_T} \left[ \sum^{T}_{j=1} \log p_\theta \left( {\cal{T}}^{z_j} | 
 {\cal{T}}^{z_{<j}}\right)\right] $; 
%
where, $\theta$ indicates the model parameters, ${\cal{Z}}_T$ is the set of all possible permutations with length $T$, $z_j$ is the $j^{\text{th}}$ element and $z_{<j}$ denotes the previous $(j-1)$ elements in the permutation $z \in {\cal{Z}}_T$. 
% For a given blurb ${\cal{T}}_i$, we sample a factorization order $z$ at a time and decompose the likelihood $p_\theta \left( {\cal{T}}_i \right)$ according to factorization order.
For a given blurb ${\cal{T}}_i$, a factorization order $z$ is sampled at each step, and the likelihood $p_\theta \left( {\cal{T}}_i \right)$ is decomposed based on the chosen factorization order.
%
Additionally, XLNet incorporates relative positional encoding and segment recurrence mechanism from Transformer-XL to manage long-rage dependencies better \cite{XLNet,transformerXL}.

% We adopt XLNet-Base in our framework. We extracted a $D_t$ dimensional feature vector $g_i^T$ from it. This $g_i^T$ is then fed to four different FNNs, each containing a learnable layer with $D$ neurons,
% $ g_{ij}^{\prime T} = FNN_j^T (g_i^T); \text{~for~} j=1,2,\ldots, 4$. The feature vector $g_{ij}^{\prime T}$'s are engaged in a latter phase.

We adopt XLNet-Base \cite{XLNet} into our framework to extract a feature vector $g_i^T \in \mathbb{R}^{D_t}$, which  is then processed by 4 distinct $FNN$s, each equipped with a learnable layer containing $D$ neurons; 
$g_{ij}^{\prime T} = FNN_j^T (g_i^T)$; for $j = 1,2,\dots,4$. 
The resulting feature vectors, $g_{ij}^{\prime T} \in \mathbb{R}^D$, are utilized in latter stages.
We empirically set $D_t$ equals to $768$. 




% \emph{(c) Cover Text Feature Extraction Module:}  
%===============================================================
\subsubsection{Textual Feature Extractor from Cover Page}
% The cover pages of books often include various details like the authors, publisher, and title in the form of cover text. Some books also have brief descriptions on their covers. These cover text elements help categorize the book's genre. The book cover design, including the image and cover text details, play a significant role in attracting potential readers.
%
Book covers often feature text elements, such as title, sub-title, author, and publisher, which aid in genre categorization. Along with the cover image, these textual details play a crucial role in attracting potential readers.

We engage Gemini Pro Vision \cite{gemini} on book cover image ${\cal{I}}_i$ and perform optical character recognition (OCR) to extract cover texts ${\cal{C}}_i$. 
Similar to the feature extraction from blurb ${\cal{T}}_i$, we apply XLNet-Base \cite{XLNet} on ${\cal{C}}_i$ to get cover-text feature vector $g_i^C \in \mathbb{R}^{D_c}$.
Now, $g_i^C$ is passed through a $FNN$ consists of a $D$-dimensional learnable layer to generate projected feature $g_i^{\prime C} \in \mathbb{R}^D$; $g_i^{\prime C} = FNN(g_i^C)$. 
Empirically, we fix $D_c = 768$. 


% \emph{(d) Metadata Feature Extraction Module:} 
%===============================================================
\subsubsection{Feature Extractor from Metadata}
We construct a knowledge graph from metadata to extract meaningful features. By capturing relationships between entities based on metadata fields, the knowledge graph provides a structured representation of data, enhancing semantic understanding and improving feature representation.
%
% We have defined four types of entities as $E=\{A, P, L^1, L^2\}$ corresponding to metadata fields author, publisher, Level-1 genres, Level-2 genres respectively. Further, we define six relations among them as 
% $R = \{A-P, A-L^1, A-L^2, P-L^1, P-L^2, L^1-L^2 \}$. 
% To prevent data leakage, we only use ${\cal{D}}_{train}$. 
We engage $4$ entities as $E = \{A, P, L^1, L^2\}$ corresponding to metadata fields: author, publisher, Level-1 genres, and Level-2 genres, respectively. 
% We consider a set of four entities, defined as $E = \{A, P, L^1, L^2\}$, corresponding to the metadata fields: author ($A$), publisher ($P$), Level-1 genres ($L^1$), and Level-2 genres ($L^2$).
Among entities, we define six relationships as $R = \{A \text{-} P, A \text{-} L^1, A \text{-} L^2, P \text{-} L^1, P \text{-} L^2, L^1 \text{-} L^2\}$.
To avoid data leakage, these relationships are constructed solely from the training data.
%. 
% We extract each field value of metadata as an entity and assign it a corresponding unique matching id. 
% We treat each metadata field value as an entity and assign it a unique corresponding ID.
We examine each entity-pairs $(h_i,t_i)$ in the metadata, and form triplets $(h_i,t_i,r_i)$ for each observed relation $r_i$; where, $h_i$ and $t_i$ denote $i^{\text{th}}$ head and tail entities, respectively. 
% We create a set of all triplet $MT$.

% We apply TransD \cite{transD}, a translation-based model, for knowledge graph embedding due to its ability to dynamically model entities and relations, and reduce overfitting. Each entity and relation is represented with two vectors. 
We employ TransD \cite{transD}, a translation-based knowledge graph embedding model, for its ability to dynamically represent entities and relations while mitigating overfitting. Here, each entity and relation is associated with two distinct vectors.
%==========================
% The first vector captures the semantic representation of the entity or relation, while the second vector is utilized to construct dynamic mapping matrices for projection.
% For the $i^{th}$ triplet $(h_i,t_i,r_i)$, its vectors are $\mathbf{h_i}, \mathbf{h^p_i},\mathbf{t_i}, \mathbf{t^p_i}, \mathbf{r_i}, \mathbf{r^p_i}$, where $\mathbf{h^p_i},\mathbf{t^p_i}, \mathbf{r^p_i}$ are the projection vectors, $\mathbf{h_i}, \mathbf{h^p_i},\mathbf{t_i}, \mathbf{t^p_i} \in \mathbb{R}^{D_e}$ and $\mathbf{r_i}, \mathbf{r^p_i} \in \mathbb{R}^{D_r}$. 
% For each triplet, it defines two mapping matrics $\mathbf{M}_{hr}$, $\mathbf{M}_{tr} \in \mathbb{R}^{D_r \times D_e}$ to project entities from entity domain to relation domain. This can be formulated as follows:
%==============
The first vector captures the semantic representation of the entity or relation, while the second vector serves as a projection vector used to dynamically construct mapping matrices.
For the $i^{\text{th}}$ triplet $(h_i, t_i, r_i)$, the corresponding vectors are $\mathbf{h}_i, \mathbf{h}^p_i, \mathbf{t}_i, \mathbf{t}^p_i, \mathbf{r}_i, \mathbf{r}^p_i$, where 
$\mathbf{h}^p_i, \mathbf{t}^p_i, \mathbf{r}^p_i$ are the projection vectors,  
$\mathbf{h}_i, \mathbf{h}^p_i, \mathbf{t}_i, \mathbf{t}^p_i \in \mathbb{R}^{D_e}$, and $\mathbf{r}_i, \mathbf{r}^p_i \in \mathbb{R}^{D_r}$.
For each triplet, two dynamic mapping matrices $\mathbf{M}_{hr}, \mathbf{M}_{tr} \in \mathbb{R}^{D_r \times D_e}$ to project entity embeddings from the entity domain to the relation domain, are formulated as follows: 
% These matrices are constructed using the respective projection vectors of entities and the relation.
%=====================
\begin{equation}
\small
    \mathbf{M}_{hr} = \mathbf{r}^p_i\mathbf{h}^{p\top}_i + \mathds{I} ~;~
    \mathbf{M}_{tr} = \mathbf{r}^p_i\mathbf{t}^{p\top}_i + \mathds{I}
\end{equation}
%
% where, $\mathds{I}$ is an identity matrix of size $D_r \times D_e$. We initialize mapping matrices with $\mathds{I}$ and add it to corresponding $\mathbf{M}_{hr}$,  $\mathbf{M}_{tr}$. Using these mapping matrices, the projected vectors are defined as follows:
where, $\mathds{I}$ denotes the identity matrix of size $D_r \times D_e$. We initialize the mapping matrices as $\mathds{I}$ and subsequently add them to $\mathbf{M}_{hr}$ and $\mathbf{M}_{tr}$. 
% Using these mapping matrices, the projected vectors are defined as below:
% \begin{equation}
% \small
%     \mathbf{h_{\bot}} = \mathbf{M}_{hr}\mathbf{h} ~;~
%     \mathbf{t_{\bot}} = \mathbf{M}_{tr}\mathbf{t}
% \end{equation}
% the score function is defined as below:
% \begin{equation}
%     S_r\left( h,t\right) = - ||\mathbf{h_{\bot}} + r - \mathbf{t_{\bot}} ||^2_2
% \end{equation}
%
Using these mapping matrices, the score function is defined below:
\begin{equation}
    S_r\left( h,t\right) = - ||\mathbf{M}_{hr}\mathbf{h} + r - \mathbf{M}_{tr}\mathbf{t}||^2_2
\end{equation}

%===============================
% For $i^{th}$ sample ${\cal{M}}_i$, we get all author and publisher entities and obtain entities embedding of them from $\mathbf{M}_e$, $g_i^{M} = \{\mathbf{e}^{A_1}_i, \mathbf{e}^{A_2}_i, \dots, \mathbf{e}^{A_{N_{ai}}}_i, \mathbf{e}^{P_1}_i, \mathbf{e}^{P_2}_i, \dots, \mathbf{e}^{P_{N_{pi}}}_i \}$, Here $\mathbf{e}^A_i$ and $\mathbf{e}^P_i$ denote the entity embedding of authors and publishers from ${\cal{M}}_i$ respectively. $N_{ai}$ and $N_{pi}$ are the number of authors and publishers of ${\cal{M}}_i$ respectively. The final feature of knowledge graph $g_i^{\prime M} \in \mathbb{R}^{D_e}$ is defined as the sum of all the entities embedding present in $g_i^{M}$. It is worth noting that all $\mathbf{e}^A$ and $\mathbf{e}^P$ of many ${\cal{D}}_{test}$ samples do not exist in $\mathbf{M}_e$ due to it is trained through entities of ${\cal{D}}_{train}$. In this instance, $g^{\prime M}$ become 0 vector.
% \begin{equation}
%     g_i^{\prime M} = 
%     \begin{cases}
%         \sum_{\mathbf{e}^k\in {g_i^{M}}} \mathbf{e}^k ~, & ~~ {g_i^{M}} \cap \mathbf{M}_e \neq \emptyset \\
%         0 ~, & ~~ \text{otherwise}
%     \end{cases}
% \end{equation}
% We empirically set $D_r =256$ and $D_e = 512$. 
%
%===============
The TransD model effectively captures complex multi-relational data by learning entity embeddings denoted as $ \mathbf{M}_e = \{ \mathbf{e}_i \}_{i=1}^{N_e} $, where each $ \mathbf{e}_i \in \mathbb{R}^{D_e} $ represents the embedding of the $ i^{\text{th}} $ entity, and $ N_e $ is the total number of entities in the knowledge graph. 
For each sample $\mathcal{M}_i$, we extract associated author and publisher entities and retrieve their embeddings $g_i^M$ from $ \mathbf{M}_e $; 
$g_i^{M} = \left\{ \mathbf{e}_i^{A_1}, \mathbf{e}_i^{A_2}, \dots, \mathbf{e}_i^{A_{N_{ai}}}, \mathbf{e}_i^{P_1}, \mathbf{e}_i^{P_2}, \dots, \mathbf{e}_i^{P_{N_{pi}}} \right\}$, 
where $\mathbf{e}_i^{A_j}$ and $\mathbf{e}_i^{P_k}$ denote the embeddings of the $j^{\text{th}}$ author and $k^{\text{th}}$ publisher for $\mathcal{M}_i$, respectively. Here, $N_{ai}$ and $N_{pi}$ represent corresponding total count of authors and publishers associated with $\mathcal{M}_i$.

The final knowledge graph feature vector $ g_i^{\prime M} \in \mathbb{R}^{D_e} $ is computed as the sum of all entity embeddings in $ g_i^{M} $. If none of the entities in $ g_i^{M} $ are present in $ \mathbf{M}_e $ (e.g., due to being unseen during training), $ g_i^{\prime M} $ is set to the zero vector:
\begin{equation}
g_i^{\prime M} = 
\begin{cases}
\sum_{\mathbf{e}^k \in g_i^{M}} \mathbf{e}^k, & \text{if } g_i^{M} \cap \mathbf{M}_e \neq \emptyset \\
\mathbf{0}, & \text{otherwise}
\end{cases}
\end{equation}

% Empirically, we set the embedding dimensions as $ D_r = 256 $ for relations and $ D_e = 512 $ for entities.
% Empirically, we set $D_r = 256$, and $D_e = 512$.
%===============








% \emph{(i) Loss Function for knowledge graph creation:} 
% We utilize margin-based ranking loss for the translation-based knowledge graph model. We assume the training set contains $N_t$ triplets and $i^{th}$ triplet denoted as $(h_i,t_i,r_i)$. It is worth noting that the knowledge graph only encodes positive training triplet, it does not consist of negative examples. We make use of positive golden triplets set $\Delta^+$ to generate negative triplets set $\Delta^-$ as $\Delta^- = \{ (h_i,t_j,r_j) | h_i \neq h_j \} \cup \{ (h_j,t_i,r_j) | t_i \neq t_j \}$. 
% Margin-based ranking loss can be formulated as below:
% \begin{equation}
% \footnotesize
%     f_{Lm} = \sum_{(h, t, r) \in \Delta^+} \sum_{(h^-, t^-, r^-) \in \Delta^-} [\Gamma + S_r(h,t) - S_r(h^-,t^-)]_+
% \end{equation}
% where $[x]_+ \triangleq max(x,0)$ and $\Gamma$ is the margin separating positive golden triplet and negative triplet.
%============

We employ a margin-based ranking loss for training the translation-based knowledge graph model. 
% Let the training set consist of $N_t$ triplets, where the $ i^{\text{th}} $ triplet is denoted as $ (h_i, t_i, r_i) $. 
It is worth noting the knowledge graph only encodes positive triplets; negative examples are not included. 
We leverage the positive golden triplet set $\Delta^+$ to generate the negative triplet set $\Delta^-$ as follows: 
$\Delta^- = \{ (h_i, t_j, r_j) \mid h_i \neq h_j \} \cup \{ (h_j, t_i, r_j) \mid t_i \neq t_j \}$. 
% The margin-based ranking loss ($f_{Lm}$) is then formulated as below:
The margin-based ranking loss ($f_{Lm}$) is formulated as:
%
% \begin{equation}
% \footnotesize
% f_{Lm} = \sum_{(h, t, r) \in \Delta^+} \sum_{(h^-, t^-, r^-) \in \Delta^-} \left[ \Gamma + S_r(h,t) - S_r(h^-,t^-) \right]_+
% \end{equation}
%
\begin{equation}
\footnotesize
f_{Lm} = \sum_{\substack{(h, t, r) \\ \in \Delta^+}} \sum_{\substack{(h^{\text{\---}}, t^{\text{\---}}, r^{\text{\---}}) \\ \in \Delta^-}}  \max\left(\left[ \Gamma + S_r(h,t) - S_r(h^{\text{\---}},t^{\text{\---}}) \right], 0\right)
\end{equation}
%
where, $\Gamma$ is the margin used to separate positive and negative triplets. 
Empirically, we set $D_r = 256$, and $D_e = 512$.

==> OCR_stat.tex <==
% \emph{\textbf{Statistics of OCR extracted text}}
\begin{table}[h]
\centering  
\caption{Statistics analysis of cover text}
% \footnotesize
% \caption{Word-count wise distribution of OCR extracted text from book cover page} 
\label{tab1} % Move the \label{} here
\begin{adjustbox}{width=0.25\textwidth}
\begin{tabular}{c|c}
\hline
Word count range& Number of books \\
\hline 
1 \--- 10 & 8055\\
11 \--- 20 & 8989\\
21 \--- 30 & 4174\\
31 \--- 40 & 2225\\
41 \--- 50 & 815\\
51 \--- 60 & 426\\
61 \--- 70 & 159\\
71 \--- 80 & 60\\
81 \--- 90 & 39\\
91 \--- 100 & 27\\
101 \--- 200 & 108\\
201 \--- 300 & 44\\
301 \--- 400 & 16\\
401 \--- 500 & 2\\
501 \--- 600 & 72\\
601 \--- 700 & 0\\
701 \--- 800 & 1\\
801 \--- 900 & 3\\
 \hline
\end{tabular}
\end{adjustbox}
\label{OCR_stat}
\end{table}




% \begin{table}[H]
% \centering  
% \footnotesize
% \caption{\small Statistical analysis of OCR extracted text from cover page image:}

% \begin{adjustbox}{width=0.47\textwidth}

% \begin{tabular}{p{2cm}|p{2cm}|c|c|c}
% \hline
% \centering{Minimum word count in an OCR extracted text} & \centering{Maximum word count in an OCR extracted text} & \centering{Mean} & \centering{Median} & Standard deviation\\
% \hline 
% \centering{1} & \centering{862} & 21.327 & 15 & 33.390\\
% \hline
% \end{tabular}
% \end{adjustbox}
% \label{tab:prob_analysis}
% \end{table}












==> description_statistical_info.tex <==
% \begin{table}[H]
% \centering
% \caption{Statistics analysis of description text}
% % \caption{Word-count wise distribution of descriptions before and after augmentation}
% \begin{adjustbox}{width=0.45\textwidth} 
% \begin{tabular}{p{2cm}|p{3.5cm}|c|c}
% \hline
% \textbf{Word count range} & \textbf{\centering{Number of samples in that range \\(before augmentation)}} & \multicolumn{2}{c}{\textbf{\centering{Number of samples in that range(after augmentation)}}} \\ \cline{3-4}
%  & & \textbf{Before preprocessing} & \textbf{After preprocessing} \\ \hline
% 1 \--- 100 & \centering{6232} & 16767 & 19997\\ \hline
% 101 \--- 200 & \centering{3502} & 8959 & 3685\\ \hline
% 201 \--- 300 & \centering{1078} & 1567 & 266\\ \hline
% 301 \--- 400 & \centering{296} & 332 & 31\\ \hline
% 401 \--- 500 & \centering{73} & 74 & 9\\ \hline
% 501 \--- 600 & \centering{20} & 22 & 4\\ \hline
% 601 \--- 700 & \centering{8} & 8 & 2\\ \hline
% 701 \--- 800 & \centering{5} & 5 & 1\\ \hline
% 801 \--- 900 & \centering{0} & 0 & 1\\ \hline
% 901 \--- 1000 & \centering{0} & 0 & 1\\ \hline
% 1001 \--- 1100 & \centering{3} & 3 & 0\\ \hline
% 1100 \--- 1200 & \centering{1} & 1 & 0\\ \hline
% 1201 \--- 1300 & \centering{0} & 0 & 0\\ \hline 
% 1301 \--- 1400 & \centering{1} & 1 & 0\\ \hline
% 1401 \--- 1500 & \centering{0} & 0 & 0\\ \hline
% 1501 \--- 1600 & \centering{1} & 1 & 0\\ \hline
% \end{tabular}
% \end{adjustbox}
% \label{Word-count wise distribution of descriptions}
% \end{table}





% \begin{table}[H]
% \centering  
% \footnotesize
% \caption{Word-count wise distribution of descriptions before augmentation} 
% \label{tab1} % Move the \label{} here
% \begin{adjustbox}{width=0.47\textwidth}
% \begin{tabular}{c|p{3cm}}
% \hline
% Word-count range in description & Number of books containing that many words in their description\\
% \hline 
% 1 \--- 100 & 6232\\
% 101 \--- 200 & 3502\\
% 201 \--- 300 & 1078\\
% 301 \--- 400 & 296\\
% 401 \--- 500 & 73\\
% 501 \--- 600 & 20\\
% 601 \--- 700 & 8\\
% 701 \--- 800 & 5\\
% 801 \--- 900 & 0\\
% 901 \--- 1000 & 0\\
% 1001 \--- 1100 & 3\\
% 1100 \--- 1200 & 1\\
% 1201 \--- 1300 & 0\\
% 1301 \--- 1400 & 1\\
% 1401 \--- 1500 & 0\\
% 1501 \--- 1600 & 1\\
%  \hline
% \end{tabular}
% \end{adjustbox}
% \label{before_augmentation}
% \end{table}





% \begin{table}[H]
% \centering  
% \footnotesize
% \caption{Word-count wise distribution of descriptions after augmentation (Before preprocessing)} 
% \label{tab1} % Move the \label{} here
% \begin{adjustbox}{width=0.47\textwidth}
% \begin{tabular}{c|p{3cm}}
% \hline
% Word-count range in description & Number of books containing that many words in their description\\
% \hline 
% 1 \--- 100 & 16767\\
% 101 \--- 200 & 8959\\
% 201 \--- 300 & 1567\\
% 301 \--- 400 & 332\\
% 401 \--- 500 & 74\\
% 501 \--- 600 & 22\\
% 601 \--- 700 & 8\\
% 701 \--- 800 & 5\\
% 801 \--- 900 & 0\\
% 901 \--- 1000 & 0\\
% 1001 \--- 1100 & 3\\
% 1100 \--- 1200 & 1\\
% 1201 \--- 1300 & 0\\
% 1301 \--- 1400 & 1\\
% 1401 \--- 1500 & 0\\
% 1501 \--- 1600 & 1\\
%  \hline
% \end{tabular}
% \end{adjustbox}
% \label{after_aug_without_preprocessing}
% \end{table}






% \begin{table}[H]
% \centering  
% \footnotesize
% \caption{Word-count wise distribution of descriptions after augmentation (After preprocessing)} 
% \label{tab1} % Move the \label{} here
% \begin{adjustbox}{width=0.47\textwidth}
% \begin{tabular}{c|p{3cm}}
% \hline
% Word-count range in description & Number of books containing that many words in their description\\
% \hline 
% 1 \--- 100 & 19997\\
% 101 \--- 200 & 3685\\
% 201 \--- 300 & 266\\
% 301 \--- 400 & 31\\
% 401 \--- 500 & 9\\
% 501 \--- 600 & 4\\
% 601 \--- 700 & 2\\
% 701 \--- 800 & 1\\
% 801 \--- 900 & 1\\
% 901 \--- 1000 & 1\\

%  \hline
% \end{tabular}
% \end{adjustbox}
% \label{after_aug_with_preprocessing}
% \end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Version -2
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[H]
\centering
\caption{Statistics analysis of description text}
% \caption{Word-count wise distribution of descriptions before and after augmentation}
\begin{adjustbox}{width=0.45\textwidth} 
\begin{tabular}{c|c|c}
\hline
Word count & Number of samples   & Number of samples \\ 
range & (before augmentation) & (after augmentation) \\
\hline
1 \--- 100 & 6232 & 16767 \\ \hline
101 \--- 200 & 3502 & 8959 \\ \hline
201 \--- 300 & 1078 & 1567 \\ \hline
301 \--- 400 & 296 & 332 \\ \hline
401 \--- 500 & 73 & 74 \\ \hline
501 \--- 600 & 20 & 22\\ \hline
601 \--- 700 & 8 & 8 \\ \hline
701 \--- 800 & 5 & 5 \\ \hline
801 \--- 900 & 0 & 0 \\ \hline
901 \--- 1000 & 0 & 0 \\ \hline
1001 \--- 1100 & 3 & 3 \\ \hline
1100 \--- 1200 & 1 & 1 \\ \hline
1201 \--- 1300 & 0 & 0 \\ \hline 
1301 \--- 1400 & 1 & 1 \\ \hline
1401 \--- 1500 & 0 & 0 \\ \hline
1501 \--- 1600 & 1 & 1 \\ \hline
\end{tabular}
\end{adjustbox}
\label{tab:stat_description}
\end{table}






==> hierarchical_genre_analysis.tex <==

    
% \begin{table}[H] 
% \centering  
% %\footnotesize
% \normalsize
% \caption{Hierarchical genre-wise count of the dataset} \label{tab1} % Move the \label{} here
% \begin{adjustbox}{width=0.49\textwidth}
% \begin{tabular}{c |l |c |c |c |c}
% \hline
% {Class Id} & {Genre label} & {Fiction} & Fiction & NonFiction & Nonfiction\\

% & & (Before augmentation) & (After augmentation) & (Before augmentation) & (After augmentation)\\
% \hline 
% 1 & {Animals \& Wildlife \& Pets} & 590 & 1260 & 235 & 924\\
% 2 & \centering{Arts \& Photography} & 1188 & 2566 & 606 & 1782\\
% 3 & \centering{Business \& Money} & 42 & 624 & 256 & 760\\
% 4 & \centering{Childrens Book} & 1714 & 3281 & 298 & 1080\\
% 5 & \centering{Comics \& Graphic} & 364 & 791 & 96 & 1002\\
% 6 & \centering{Computers \& Technology} & 27 & 596 & 92 & 595\\
% 7 & \centering{Cookbooks \& Food \& Wine} & 72 & 808 & 223 & 608\\
% 8 & \centering{Crafts \& Hobbies \& Home} & 40 & 520 & 61 & 541\\
% 9 & \centering{Environment \& Plant} & 92 & 905 & 337 & 1028\\
% \multirow{2}{*}{10} & \centering{Family \& Parenting} & \multirow{2}{*}{208} & \multirow{2}{*}{800} & \multirow{2}{*}{257} & \multirow{2}{*}{1089}\\
% &  \& Relationships & & & &\\
% 11 & \centering{Fashion \& Lifestyle} & 732 & 1426 & 204 & 1100\\
% 12 & \centering{Health \& Fitness \& Dieting} & 32 & 710 & 320 & 1171\\
% 13 & \centering{History} & 1677 & 3123 & 1619 & 4095\\
% 14 & \centering{Humanities} & 537 & 1481 & 1555 & 4223\\
% 15 & \centering{Humor \& Entertainment} & 972 & 2009 & 376 & 1360\\
% 16 & \centering{Literature} & 2615 & 6088 & 670 & 1786\\
% \multirow{2}{*}{17} & \centering{Mystery \& Thriller} & \multirow{2}{*}{2043} & \multirow{2}{*}{4289} & \multirow{2}{*}{404} & \multirow{2}{*}{920}\\
% & \& Suspense \& Horror & & & &\\
% 18 & \centering{Medical} & 70 & 950 & 165 & 1080\\
% 19 & \centering{Meta Text} & 35 & 774 & 88 & 954\\
% \multirow{2}{*}{20} & \centering{Mythology \& Religion} & \multirow{2}{*}{890} & \multirow{2}{*}{1909} & \multirow{2}{*}{748} & \multirow{2}{*}{1376}\\
% &  \& Spirituality & & & &\\
% 21 & \centering{Press \& Media} & 138 & 486 & 167 & 903\\
% 22 & \centering{Reference \& Language} & 97 & 694 & 1003 & 3077\\
% 23 & \centering{Romance} & 1445 & 2275 & 80 & 1065\\
% 24 & \centering{Science \& Math} & 419 & 718 & 712 & 2221\\
% % &  \& Mathematics & & & &\\
% 25 & \centering{Self-help \& Motivation} & 72 & 993 & 630 & 1865\\
% 26 & \centering{Sports \& Outdoors} & 183 & 825 & 157 & 522\\
% 27 & \centering{Teen \& Young Adult} & 1712 & 2524 & 170 & 817\\
% 28 & \centering{Travel} & 92 & 743 & 393 & 1090\\
% 29 & \centering{Science Fiction \& Fantasy} & 2715 & 5034 & 0 & 0\\
% 30 & \centering{Biographies \& Memoir} & 0 & 0 & 1256 & 3466\\
% \hline
% \end{tabular}
% \end{adjustbox}
% \label{hierarchical_genre_analysis}
% \end{table}




% % \begin{table}[H]
% % \centering   
% % \footnotesize
% % \caption{Poster and movie counts across genre labels}\label{tab1}
% % \begin{adjustbox}
% % \begin{tabular}{c|c|c|c|c|c}
% % \hline
% % Class Id & Genre label & Poster count & Movie count & Movie count & Movie count\\
% % \hline 
% % 1 & Action &  4985 & 1426 & 11 & 12\\
% % 2 & Adventure & 3702 & 1024 & 11 & 12\\
% % 3 & Animation &  1196 & 325\\
% % 4 & Biography &  1076 & 348\\
% % 5 & Comedy & 4380 & 1517\\
% % 6 & Crime &  3052 & 1003\\
% % 7 & Drama & 6609 & 2217\\
% % 8 & Fantasy &  1379 & 423\\
% % 9 & Horror & 2646 & 860\\
% % 10 & Mystery &  2285 & 750\\
% % 11 & Romance &  2406 & 913\\
% % 12 & Sci-Fi &  1542 & 458\\
% % 13 & Thriller &  3455 & 1092\\
% % \hline
% % \end{tabular}
% % \end{adjustbox}
% % % \end{tabular}
% % \label{tab:class_no}
% % \end{table}



% % \begin{table}[]
% % \centering
% % \caption{\small Ablation Study}
% %  \begin{adjustbox}{width=0.45\textwidth} 
% % \begin{tabular}{l|c|c|c|c|c|c}
% % \hline 
% % Model & $\cal{P}$ & $\cal{R}$ & ${\cal{S}}p$ &  ${\cal{BA}}$ & ${\cal{FM}}$ & ${\cal{HL}}$ \\
% % \hline 
% % R        & 52.04 & 50.44 & 85.36   &  67.90 & 48.97 & 0.18524 \\
% % T        & 29.11 & 27.40 & 78.61   &  53.01 & 22.58 & 0.25243 \\
% % RT       & 52.54 & 55.53 & 86.67    & 71.10 & 53.57 & 0.17833 \\
% % DT       & 33.78 & 29.81 & 79.14    & 54.48 & 25.42 & 0.26509 \\
% % RDT      & 55.01 & 57.25 & 87.08    & 72.16 & 55.69 & 0.17069 \\
% % R + RDT  & 55.35 & 56.46 & 86.97    & 71.72 & 55.20 & 0.16954 \\
% % RT + RDT & 54.96 & 57.44 & 87.28    & 72.36 & 55.70 & 0.16755 \\
% % ERDT     & 55.95 & \textbf{57.88}  & 87.35    & \textbf{72.61}    & \textbf{56.40}    & 0.16546 \\
% % PrERDT   & \textbf{57.77}     & 54.65 & \textbf{88.71}           & 71.68& 55.26 & \textbf{0.16216} \\
% % \hline 
% % \end{tabular}
% % \end{adjustbox}
% % \label{tab:ablation}
% % \end{table}

==> image_area-wise_distribution.tex <==
% \emph{\textbf{Statistics of cover page images}}

\begin{table}[H]
\centering  
% \footnotesize
% \caption{ Image area-wise distribution  before and after augmentation} 
\caption{Statistics analysis of cover page images}
\begin{adjustbox}{width=0.5\textwidth}
\begin{tabular}{c|c|c}%{p{2.5cm}|p{2.5cm}|p{2.5cm}}
\hline
Image area range  & Number of samples before & Number of samples after\\
(10000 pixel$^2$) & augmentation & augmentation \\
\hline 
< 5 & 20 & 50\\
5 \--- 10 & 264 & 9847\\
10 \--- 15 & 7057 & 11124\\
15 \--- 20 & 2205 & 3906\\
20 \--- 25 & 278 & 584\\
25 \--- 30 & 125 & 269\\
30 \--- 35 & 52 & 87\\
35 \--- 40 & 41 & 63\\
> 40 & 1298 & 2091\\
 \hline
\end{tabular}
\end{adjustbox}
\label{image_distribution_before_and_after_aug}
\end{table}





% \begin{table}[H]
% \centering  
% \footnotesize
% \caption{ Image area-wise distribution after augmentation} 
% \label{tab1} % Move the \label{} here
% \begin{tabular}{l|l}
% \hline
% Image area range (10000 pixel$^2$) & Image count\\
% \hline 
% < 5 & 50\\
%  5 \--- 10 & 9847\\
%  10 \--- 15 & 11124\\
%  15 \--- 20 & 3906\\
%  20 \--- 25 & 584\\
%  25 \--- 30 & 269\\
%  30 \--- 35 & 87\\
%  35 \--- 40 & 63\\
%  > 40 & 2091\\
%  \hline
% \end{tabular}
% \label{image_distribution_after_aug}
% \end{table}








==> metadata_stat.tex <==
% \emph{\textbf{Metadata statistics}}
% \begin{table}[H]
% \centering  
% \footnotesize
% \caption{Distribution of number of books written by an author} 
% \label{tab1} % Move the \label{} here
% \begin{tabular}{p{2cm}|c}
% \hline
% \centering{Number of books published by an author} & \# author\\
% \hline 
% \centering{1 \--- 10} & 14355\\
% \centering{10 \--- 20} & 960\\
% \centering{20 \--- 30} & 386\\
% \centering{30 \--- 40} & 258\\
% \centering{40 \--- 50} & 150\\
% \centering{50 \--- 60} & 121\\
% \centering{60 \--- 70} & 78\\
% \centering{70 \--- 80} & 64\\
% \centering{80 \--- 90} & 48\\
% \centering{90 \--- 100} & 29\\
% \centering{100 \--- 200} & 96\\
% \centering{200 \--- 300} & 12\\
% \centering{300 \--- 400} & 5\\
% \centering{400 \--- 500} & 2\\
% \centering{500 \--- 600} & 2\\
% \centering{600 \--- 700} & 1\\

%  \hline
% \end{tabular}
% \label{books_per_author}
% \end{table}

% %\vspace{1cm}
% % \begin{table}[H]
% % \caption{Statistical analysis of books written by an author} 


% % \begin{adjustbox}{width=0.47\textwidth}

% % \begin{tabular}{p{2cm}|p{2cm}|c|c|c}
% % \hline
% % \centering{Minimum count} & \centering{Maximum count} & \centering{Mean} & \centering{Median} & Standard deviation\\
% % \hline 
% % \centering{1} & \centering{632} &  9.89 & 5.5 & 19.82\\
% %  \hline
% % \end{tabular}
% % \end{adjustbox}
% % \label{tab:prob_analysis}
% % \end{table}





% \begin{table}[H]
% \centering  
% \footnotesize
% \caption{Distribution of the number of books published by a publisher} 
% \label{tab1} % Move the \label{} here
% \begin{tabular}{p{2cm}|c}
% \hline
% \centering{Number of books published by a publisher} & \# publisher\\
% \hline 

% \centering{1 \--- 100} & 16170\\
% \centering{100 \--- 200} & 174\\
% \centering{200 \--- 300} & 80\\
% \centering{200 \--- 300} & 80\\
% \centering{300 \--- 400} & 39\\
% \centering{400 \--- 500} & 21\\
% \centering{500 \--- 600} & 21\\
% \centering{600 \--- 700} & 16\\
% \centering{700 \--- 800} & 12\\
% \centering{800 \--- 900} & 6\\
% \centering{900 \--- 1000} & 3\\
% \centering{1000 \--- 2000} & 22\\
% \centering{2000 \--- 3000} & 8\\
% \centering{3000 \--- 4000} & 5\\
% \centering{4000 \--- 5000} & 1\\
% \centering{5000 \--- 6000} & 0\\
% \centering{6000 \--- 7000} & 0\\
% \centering{7000 \--- 8000} & 1\\

%     \hline
% \end{tabular}
% \label{books_per_publisher}
% \end{table}


% % \begin{table}[H]
% % \caption{Statistical analysis of books published by a publisher} 


% % \begin{adjustbox}{width=0.47\textwidth}

% % \begin{tabular}{p{2cm}|p{2cm}|c|c|c}
% % \hline
% % \centering{Minimum count} & \centering{Maximum count} & \centering{Mean} & \centering{Median} & Standard deviation\\
% % \hline 
% % \centering{1} & \centering{7536} & 60.75 & 50.5 & 125.74\\
% %  \hline
% % \end{tabular}
% % \end{adjustbox}
% % \label{tab:prob_analysis}
% % \end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Version 2
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table}[H]
\centering  
% \footnotesize
\caption{Statistics analysis of metadata} 
 \begin{adjustbox}{width=0.5\textwidth}
\begin{tabular}{c|c||c|c}
\hline
Number of books  &  & Number of books & \\
published by & \# author & published by  & \# publisher \\ 
an author & & a publisher & \\
\hline
1 \--- 10 & 14355 & 1 \--- 100 & 16170\\
10 \--- 20 & 960 & 100 \--- 200 &  174 \\
20 \--- 30 & 386 & 200 \--- 300 & 80 \\
30 \--- 40 & 258 & 300 \--- 400 & 39 \\
40 \--- 50 & 150 & 400 \--- 500 & 21 \\
50 \--- 60 & 121 & 500 \--- 600 & 21 \\
60 \--- 70 & 78 & 600 \--- 700 & 16 \\
70 \--- 80 & 64 & 700 \--- 800 & 12 \\
80 \--- 90 & 48 & 800 \--- 900 & 6 \\
90 \--- 100 & 29 & 900 \--- 1000 & 3 \\
100 \--- 200 & 96 & 1000 \--- 2000 & 22 \\
200 \--- 300 & 12 & 2000 \--- 3000 & 8 \\
300 \--- 400 & 5 & 3000 \--- 4000 & 5 \\
400 \--- 500 & 2 & 4000 \--- 5000 & 1 \\
500 \--- 600 & 2 & 5000 \--- 6000 & 0 \\
600 \--- 700 & 1 & 6000 \--- 7000 & 0\\
& & 7000 \--- 8000 & 1 \\

 \hline
\end{tabular}
\end{adjustbox}
\label{books_per_author}
\end{table}




==> stat.tex <==
\begin{table}[]
 \centering
 \caption{Statistical analysis}
 \vspace{1em} % Adjust the vertical space here
 \begin{adjustbox}{width=0.49\textwidth}
 \begin{tabular}{c |c |c |c |c |c |c}
   \hline
   
   \multirow{2}{*}{Input} &  \multirow{2}{*} & \multirow{2}{*}{Minimum} & \multirow{2}{*}{Maximum} & \multirow{2}{*}{Mean} & \multirow{2}{*}{Median} & \multirow{2}{*}{Standard deviation} \\\\
   \hline
   \multirow{4}{*}{\rotatebox{0}{\textbf{Cover page images}}} & \multirow{2}{*}{Before augmentation} & \multirow{2}{*}{20460} & \multirow{2}{*}{16301712} & \multirow{2}{*}{176507.93} & \multirow{2}{*}{125000} & \multirow{2}{*}{104410.22}\\\\ \cline{2-7}
   & \multirow{2}{*}{After augmentation} & \multirow{2}{*}{20460} & \multirow{2}{*}{16301712} & \multirow{2}{*}{143180.11} & \multirow{2}{*}{125000} & \multirow{2}{*}{97393.49}\\\\ \cline{2-7}
    \hline

   \multirow{6}{*}{\rotatebox{0}{\textbf{Description}}} & \multirow{2}{*}{Before augmentation} & \multirow{2}{*}{0} & \multirow{2}{*}{1580} & \multirow{2}{*}{108.217} & \multirow{2}{*}{87} & \multirow{2}{*}{90.925}\\\\ \cline{2-7}
   & \multirow{2}{*}{After augmentation (Without preprocessing)} & \multirow{2}{*}{0} & \multirow{2}{*}{1580} & \multirow{2}{*}{97.368} & \multirow{2}{*}{85} & \multirow{2}{*}{33.023}\\\\ \cline{2-7}
   & \multirow{2}{*}{After augmentation (With preprocessing)} & \multirow{2}{*}{21} & \multirow{2}{*}{949} & \multirow{2}{*}{69.483} & \multirow{2}{*}{61} & \multirow{2}{*}{20.394}\\\\ \cline{2-7}
   \hline
   \multirow{2}{*}{\rotatebox{0}{\textbf{OCR text}}} & \multirow{2}{*}{Before and after augmentation} & \multirow{2}{*}{1} & \multirow{2}{*}{862} & \multirow{2}{*}{21.327} & \multirow{2}{*}{15} & \multirow{2}{*}{33.390}\\\\
   

   \hline

   \multirow{4}{*}{\rotatebox{0}{\textbf{Metadata}}} & \multirow{2}{*}{Books written by an author} & \multirow{2}{*}{1} & \multirow{2}{*}{632} & \multirow{2}{*}{9.89} & \multirow{2}{*}{5.5} & \multirow{2}{*}{19.82}\\\\ \cline{2-7}
   & \multirow{2}{*}{Books published by a publisher} & \multirow{2}{*}{1} & \multirow{2}{*}{7536} & \multirow{2}{*}{60.75} & \multirow{2}{*}{50.5} & \multirow{2}{*}{125.74}\\\\ \cline{2-7}
   \hline
 \end{tabular}
 \end{adjustbox}
 \end{table}





==> statistical_analysis_image.tex <==

\begin{table}[H]
\centering  
\footnotesize
\caption{\small Statistical analysis of the cover page images based on dimension:}

\begin{adjustbox}{width=0.47\textwidth}

\begin{tabular}{p{2cm}|p{2cm}|c|c|c}
\hline
\centering{Minimum dimension(10,000-pixel square)} & \centering{Maximum dimension(10,000-pixel square)} & \centering{Mean(10,000-pixel square)} & \centering{Median(10,000-pixel square)} & Standard deviation(10,000-pixel square)\\
\hline 
\centering{2.0460} & \centering{1630.1712} & 14.318011 & 12.5000 & 9.739349\\
\hline
\end{tabular}
\end{adjustbox}
\label{tab:prob_analysis}
\end{table}












==> statistical_analysis_table.tex <==
% \begin{table}[H]
% \caption{Statistical analysis of books} 


% \begin{adjustbox}{width=0.47\textwidth}

% \begin{tabular}{p{2cm}|p{2cm}|p{2cm}|c|c|c}
% \hline
% \centering{Input feature} &
% \centering{Minimum count} & \centering{Maximum count} & \centering{Mean} & \centering{Median} & Standard deviation\\
% \hline 
% \centering{Cover page images} & \centering{20460} & \centering{16301712} & \centering{143180.11} & \centering{125000} & 97393.49\\  

% %\centering{1} & \centering{7536} & 60.75 & 50.5 & 125.74\\
%  \hline
% \end{tabular}
% \end{adjustbox}
% \label{tab:prob_analysis}
% \end{table}

==> tables/OCR_challenges_table.tex <==
% \begin{figure*}[t]
% \centering
% \footnotesize
% % \makebox[\textwidth][c]{
% % \begin{adjustbox}{width=.95\linewidthwidth} 
% \begin{tabular}{c|c|c|c || c|c|c|c}
% %%%%%%%%%%%%%%%
% \hline 
% &&& &&&&  \\[\dimexpr-\normalbaselineskip+1.5pt]
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/414.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/12916.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/12937.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/81539.jpg} &
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/67010.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/64126.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/11708.jpg} &
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/spanish_book.jpeg}\\
% \textcolor{blue}{\emph{i.}} F : (16) & \textcolor{blue}{\emph{ii.}}  F : (16, 20, 29, 27) & \textcolor{blue}{\emph{iii.}}  F : (4, 27) & \textcolor{blue}{\emph{iv.}}  F : (11, 14, 16) & 
% \textcolor{blue}{\emph{v.}}  F : (13, 16, 28) & \textcolor{blue}{\emph{vi.}}  F : (2, 4, 29, 27) & \textcolor{blue}{\emph{vii.}} NF : (13, 16, 28) & \textcolor{blue}{\emph{viii.}}  F : (22, 29) \\ 
% \multicolumn{4}{c||}{less info(only book/ author name)} & \multicolumn{4}{c|}{Non-English Languages on the Cover Page}\\
% %%%%%%%%%%%%%%%

% %%%%%%%%%%%%%%%
% \hline 
% &&& &&&&  \\[\dimexpr-\normalbaselineskip+1.5pt]
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/67009.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/35105.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/106434.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/38307.jpg} &
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/22274.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/32461.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/22348.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/43798.jpg}\\ 

% \textcolor{blue}{\emph{ix.}} F : (14, 16, 17) & \textcolor{blue}{\emph{x.}}  NF : (15, 22) & \textcolor{blue}{\emph{xi.}}  NF : (14, 20, 24) & \textcolor{blue}{\emph{xii.}}  NF : (13, 14, 24) & 
% \textcolor{blue}{\emph{xiii.}}  NF : (1, 2, 4) & \textcolor{blue}{\emph{xiv.}}  F : (17,24, 29) & \textcolor{blue}{\emph{xv.}} F : (5, 17) & \textcolor{blue}{\emph{xvi.}}  F : (13, 17, 29) \\ 
% \multicolumn{4}{c||}{glossy/ low resolution cover pages} & \multicolumn{4}{c|}{colorful/ busy background}\\
% %%%%%%%%%%%%%%%
% \hline
% \end{tabular}
% % \end{adjustbox}
% \caption{Some challenges of extracting OCR from book cover page}
% \label{fig:challenge_ocr}
% \end{figure*}


\begin{figure*}[t]
\centering
\footnotesize
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|c|c || c|c|c|c}
%%%%%%%%%%%%%%%
\hline 
&&& &&&&  \\[\dimexpr-\normalbaselineskip+1.5pt]
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/414.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/12916.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/12937.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/81539.jpg} &
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/67010.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/64126.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/11708.jpg} &
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/spanish_book.jpeg}\\
\textcolor{blue}{\emph{i.}} F : (16) & \textcolor{blue}{\emph{ii.}}  F : (16, 20, 29, 27) & \textcolor{blue}{\emph{iii.}}  F : (4, 27) & \textcolor{blue}{\emph{iv.}}  F : (11, 14, 16) & 
\textcolor{blue}{\emph{v.}}  F : (13, 16, 28) & \textcolor{blue}{\emph{vi.}}  F : (2, 4, 29, 27) & \textcolor{blue}{\emph{vii.}} NF : (13, 16, 28) & \textcolor{blue}{\emph{viii.}}  F : (22, 29) \\ 
\multicolumn{4}{c||}{Limited information} & \multicolumn{4}{c}{Non-English cover text}\\
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
\hline 
&&& &&&&  \\[\dimexpr-\normalbaselineskip+1.5pt]
%\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/67009.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/592713.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/35105.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/106434.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/38307.jpg} &
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/22274.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/32461.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/22348.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/OCR_challenges/43798.jpg}\\ 

\textcolor{blue}{\emph{ix.}} NF : (2, 13, 22) & \textcolor{blue}{\emph{x.}}  NF : (15, 22) & \textcolor{blue}{\emph{xi.}}  NF : (14, 20, 24) & \textcolor{blue}{\emph{xii.}}  NF : (13, 14, 24) & 
\textcolor{blue}{\emph{xiii.}}  NF : (1, 2, 4) & \textcolor{blue}{\emph{xiv.}}  F : (17,24, 29) & \textcolor{blue}{\emph{xv.}} F : (5, 17) & \textcolor{blue}{\emph{xvi.}}  F : (13, 17, 29) \\ 
\multicolumn{4}{c||}{Low resolution cover images} & \multicolumn{4}{c}{Complex background}\\
%%%%%%%%%%%%%%%
\hline
\end{tabular}
}
% \caption{Some challenges of extracting OCR from book cover page}
% \caption{Some challenges of extracted text from cover page}
\caption{Examples of some challenging cases involving text on cover page}
\label{fig:challenge_ocr}
\end{figure*}

% Examples of complex cases involving text elements on book covers.
% involving text on book covers



%%%%
   %%         1->'Animals & Wild life & Pets',
   %%		   2->'Arts & Photography',
   %%	       3->'Business & Money',
   %%	   4->'Childrens Book',
   %%	   5->'Comics & Graphic',
   %%		6->'Computers & Technology',
   %%		7->'Cookbooks & Food & Wine',
   %%		8->'Crafts & Hobbies & Home',
   %%		9->'Environment & Plant',
   %%		10->'Family & Parenting & Relationships',
   %%		11->'Fashion & Lifestyle',
   %%		12->'Health & Fitness & Dieting',
   %%		13->'History',
   %%		14->'Humanities',
   %%		15->'Humor & Entertainment',
   %%		16->'Literature',
   %%		17->'Mystery & Thriller & Suspense & Horror',
   %%		18->'Medical',
   %%		19->'Meta Text', 
   %%		20->'Mythology & Religion & Spirituality',
   %%		21->'Press & Media',
   %%		22->'Reference & Language',
   %%		23->'Romance',
   %%		24->'Science & Math & Mathematics',
   %%		25->'Self-Help & Motivation',
   %%		26->'Sports & Outdoors',
   %%		27->'Teen & Young Adult',
   %%		28->'Travel',
   %%		29->'Science Fiction & Fantasy'

  %%

==> tables/challenges_table.tex <==
% \begin{figure*}[t]
% \centering
% \footnotesize
% \makebox[\textwidth][c]{
% \begin{tabular}{c|c|c|c || c|c|c|c}
% %%%%%%%%%%%%%%%
% \hline 
% &&& &&&&  \\[\dimexpr-\normalbaselineskip+1.5pt]
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/challenes-no info.png} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/782705-less.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/2093-moderate.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/44950-moderate.jpg} &
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/19557.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/4948.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/441266.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/6357047.jpg} \\ 
% \textcolor{blue}{\emph{i.}} NF : (6) & \textcolor{blue}{\emph{ii.}}  NF : (11) & \textcolor{blue}{\emph{iii.}}  NF : (13, 14, 16, 24) & \textcolor{blue}{\emph{iv.}}  NF : (2, 13, 14) & 
% \textcolor{blue}{\emph{v.}}  NF : (7, 16, 22) & \textcolor{blue}{\emph{vi.}}  F : (1, 2, 4, 7) & \textcolor{blue}{\emph{vii.}}  NF : (3, 5, 13) & \textcolor{blue}{\emph{viii.}}  F : (16, 29)  \\ 
% \multicolumn{2}{c|}{less info} & \multicolumn{2}{c||}{moderate info} & \multicolumn{2}{c|}{adequate info} & \multicolumn{2}{c}{complex background}\\
% %%%%%%%%%%%%%%%
% \hline 
% &&& &&&&  \\[\dimexpr-\normalbaselineskip+1.5pt]
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/818388-nonliving.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/766869-nonliving.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/860691.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/901311-living.jpg} &
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/1214002-scene.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/110997.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/955747.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/1029194.jpg} \\ 
% \textcolor{blue}{\emph{ix.}} NF : (20, 28) & \textcolor{blue}{\emph{x.}}  F : (16, 17, 23, 29) & \textcolor{blue}{\emph{xi.}}  F : (2, 15, 16) & \textcolor{blue}{\emph{xii.}}  F : (9, 14) & 
% \textcolor{blue}{\emph{xiii.}}  NF : (2) & \textcolor{blue}{\emph{xiv.}}  NF : (14, 20, 24, 25) & \textcolor{blue}{\emph{xv.}}  F : (10, 11, 23) & \textcolor{blue}{\emph{xvi.}} F : (4, 29, 27)  \\ 
% \multicolumn{2}{c|}{non living object} & \multicolumn{2}{c||}{living object} & \multicolumn{4}{c|}{scene}\\
% %%%%%%%%%%%%%%%
% \hline 
% &&& &&&&  \\[\dimexpr-\normalbaselineskip+1.5pt]
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/100915-intervariation.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/60187486-intervariation.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/10785687-intervariation.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/45286449-intervariation.jpg} &
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/281979.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/4812002.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/663869-intra.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/916347-intra.jpg} \\ 
% \textcolor{blue}{\emph{xvii.}} F : (29, 27, 4) & \textcolor{blue}{\emph{xviii.}}  NF : (20) & \textcolor{blue}{\emph{xix.}}  NF : (22, 19, 27) & \textcolor{blue}{\emph{xx.}}  F : (2, 4, 16, 27) & 
% \textcolor{blue}{\emph{xxi.}}  NF : (2, 24) & \textcolor{blue}{\emph{xxii.}}  NF : (2, 24) & \textcolor{blue}{\emph{xxiii.}}  F : (13, 14, 16, 29) & \textcolor{blue}{\emph{xxiv.}}  F : (13, 14, 16, 19)  \\ 
% \multicolumn{2}{c|}{inter-variation} & \multicolumn{2}{c||}{inter-variation} & \multicolumn{2}{c|}{intra-variation} & \multicolumn{2}{c}{intra-variation}\\ 
% %%%%%%%%%%%%%%%
% \hline 
% &&& &&&&  \\[\dimexpr-\normalbaselineskip+1.5pt]
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/371776.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/36261.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/54944.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/936724.jpg} &
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/60862571.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/529109_updated_1.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/50181-hazy.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/67009-noisy.jpg} \\ 
% \textcolor{blue}{\emph{xxv.}} NF : (2, 13, 20) & \textcolor{blue}{\emph{xxvi.}}  NF : (2, 13, 14) & \textcolor{blue}{\emph{xxvii.}}  NF : (10, 11, 14, 25) & \textcolor{blue}{\emph{xxviii.}}  F : (4, 29, 27) & 
% \textcolor{blue}{\emph{xxix.}}  F : (11, 16, 23) & \textcolor{blue}{\emph{xxx.}}  F : (21, 29) & \textcolor{blue}{\emph{xxxi.}} (16, 27, 13) & \textcolor{blue}{\emph{xxxii.}}  F : (14, 16, 17) \\ 
% \multicolumn{4}{c||}{collage} & \multicolumn{2}{c|}{text/ number as image} & \multicolumn{2}{c}{hazy image}\\
% %%%%%%%%%%%%%%%
% \hline
% \end{tabular}}
% \caption{Examples of some challenging cover page images with mentioned issues}
% \label{fig:challenge}
% \end{figure*}


\begin{figure*}[t]
\centering
\footnotesize
\makebox[\textwidth][c]{
\begin{adjustbox}{width=\linewidth}
\begin{tabular}{c|c|c|c || c|c|c|c}
%%%%%%%%%%%%%%%
\hline 
&&& &&&&  \\[\dimexpr-\normalbaselineskip+1.5pt]
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/3798692_less_info.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/52699907_less_info.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/441266.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/6357047.jpg} &
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/2093-moderate.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/44950-moderate.jpg} &
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/19557.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/4948.jpg} 
\\ 
\textcolor{blue}{\emph{i.}} F : (13, 14, 28, 30) & \textcolor{blue}{\emph{ii.}}  NF : (16, 22, 24) & 
\textcolor{blue}{\emph{iii.}}  NF : (3, 5, 13) & \textcolor{blue}{\emph{iv.}}  F : (16, 29) & 
\textcolor{blue}{\emph{v.}}  NF : (13, 14, 16, 24) & \textcolor{blue}{\emph{vi.}}  NF : (2, 13, 14) & 
\textcolor{blue}{\emph{vii.}}  NF : (7, 16, 22) & \textcolor{blue}{\emph{viii.}}  F : (1, 2, 4, 7)   \\ 
\multicolumn{2}{c|}{Limited visual cues} & \multicolumn{2}{c||}{Complex background} & \multicolumn{4}{c}{Moderate info} \\
%%%%%%%%%%%%%%%
\hline 
&&& &&&&  \\[\dimexpr-\normalbaselineskip+1.5pt]
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/818388-nonliving.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/766869-nonliving.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/860691.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/901311-living.jpg} &
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/1214002-scene.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/110997.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/jack_of_souls.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/955747.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/1029194.jpg} 
\\ 
\textcolor{blue}{\emph{ix.}} NF : (20, 28) & \textcolor{blue}{\emph{x.}}  F : (16, 17, 23, 29) & \textcolor{blue}{\emph{xi.}}  F : (2, 15, 16) & \textcolor{blue}{\emph{xii.}}  F : (9, 14) & 
\textcolor{blue}{\emph{xiii.}}  NF : (2) & \textcolor{blue}{\emph{xiv.}}  F : (29, 23, 27, 17) & \textcolor{blue}{\emph{xv.}}  F : (10, 11, 23) & \textcolor{blue}{\emph{xvi.}} F : (4, 29, 27)  \\ 
\multicolumn{2}{c|}{Non-living element} & \multicolumn{2}{c||}{living element} & \multicolumn{4}{c|}{Scene image}\\
%%%%%%%%%%%%%%%
\hline 
&&& &&&&  \\[\dimexpr-\normalbaselineskip+1.5pt]
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/100915-intervariation.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/60187486-intervariation.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/10785687-intervariation.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/45286449-intervariation.jpg} &
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/281979.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/4812002.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/663869-intra.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/916347-intra.jpg} \\ 
\textcolor{blue}{\emph{xvii.}} F : (29, 27, 4) & \textcolor{blue}{\emph{xviii.}}  NF : (20) & \textcolor{blue}{\emph{xix.}}  NF : (22, 19, 27) & \textcolor{blue}{\emph{xx.}}  F : (2, 4, 16, 27) & 
\textcolor{blue}{\emph{xxi.}}  NF : (2, 24) & \textcolor{blue}{\emph{xxii.}}  NF : (2, 24) & \textcolor{blue}{\emph{xxiii.}}  F : (13, 14, 16, 29) & \textcolor{blue}{\emph{xxiv.}}  F : (13, 14, 16, 19)  \\ 
\multicolumn{2}{c|}{Inter-variation} & \multicolumn{2}{c||}{Inter-variation} & \multicolumn{2}{c|}{Intra-variation} & \multicolumn{2}{c}{Intra-variation}\\ 
%%%%%%%%%%%%%%%
\hline 
&&& &&&&  \\[\dimexpr-\normalbaselineskip+1.5pt]
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/371776.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/36261.jpg} & 
% \includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/54944.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/1196764.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/936724.jpg} &
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/60862571.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/529109_updated_1.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/50181-hazy.jpg} & 
\includegraphics[width=0.1\linewidth, height=0.145\linewidth]{figs/coverpage_challenges/67009-noisy.jpg} \\ 
\textcolor{blue}{\emph{xxv.}} NF : (2, 13, 20) & \textcolor{blue}{\emph{xxvi.}}  NF : (2, 13, 14) & \textcolor{blue}{\emph{xxvii.}}  NF : (3, 13, 14) & \textcolor{blue}{\emph{xxviii.}}  F : (4, 29, 27) & 
\textcolor{blue}{\emph{xxix.}}  F : (11, 16, 23) & \textcolor{blue}{\emph{xxx.}}  F : (21, 29) & \textcolor{blue}{\emph{xxxi.}} F : (16, 27, 13) & \textcolor{blue}{\emph{xxxii.}}  F : (14, 16, 17) \\ 
\multicolumn{4}{c||}{Collage} & \multicolumn{2}{c|}{Number/ letter as image} & \multicolumn{2}{c}{Unclear image}\\
%%%%%%%%%%%%%%%
\hline
\end{tabular}
\end{adjustbox}
}
\caption{Examples of some challenging book cover images with mentioned issues}
\label{fig:challenge}
\end{figure*}


==> tables/dt.tex <==
\begin{table}[!b] 
\centering  
\caption{Hierarchical genre-wise count of the dataset} \label{tab1} 
\begin{adjustbox}{width=\textwidth}
    \begin{tabular}{c |l |c |c | c| l |c |c}
    \hline
    \textbf{Class ID} & \textbf{Genre label} & \textbf{Fiction} & \textbf{Non-fiction} & \textbf{Class ID} & \textbf{Genre label} & \textbf{Fiction} & \textbf{Non-fiction} \\ \hline \hline
    1 & Animals \& Wildlife \& Pets & 590 & 235 & Literature & 2615 & 670 \\ \hline 
    
    \multirow{2}{*}{2} & \multirow{2}{*}{Arts \& Photography} & \multirow{2}{*}{1188} & \multirow{2}{*}{606} & 16 & \multirow{2}{*}{17} & Mystery \& Thriller \& & \multirow{2}{*}{2043} & \multirow{2}{*}{404} \\ 
    & & & & & Suspense \& Horror \& Adventure & & \\ \hline 
    
    3 & Business \& Money & 42 & 256 & 18 & Medical & 70 & 165  \\ \hline
    
    4 & {Childrens\textquoteright} Book & 1714 & 298 & 19 & Meta Text & 35 & 88  \\ \hline 
    
    5 & Comics \& Graphic & 364 & 96 & 20 & Mythology \& Religion \& Spirituality & 890 & 748 \\ \hline 
    
    6 & Computers \& Technology & 27 & 92 & 21 & Press \& Media & 138  & 167  \\ \hline 
    
    7 & Cookbooks \& Food \& Wine & 72 & 223 & 22 & Reference \& Language & 97 & 1003  \\ \hline  

    8 & Crafts \& Hobbies \& Home & 40  & 61 & 23 & Romance & 1445 & 80 \\ \hline  
    
    9 & Environment \& Plant & 92 & 337 & 24 & Science \& Math & 419  & 712 \\ \hline

    10 & Family \& Parenting \& Relationships & 208 & 257 & 25 & Self-help \& Motivation & 72 & 630 \\ \hline 

    11 & Fashion \& Lifestyle & 732 & 204 & 26 & Sports \& Outdoors & 183  & 157 \\ \hline 
    
    12 & Health \& Fitness \& Dieting & 32 & 320 & 27 & Teen \& Young Adult & 1712 & 170 \\ \hline

    13 & History & 1677 & 1619 & 28 & Travel & 92 & 393 \\ \hline
    
    14 & Humanities & 537 & 1555 & 29 & Sci-Fi \& Fantasy & 2715 & \--- \\ \hline 
    
    15 & Humor \& Entertainment & 972 & 376 & 30 & Biographies \& Memoir & \--- & 1256 \\ 


    
    % 16 & Literature & 2615 & 6088 & 670 & 1786 \\ \hline 
    % \multirow{2}{*}{17} & Mystery \& Thriller \& & \multirow{2}{*}{2043} & \multirow{2}{*}{4289} & \multirow{2}{*}{404} & \multirow{2}{*}{920} \\  
    % & Suspense \& Horror \& Adventure & & & & \\ \hline 
    % 18 & Medical & 70 & 950 & 165 & 1080 \\ \hline 
    % 19 & Meta Text & 35 & 774 & 88 & 954 \\ \hline 
    % 20 & Mythology \& Religion \& Spirituality & 890 & 1909 & 748 & 1376 \\ \hline 
    % 21 & Press \& Media & 138 & 486 & 167 & 903 \\ \hline 
    % 22 & Reference \& Language & 97 & 694 & 1003 & 3077 \\ \hline 
    % 23 & Romance & 1445 & 2275 & 80 & 1065 \\ \hline 
    % 24 & Science \& Math & 419 & 718 & 712 & 2221 \\ \hline 
    % &  \& Mathematics & & & & \\ \hline 
    % 25 & Self-help \& Motivation & 72 & 993 & 630 & 1865 \\ \hline 
    % 26 & Sports \& Outdoors & 183 & 825 & 157 & 522 \\ \hline 
    % 27 & Teen \& Young Adult & 1712 & 2524 & 170 & 817 \\ \hline 
    % 28 & Travel & 92 & 743 & 393 & 1090 \\ \hline 
    % 29 & Sci-Fi \& Fantasy & 2715 & 5034 & \--- & \--- \\ \hline 
    % 30 & Biographies \& Memoir & \--- & \--- & 1256 & 3466 \\  
    \hline
    \end{tabular}
    \end{adjustbox}
    \label{tab:dataset_table}
\end{table}






==> tables/heatmap.tex <==
\begin{figure*}[!hbt]
\centering

% \begin{adjustbox}{angle=90, height=1\textheight}
\begin{adjustbox}{width=0.88\textwidth} 
\begin{tabular}{cc|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\hline

\multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & 
\multicolumn{2}{c|}{Level-1} & \multicolumn{30}{c}{Level-2 Classification} \\
\cline{3-34} 
%%%%%% Actual
\multicolumn{1}{c}{} & \multicolumn{1}{c|}{Class ID}  & NF & F & 1 & 2& 3 & 4& 5& 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & 28 & 29 & 30 \\ 
% \cline{2-34} 
\hline \hline 

\multirow{10}{*}{\textbf{\rotatebox{90}{\underline{Ground-truth}}}} & \textcolor{blue}{\emph{(a)}} & \cellcolor[gray]{0} & \cellcolor[gray]{1} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} \\ \cline{2-34} 

 & \textcolor{blue}{\emph{(b)}} & \cellcolor[gray]{0} & \cellcolor[gray]{1} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} \\ \cline{2-34} 
 
 & \textcolor{blue}{\emph{(c)}} & \cellcolor[gray]{1} & \cellcolor[gray]{0} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} \\ \cline{2-34} 
 
 & \textcolor{blue}{\emph{(d)}} & \cellcolor[gray]{1} & \cellcolor[gray]{0} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} \\ \cline{2-34} 
 
 & \textcolor{blue}{\emph{(e)}} & \cellcolor[gray]{1} & \cellcolor[gray]{0} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} \\ \cline{2-34}
 
 & \textcolor{blue}{\emph{(f)}} & \cellcolor[gray]{1} & \cellcolor[gray]{0} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} \\ \cline{2-34} 
 
 & \textcolor{blue}{\emph{(g)}} & \cellcolor[gray]{0} & \cellcolor[gray]{1} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} \\ \cline{2-34} 
 
 &\textcolor{blue}{\emph{(h)}} & \cellcolor[gray]{1} & \cellcolor[gray]{0} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} \\ \cline{2-34} 
 & \textcolor{blue}{\emph{(i)}} & \cellcolor[gray]{0} & \cellcolor[gray]{1} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} \\ \cline{2-34} 
 & \textcolor{blue}{\emph{(j)}} & \cellcolor[gray]{1} & \cellcolor[gray]{0} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{1.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} \\ 
 \hline \hline


%%%%%%%% Predicted

 
\multirow{10}{*}{\textbf{\rotatebox{90}{\underline{Predicted score}}}} & \textcolor{blue}{\emph{(a)}} & \cellcolor[gray]{0.00044} & \cellcolor[gray]{0.99956} & \cellcolor[gray]{0.99476} & \cellcolor[gray]{0.99909} & \cellcolor[gray]{0.00001} & \cellcolor[gray]{0.99997} & \cellcolor[gray]{0.00083} & \cellcolor[gray]{0.00002} & \cellcolor[gray]{0.94047} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00563} & \cellcolor[gray]{0.99830} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00056} & \cellcolor[gray]{0.00066} & \cellcolor[gray]{0.00122} & \cellcolor[gray]{0.03674} & \cellcolor[gray]{0.99246} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00550} & \cellcolor[gray]{0.00044} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00014} & \cellcolor[gray]{0.00006} & \cellcolor[gray]{0.00023} & \cellcolor[gray]{0.00008} & \cellcolor[gray]{0.00006} & \cellcolor[gray]{0.00002} & \cellcolor[gray]{0.00533} & \cellcolor[gray]{0.00015} & \cellcolor[gray]{0.03099} & \cellcolor[gray]{0.00000} \\ \cline{2-34} 

 & \textcolor{blue}{\emph{(b)}} & \cellcolor[gray]{0.00016} & \cellcolor[gray]{0.99984} & \cellcolor[gray]{0.00133} & \cellcolor[gray]{0.01118} & \cellcolor[gray]{0.00027} & \cellcolor[gray]{0.00066} & \cellcolor[gray]{0.99569} & \cellcolor[gray]{0.04551} & \cellcolor[gray]{0.00032} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00001} & \cellcolor[gray]{0.00002} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.03169} & \cellcolor[gray]{0.00016} & \cellcolor[gray]{0.02745} & \cellcolor[gray]{0.00027} & \cellcolor[gray]{0.00545} & \cellcolor[gray]{0.00022} & \cellcolor[gray]{0.00001} & \cellcolor[gray]{0.00010} & \cellcolor[gray]{0.00255} & \cellcolor[gray]{0.00001} & \cellcolor[gray]{0.99160} & \cellcolor[gray]{0.00353} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00004} & \cellcolor[gray]{0.10041} & \cellcolor[gray]{0.00222} & \cellcolor[gray]{0.97165} & \cellcolor[gray]{0.00000} \\ \cline{2-34} 
 
 & \textcolor{blue}{\emph{(c)}} & \cellcolor[gray]{0.99994} & \cellcolor[gray]{0.00006} & \cellcolor[gray]{0.00007} & \cellcolor[gray]{0.00004} & \cellcolor[gray]{0.00007} & \cellcolor[gray]{0.03481} & \cellcolor[gray]{0.00017} & \cellcolor[gray]{0.00009} & \cellcolor[gray]{0.97895} & \cellcolor[gray]{0.00046} & \cellcolor[gray]{0.00542} & \cellcolor[gray]{0.01889} & \cellcolor[gray]{0.00044} & \cellcolor[gray]{0.99680} & \cellcolor[gray]{0.00002} & \cellcolor[gray]{0.00266} & \cellcolor[gray]{0.00002} & \cellcolor[gray]{0.00476} & \cellcolor[gray]{0.01359} & \cellcolor[gray]{0.82687} & \cellcolor[gray]{0.00702} & \cellcolor[gray]{0.00038} & \cellcolor[gray]{0.00001} & \cellcolor[gray]{0.99791} & \cellcolor[gray]{0.00092} & \cellcolor[gray]{0.00011} & \cellcolor[gray]{0.99844} & \cellcolor[gray]{0.00979} & \cellcolor[gray]{0.00001} & \cellcolor[gray]{0.00032} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00001} \\ \cline{2-34} 
 
 & \textcolor{blue}{\emph{(d)}} & \cellcolor[gray]{0.99635} & \cellcolor[gray]{0.00365} & \cellcolor[gray]{0.99472} & \cellcolor[gray]{0.00016} & \cellcolor[gray]{0.00009} & \cellcolor[gray]{0.00001} & \cellcolor[gray]{0.00002} & \cellcolor[gray]{0.00004} & \cellcolor[gray]{0.00303} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00361} & \cellcolor[gray]{0.00086} & \cellcolor[gray]{0.00008} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00635} & \cellcolor[gray]{0.00004} & \cellcolor[gray]{0.00166} & \cellcolor[gray]{0.00040} & \cellcolor[gray]{0.00005} & \cellcolor[gray]{0.00005} & \cellcolor[gray]{0.01653} & \cellcolor[gray]{0.00047} & \cellcolor[gray]{0.00008} & \cellcolor[gray]{0.00086} & \cellcolor[gray]{0.00274} & \cellcolor[gray]{0.00353} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00002} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00001} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.99131} \\ \cline{2-34} 
 
 & \textcolor{blue}{\emph{(e)}} & \cellcolor[gray]{0.99991} & \cellcolor[gray]{0.00009} & \cellcolor[gray]{0.00002} & \cellcolor[gray]{0.00099} & \cellcolor[gray]{0.99969} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00419} & \cellcolor[gray]{0.01303} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00003} & \cellcolor[gray]{0.00002} & \cellcolor[gray]{0.04246} & \cellcolor[gray]{0.00810} & \cellcolor[gray]{0.00004} & \cellcolor[gray]{0.00268} & \cellcolor[gray]{0.98886} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00006} & \cellcolor[gray]{0.00004} & \cellcolor[gray]{0.00378} & \cellcolor[gray]{0.00823} & \cellcolor[gray]{0.90046} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00545} & \cellcolor[gray]{0.00357} & \cellcolor[gray]{0.00013} & \cellcolor[gray]{0.99689} & \cellcolor[gray]{0.00008} & \cellcolor[gray]{0.00005} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00358} \\ \cline{2-34} 
 
 & \textcolor{blue}{\emph{(f)}} & \cellcolor[gray]{0.99993} & \cellcolor[gray]{0.00007} & \cellcolor[gray]{0.00021} & \cellcolor[gray]{0.00002} & \cellcolor[gray]{0.00009} & \cellcolor[gray]{0.00027} & \cellcolor[gray]{0.00241} & \cellcolor[gray]{0.00001} & \cellcolor[gray]{0.02858} & \cellcolor[gray]{0.01158} & \cellcolor[gray]{0.93981} & \cellcolor[gray]{0.00048} & \cellcolor[gray]{0.00162} & \cellcolor[gray]{0.03215} & \cellcolor[gray]{0.00400} & \cellcolor[gray]{0.00079} & \cellcolor[gray]{0.00082} & \cellcolor[gray]{0.00392} & \cellcolor[gray]{0.91136} & \cellcolor[gray]{0.00001} & \cellcolor[gray]{0.00181} & \cellcolor[gray]{0.00202} & \cellcolor[gray]{0.00007} & \cellcolor[gray]{0.99415} & \cellcolor[gray]{0.00998} & \cellcolor[gray]{0.00002} & \cellcolor[gray]{0.00505} & \cellcolor[gray]{0.99881} & \cellcolor[gray]{0.01750} & \cellcolor[gray]{0.97146} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.11416} \\ \cline{2-34} 
 
 & \textcolor{blue}{\emph{(g)}} & \cellcolor[gray]{0.00008} & \cellcolor[gray]{0.99992} & \cellcolor[gray]{0.00213} & \cellcolor[gray]{0.04993} & \cellcolor[gray]{0.00258} & \cellcolor[gray]{0.00845} & \cellcolor[gray]{0.00705} & \cellcolor[gray]{0.00096} & \cellcolor[gray]{0.00517} & \cellcolor[gray]{0.00225} & \cellcolor[gray]{0.00287} & \cellcolor[gray]{0.42612} & \cellcolor[gray]{0.71277} & \cellcolor[gray]{0.01147} & \cellcolor[gray]{0.92822} & \cellcolor[gray]{0.00258} & \cellcolor[gray]{0.17138} & \cellcolor[gray]{0.07084} & \cellcolor[gray]{0.00624} & \cellcolor[gray]{0.04806} & \cellcolor[gray]{0.03481} & \cellcolor[gray]{0.04279} & \cellcolor[gray]{0.01641} & \cellcolor[gray]{0.00774} & \cellcolor[gray]{0.85877} & \cellcolor[gray]{0.11464} & \cellcolor[gray]{0.00673} & \cellcolor[gray]{0.00154} & \cellcolor[gray]{0.05980} & \cellcolor[gray]{0.00338} & \cellcolor[gray]{0.01469} & \cellcolor[gray]{0.00000} \\ \cline{2-34} 
 & \textcolor{blue}{\emph{(h)}} & \cellcolor[gray]{0.99975} & \cellcolor[gray]{0.00025} & \cellcolor[gray]{0.00133} & \cellcolor[gray]{0.00295} & \cellcolor[gray]{0.92140} & \cellcolor[gray]{0.01267} & \cellcolor[gray]{0.01531} & \cellcolor[gray]{0.87444} & \cellcolor[gray]{0.04635} & \cellcolor[gray]{0.00045} & \cellcolor[gray]{0.00879} & \cellcolor[gray]{0.00264} & \cellcolor[gray]{0.01290} & \cellcolor[gray]{0.00145} & \cellcolor[gray]{0.98127} & \cellcolor[gray]{0.33684} & \cellcolor[gray]{0.00039} & \cellcolor[gray]{0.05179} & \cellcolor[gray]{0.00029} & \cellcolor[gray]{0.05201} & \cellcolor[gray]{0.01190} & \cellcolor[gray]{0.00225} & \cellcolor[gray]{0.06651} & \cellcolor[gray]{0.00788} & \cellcolor[gray]{0.00283} & \cellcolor[gray]{0.82674} & \cellcolor[gray]{0.00126} & \cellcolor[gray]{0.00023} & \cellcolor[gray]{0.24525} & \cellcolor[gray]{0.03039} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.18526} \\ \cline{2-34} 
 & \textcolor{blue}{\emph{(i)}} & \cellcolor[gray]{0.00315} & \cellcolor[gray]{0.99685} & \cellcolor[gray]{0.00671} & \cellcolor[gray]{0.80333} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.85072} & \cellcolor[gray]{0.00034} & \cellcolor[gray]{0.00014} & \cellcolor[gray]{0.00026} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00001} & \cellcolor[gray]{0.00009} & \cellcolor[gray]{0.00004} & \cellcolor[gray]{0.00500} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00001} & \cellcolor[gray]{0.99992} & \cellcolor[gray]{0.00002} & \cellcolor[gray]{0.03822} & \cellcolor[gray]{0.00001} & \cellcolor[gray]{0.99222} & \cellcolor[gray]{0.00018} & \cellcolor[gray]{0.00008} & \cellcolor[gray]{0.00030} & \cellcolor[gray]{0.00001} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.01542} & \cellcolor[gray]{0.04668} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.99957} & \cellcolor[gray]{0.00000} \\ \cline{2-34} 
 & \textcolor{blue}{\emph{(j)}} & \cellcolor[gray]{0.99802} & \cellcolor[gray]{0.00198} & \cellcolor[gray]{0.01750} & \cellcolor[gray]{0.97278} & \cellcolor[gray]{0.05179} & \cellcolor[gray]{0.17395} & \cellcolor[gray]{0.00997} & \cellcolor[gray]{0.05670} & \cellcolor[gray]{0.00747} & \cellcolor[gray]{0.13790} & \cellcolor[gray]{0.00693} & \cellcolor[gray]{0.00516} & \cellcolor[gray]{0.07648} & \cellcolor[gray]{0.00456} & \cellcolor[gray]{0.07431} & \cellcolor[gray]{0.08559} & \cellcolor[gray]{0.14760} & \cellcolor[gray]{0.01880} & \cellcolor[gray]{0.00740} & \cellcolor[gray]{0.01624} & \cellcolor[gray]{0.01769} & \cellcolor[gray]{0.00190} & \cellcolor[gray]{0.66830} & \cellcolor[gray]{0.96815} & \cellcolor[gray]{0.07242} & \cellcolor[gray]{0.15810} & \cellcolor[gray]{0.13284} & \cellcolor[gray]{0.00079} & \cellcolor[gray]{0.68137} & \cellcolor[gray]{0.00128} & \cellcolor[gray]{0.00000} & \cellcolor[gray]{0.00036} \\ 
 \hline

 \multicolumn{34}{r}{L-1: Level-1 classification, NF: \textit{non-fiction}, F: \textit{fiction}}
\end{tabular}
\end{adjustbox}
\caption{Ground-truth and IMaGINe-predicted confidence score heat-map encodings in gray color code}
\label{tab:heatmap}
\end{figure*}

==> tables/heatmap_sample.tex <==
\begin{table*}[!hbt]
\centering
\caption{Data samples for heatmap}
\begin{adjustbox}{width=0.88\textwidth}
% \begin{adjustbox}{angle=90, height=1\textheight}
% \footnotesize
\begin{tabular}{c|ll}%p{0.9\textwidth}}
% \multicolumn{3}{c}{(a) Samples for heatmap analysis}\\
\hline %\hline
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \\[\dimexpr -\normalbaselineskip+1.5pt]

\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textcolor{blue}{\emph{(a)}} \textbf{9780060223595: Bread and Jam for Frances; Author: Russell Hoban; Publisher: HarperCollins Publishers}}\\
\hline %\hline
% & \\ [\dimexpr-\normalbaselineskip+1.5pt]

\multirow{5}{*}{\includegraphics[width=0.04\linewidth, height=0.05\linewidth]{figs/heatmap/1.jpg}} & \multirow{4}{*}{\textbf{Blurb}:} & The classic funny story about a stubborn little badger with very particular tastes in food. Frances is a fussy eater. In fact, the only thing she likes is bread and jam. She won't  \\
& & touch her squishy soft-boiled egg. She trades away her chicken-salad sandwich at lunch. She turns up her nose at boring veal cutlets. Unless her parents can come up with a \\
& &    plan, Frances just might go on eating bread and jam forever! Join the generations of families that have laughed along as Frances sings "Jam on biscuits, jam on bread,\\
& &   Jam is the thing I like most, Jam is sticky, jam is sweet, Jam is tasty, jam’s a treat—raspberry, strawberry, gooseberry, I’m very FOND…OF…JAM!"\\ \cline{2-3}
% & ${\cal{M}}$ & \{"author":"Russell Hoban","publisher":"HarperCollins Publishers"\}\\ \hline
& \multicolumn{1}{l}{\textbf{Actual Genre}:} & (Fiction, \{Animals \& Wildlife \& Pets, Arts \& Photography, {Childrens\textquoteright} Book, Cookbooks \& Food \& Wine, Family \& Parenting \& Relationships, Literature\})\\ 

\hline \hline

\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textcolor{blue}{\emph{(b)}} \textbf{9782723423014: Sailor Moon, tome 14 : Le royaume Elusion; Author: Naoko Takeuchi; Publisher: GLÉNAT}}\\
\hline 

\multirow{3}{*}{\includegraphics[width=0.04\linewidth, height=0.05\linewidth]{figs/heatmap/2.jpg}} & \multirow{2}{*}{\textbf{Blurb}:} & A graphic novel offers the continuing adventures of Serena and her friends, who use the power of the moon and the planets, as the superhero Sailor Moon and her comrades, \\
& &  to battle the forces of evil. \\ \cline{2-3}

% & ${\cal{M}}$ & \{"author":"Naoko Takeuchi","publisher":"GLÉNAT"\}\\ \hline
& \multicolumn{1}{l}{\textbf{Actual Genre}:} & (Fiction, \{Comics \& Graphic, Romance, Science Fiction \& Fantasy\})\\

\hline \hline
\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textcolor{blue}{\emph{(c)}} \textbf{9780895297273: Prescription for Nutritional Healing: A Practical A-Z Reference to Drug-Free Remedies Using Vitamins, Minerals, Herbs \& Food Supplements;}}\\
\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{ \textbf{
Author: James F. Balch; Publisher: Avery Publishing Group}} \\
\hline 
\multirow{3}{*}{\includegraphics[width=0.04\linewidth, height=0.05\linewidth]{figs/heatmap/3.jpg}} & \multirow{2}{*}{\textbf{Blurb}:} & An alphabetical encyclopedia of nutritional treatments for a wide range of common ailments explains how to use vitamins, herbs, minerals, and food supplements to promote \\
& &  healing and wellness.\\ \cline{2-3}
% & ${\cal{M}}$ & \{"author":"James F.,Md. Balch","publisher":"Avery Publishing Group"\}\\ \hline
& \multicolumn{1}{l}{\textbf{Actual Genre}:} & (Non-fiction, \{Cookbooks \& Food \& Wine, Health \& Fitness \& Dieting, Medical, Reference \& Language, Self-Help \& Motivation\})\\



\hline \hline
\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textcolor{blue}{\emph{(d)}} \textbf{9780060172732: The Dog Who Rescues Cats: The True Story of Ginny; Author: Philip Gonzalez; Publisher: Harpercollins}}\\
\hline 
\multirow{3}{*}{\includegraphics[width=0.04\linewidth, height=0.05\linewidth]{figs/heatmap/4.jpg}} & \multirow{2}{*}{\textbf{Blurb}:} & The true story of Ginny, an abused dog with an affinity for rescuing cats in trouble, describes Ginny's part in the saving of such handicapped felines as the one-eyed Revlon, \\
& &  deaf Madam, and the paralyzed Topsy. \\ \cline{2-3}

% & ${\cal{M}}$ & \{"author":"Philip Gonzalez","publisher":"Harpercollins"\}\\ \hline
& \multicolumn{1}{l}{\textbf{Actual Genre}:} & (Non-fiction, \{Animals \& Wildlife \& Pets, Biographies \& Memoir\})\\





\hline \hline
\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textcolor{blue}{\emph{(e)}} \textbf{9780671668365: MAGIC OF CONFLICT; Author: Thomas Crum; Publisher: Touchstone}}\\
\hline 
\multirow{3}{*}{\includegraphics[width=0.04\linewidth, height=0.05\linewidth]{figs/heatmap/5.jpg}} & \multirow{2}{*}{\textbf{Blurb}:} & Gives techniques for transforming conflict into an opportunity for choice and change and how to grow beyond the striving competitiveness, and pressure of personal and \\
& &  professional life. \\ \cline{2-3}

% & ${\cal{M}}$ & \{"author":"Thomas Crum","publisher":"Touchstone"\}\\
% \hline

& \multicolumn{1}{l}{\textbf{Actual Genre}:} & (Non-fiction, \{Business \& Money, Humanities, Mythology \& Religion \& Spirituality, Self-Help \& Motivation\})\\



\hline \hline
\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textcolor{blue}{\emph{(f)}} \textbf{9780963235930: Beyond Backpacking: Ray Jardines Guide to Lightweight Hiking; Author: Ray Jardine; Publisher: Adventurelore Press}}\\
\hline 


\multirow{3}{*}{\includegraphics[width=0.04\linewidth, height=0.05\linewidth]{figs/heatmap/6.jpg}} & \multirow{2}{*}{\textbf{Blurb}:} & Beyond Backpacking has 517 pages of "practical methods for all who love the out-of-doors". Chapters include Equipment, Hiking Considerations, Obstacles, Longer  \\
& & Journeys and Back to Basics.  \\
\cline{2-3}
% & ${\cal{M}}$ & \{"author":"Ray Jardine","publisher":"Adventurelore Press"\}\\
% \hline
& \multicolumn{1}{l}{\textbf{Actual Genre}:} & (Non-fiction, \{Environment \& Plant, Mystery \& Thriller \& Suspense \& Horror, Reference \& Language, Sports \& Outdoors, Travel\})\\



\hline \hline
\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textcolor{blue}{\emph{(g)}} \textbf{9780380773527: Dreaming of You; Author: Lisa Kleypas; Publisher: Avon}}\\
\hline 
\multirow{7}{*}{\includegraphics[width=0.04\linewidth, height=0.05\linewidth]{figs/heatmap/7.jpg}} & \multirow{6}{*}{\textbf{Blurb}:} & She stood at danger's threshold—then love beckoned her in.A prim, well-bred gentlewoman, Sara Fielding is a writer who puts pen to paper to create dreams. But now\\
& &   curiosity is luring her from the shelter of her country cottage into the dangerous world of Derek Craven—handsome, tough, and tenacious—and the most exciting man Sara \\
& &  has ever met. Derek rose from poverty to become the wealthy lord of London’s most exclusive gambling house. And now duty demands that he allow Sara Fielding to \\
& &  enter his perilous realm of ever-shifting fortunes—with her impeccable manners and her infuriating innocence. But there is a hidden strength and sensuality to the lady that\\
& &    captivates him beyond  his better judgment.And in this world, where danger lurks behind every shadow, even a proper “mouse” can be transformed into a breathtaking \\
& &  enchantress—and a cynical gambler can be shaken to his core by the power of passion and the promise of love.\\
\cline{2-3}
& \multicolumn{1}{l}{\textbf{Actual Genre}:} & (Fiction, \{Fashion \& Lifestyle, History, Romance\})\\



\hline \hline

\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textbf{{\emph{(h).}} 9780679602613: The Soul of a New Machine; Author: TRACY KIDDER; Publisher: Modern Library}}\\
\hline \hline

\multirow{13}{*}{\includegraphics[width=0.04\linewidth, height=0.05\linewidth]{figs/heatmap/8.jpg}} & \multirow{12}{*}{\textbf{Blurb}:} & Winner of the Pulitzer Prize and the American Book Award, The Soul of a New Machine was a bestseller on its first publication in 1981. With the touch of an expert thriller\\
& &    writer, Tracy Kidder recounts the feverish efforts of a team of Data General researchers to create a new 32-bit superminicomputer. A compelling account of individual sacrifice \\
& &    and human ingenuity, The Soul of a New Machine endures as the classic chronicle of the computer age and the masterminds behind its technological advances. "A superb \\
& &   book," said Robert Pirsig, author of Zen and the Art of Motorcycle Maintenance. "All the incredible complexity and chaos and exploitation and loneliness and strange,\\
& &     half-mad beauty of this field are honestly and correctly drawn." The Washington Post Book World said, "Kidder has created compelling entertainment.  He offers a fast,\\
& &    painless, enjoyable means to an initial understanding of computers, allowing us to understand the complexity of machines  we could only marvel at before, and to appreciate\\

& &   the skills of the people who create them."The Modern Library has played a significant role in American cultural  life for the better part of a century. The series was founded\\
& &   in 1917 by the publishers Boni and Liveright and eight years later acquired by Bennett Cerf and Donald Klopfer. It provided the foundation for their next publishing venture,\\

& &   Random House. The Modern Library has been a staple of the American book trade, providing readers with affordable hardbound editions of important works of literature and \\
& & thought. For the Modern Library's seventy-fifth anniversary, Random House redesigned the series, restoring as its emblem the running torch-bearer created by Lucian Bernhard \\

&  & in 1925 and refurbishing jackets, bindings, and type, as well as inaugurating a new program of selecting titles. The Modern Library continues to provide the world's best \\

& & books, at the best prices. Tracy Kidder has written a new Introduction to this Modern Library edition.\\ \cline{2-3}

 % & ${\cal{M}} $ & \{"author":"TRACY KIDDER","publisher":"Modern Library"\}\\ \hline
& \multicolumn{1}{c}{\textbf{Actual Genre}:} & (Non-fiction, {Business \& Money, Computers \& Technology, History, Science \& Math })\\




\hline \hline
\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textcolor{blue}{\emph{(i)}} \textbf{9780803716988: Library Lil; Author: Suzanne Williams; Publisher: Dial Books}}\\
\hline 

\multirow{3}{*}{\includegraphics[width=0.04\linewidth, height=0.05\linewidth]{figs/heatmap/9.jpg}} & \multirow{2}{*}{\textbf{Blurb}:} & A formidable librarian makes readers not only out of the once resistant residents of her small town, but out of a tough-talking, television-watching motorcycle gang as well. \\
& & \\
\cline{2-3}
% & ${\cal{M}}$ & \{"author":"Suzanne Williams","publisher":"Dial Books"\}\\

% \hline
& \multicolumn{1}{l}{\textbf{Actual Genre}:} & (Fiction, \{Arts \& Photography, {Childrens\textquoteright} Book, Humor \& Entertainment, Meta Text, Sci-Fi\})\\



\hline \hline
\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textcolor{blue}{\emph{(j)}} \textbf{9780130255792: Understanding Movies; Author: Louis D. Giannetti; Publisher: Prentice Hall}}\\
\hline 
\multirow{5}{*}{\includegraphics[width=0.04\linewidth, height=0.05\linewidth]{figs/heatmap/10.jpg}} & \multirow{4}{*}{\textbf{Blurb}:} & Designed to help movie watchers analyze films with precision and technical sophistication, this book focuses on formalism how the forms of the film (e.g., camera work, \\
& &  editing, photography, etc.) create meaning. It sheds light on how television and movies communicate, and the complex network of language systems they use. Chapter topics\\

& &    cover recent developments from all aspects of cinema, contemporary films, personalities in the field, photography, movement, editing, sound, acting, drama, story writing, and   \\ 

& & theory. For movie critics and fans alike.\\
\cline{2-3}

& \multicolumn{1}{l}{\textbf{Actual Genre}:} & (Non-fiction, \{Arts \& Photography, Press \& Media, Reference \& Language, Teen \& Young Adult\}) \\
\hline

\end{tabular}
\end{adjustbox}


\label{tab:heatmap_samples}

\end{table*}

==> tables/indistinguish_table.tex <==

\begin{table*}[hbt]
\centering
\caption{Example of misclassified data samples due to genre indistinguishability.}
\begin{adjustbox}{width=0.95\textwidth}
% \begin{adjustbox}{angle=90, height=1\textheight}
% \footnotesize
\begin{tabular}{c|ll}%p{0.9\textwidth}}
%

\hline \hline


\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textbf{\emph{(a)} 9780671501075: Dragon's Honor (Star Trek: The Next Generation, No. 38); Author: Kij Johnson; Publisher: Star Trek}}\\
\hline \hline
& \\ [\dimexpr-\normalbaselineskip+1.5pt]

\multirow{8}{*}{\includegraphics[width=0.08\linewidth]{figs/indistinguish_genre/3.jpg}} & \multirow{5}{*}{\textbf{Blurb}:} & Isolated for centuries, the exotic Dragon Empire is finally ready to join the United Federation of Planets. But first the emperor's eldest son must marry the only   \\
 &  & daughter of his oldest enemy, bringing to an end decades of civil war. Without the wedding, there can be no peace -- and no treaty with the Federation.As honored \\
 & & guests of  the  Dragon Empire, Captain Picard and the crew of the "Starship Enterprise" TM must ensure that the royal wedding occurs on schedule, despite the  \\
 & & Empire's complicated and difficult codes of honor. And Dr. Beverly Crusher finds her loyalties torn when she wins the confidence of the unusually reluctant  \\
 & & bride-to-be.  More than just of the Federation. Picard a treaty is at stake, for a vicious race of alien conquerors will stop at nothing, from assassination to invasion,\\
 & &   to keep the Empire out must use all  his skills to save the Empire, and preserve the Dragon's Honor.\\
\cline{2-3}
% & ${\cal{M}}$ & \{"author":"Kij Johnson","publisher":"Star Trek"\}\\ \hline

& \multicolumn{1}{l}{\textbf{Actual Genre}:} & (Fiction, \{Press \& Media, Sci-Fi\})\\ \cline{2-3} %\hline

& \multicolumn{1}{l}{\textbf{Predicted Genre}:} & (Fiction, \{Sci-Fi\})\\ 


\hline \hline


\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textbf{\emph{(b)} 9780380808175: T2: Rising Storm (T2); Author: S.M. Stirling; Publisher: HarperEntertainment}}\\
\hline \hline
& \\ [\dimexpr-\normalbaselineskip+1.5pt]

\multirow{6}{*}{\includegraphics[width=0.08\linewidth]{figs/indistinguish_genre/5.jpg}} & \multirow{4}{*}{\textbf{Blurb}:} & \multirow{4}{*}{The war is far from over ... Those who fight for the future face the ultimate challenge ... As the electronic brain behind humanity's destruction comes alive.} \\
 &  & \\
  &  & \\
  &  & \\
\cline{2-3}
% & ${\cal{M}}$ & \{"author":"S.M. Stirling","publisher":"HarperEntertainment"\}\\ \hline

& \multicolumn{1}{l}{\textbf{Actual Genre}:} & (Fiction, \{Mystery \& Thriller \& Suspense \& Horror, Press \& Media, Sci-Fi\})\\ \cline{2-3} %\hline

& \multicolumn{1}{l}{\textbf{Predicted Genre}:} & (Fiction, \{Humanities, Mystery \& Thriller \& Suspense \& Horror, Medical, Sci-Fi\})\\ 



\hline \hline


\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textbf{\emph{(c)} 9781569711293: Star Wars: Battle of the Bounty Hunters; Author: Ryder Windham; Publisher: Dark Horse Comics}}\\
\hline \hline
& \\ [\dimexpr-\normalbaselineskip+1.5pt]

\multirow{6}{*}{\includegraphics[width=0.08\linewidth]{figs/indistinguish_genre/1.jpg}} & \multirow{4}{*}{\textbf{Blurb}:} &  \\
 & & Battle of the Bounty Hunters was a pop-up comic and part of the Star Wars: Shadows of the Empire multimedia campaign. It showed the space battle between \\
 &  &  Boba Fett and IG-88D.\\
 &  &  \\
\cline{2-3}
% & ${\cal{M}}$ & \{"author":"Ryder Windham","publisher":"Dark Horse Comics"\}\\ \hline

& \multicolumn{1}{l}{\textbf{Actual Genre}:} & (Fiction, \{Comics \& Graphic, Press \& Media, Sci-Fi\})\\ \cline{2-3} %\hline

& \multicolumn{1}{l}{\textbf{Predicted Genre}:} & (Fiction, \{Comics \& Graphic, Sci-Fi\})\\ 

\hline \hline

\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textbf{\emph{(d)} 9780425051849: 
 Dance of the Tiger; Author: Bjorn Kurten; Publisher: Berkley Publishing Group}}\\
\hline \hline
& \\ [\dimexpr-\normalbaselineskip+1.5pt]


\multirow{6}{*}{\includegraphics[width=0.08\linewidth]{figs/indistinguish_genre/7.jpg}} & \multirow{4}{*}{\textbf{Blurb}:} & \multirow{2}{*}{Björn Kurtén's compelling novel gives the reader a detailed picture of life 35,000 years ago in Western Europe. One of the world's leading scholars of Ice Age}   \\
& & \multirow{2}{*}{fauna, Kurtén fuses extraordinary knowledge and imagination in this vivid evocation of our deepest past. This novel illuminates the lives of the humans who left}    \\ 
& & \multirow{2}{*}{us magnificent paintings in the caves of France and Spain.} \\ 
& & \\ \cline{2-3}

% & ${\cal{M}}$ & \{"author":"Bjorn Kurten","publisher":"Berkley Publishing Group"\}\\ \hline
& \multicolumn{1}{l}{\textbf{Actual Genre}:} & (Fiction, \{History, Humanities, Sci-Fi\})\\ \cline{2-3} %\hline

& \multicolumn{1}{l}{\textbf{Predicted Genre}:} & (Fiction, \{Environment \& Plant, History, Literature, Travel, Sci-Fi\})\\


\hline \hline

\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textbf{\emph{(e)} 9780789425225: Voices in the Park; Author: Anthony Browne; Publisher: Dorling Kindersley Publishing}}\\
\hline \hline
& \\ [\dimexpr-\normalbaselineskip+1.5pt]

\multirow{5}{*}{\includegraphics[width=0.08\linewidth]{figs/indistinguish_genre/9.jpg}} & \multirow{3}{*}{\textbf{Blurb}:} & \multirow{2}{*}{Four people enter a park and through their eyes young readers see different visions, from the bossy woman and the sad man to the lonely boy and the warm young} \\

 &  &  \multirow{2}{*}{girl, moving from one voice to another and shifting landscapes and seasons.} \\

  &  & \\

 
\cline{2-3}
% & ${\cal{M}}$ & \{"author":"Anthony Browne","publisher":"Dorling Kindersley Publishing"\}\\ \hline
& \multicolumn{1}{l}{\textbf{Actual Genre}:} & (Fiction, \{Animals \& Wildlife \& Pets, Arts \& Photography, {Childrens\textquoteright} Book, Family \& Parenting \& Relationships, Teen \& Young Adult\})\\ \cline{2-3} %\hline

& \multicolumn{1}{l}{\textbf{Predicted Genre}:} & (Fiction, \{Arts \& Photography, {Childrens\textquoteright} Book, Family \& Parenting \& Relationships, Teen \& Young Adult\})\\ %\hline

\hline \hline

\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textbf{\emph{(f)} 9780894712661: The Classic Tale of Velveteen Rabbit or How Toys Become Real; Author: Margery Williams; Publisher: Running Press}}\\
\hline \hline
& \\ [\dimexpr-\normalbaselineskip+1.5pt]


\multirow{5}{*}{\includegraphics[width=0.08\linewidth]{figs/indistinguish_genre/11.png}} & \multirow{3}{*}{\textbf{Blurb}:} & \multirow{2}{*}{A beautiful large-format edition of this timeless children's tale, replete with enchanting full-color illustrations. A charming fable with the moral that love can make} \\
& & \multirow{2}{*}{all things real and beautiful. 10" x 13".}\\ 
& & \\ \cline{2-3}

% & ${\cal{M}}$ & \{"author":"Margery Williams","publisher":"Courage Books"\}\\ \hline
& \multicolumn{1}{l}{\textbf{Actual Genre}:} & (Fiction, \{Animals \& Wildlife \& Pets, Arts \& Photography, {Childrens\textquoteright} Book, Literature, Sci-Fi, Teen \& Young Adult\})\\ \cline{2-3} %\hline

& \multicolumn{1}{l}{\textbf{Predicted Genre}:} & (Fiction, \{Arts \& Photography, {Childrens\textquoteright} Book, Literature, Mythology \& Religion \& Spirituality, Teen \& Young Adult, Sci-Fi\})\\
% \hline

\hline \hline

\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textbf{\emph{(g)} 9780440436836: Homesick: My Own Story; Author: Jean Fritz; Publisher: Yearling Books}}\\
\hline \hline
& \\ [\dimexpr-\normalbaselineskip+1.5pt]

\multirow{8}{*}{\includegraphics[width=0.08\linewidth]{figs/indistinguish_genre/18.jpg}} & \multirow{6}{*}{\textbf{Blurb}:} & Jean Fritz was born in China and lived there until 1927, when she was twelve. Young Jean had spent her entire life in China, but her parents' memories of home  \\
 &  & and letters from relatives in  Pennsylvania made her feel that she was American--and homesick for a place she'd never seen!Family photographs and illustrations   \\
 & &  by Margot Tomes show us the real people behind Jean's vivid and unforgettable stories--memories of picnics on the Great Wall, pranks, holidays in the foreign \\
 & &  compound, rebellious moments at her British school. close ties to Chinese friends, and how it felt to be called a "foreign devil" and spat upon in the streets of \\
 & &  a turbulent China on the eve of revolution. When her family embarks upon its long journey home, Jean is thrilled, but she When she arrives in America at last,  \\
  & & will she fit in after growing up on "the wrong side of the world?" \\
 
\cline{2-3}
% & ${\cal{M}}$ & \{"author":"Jean Fritz","publisher":"Yearling Books"\}\\ \hline
& \multicolumn{1}{l}{\textbf{Actual Genre}:} & (Non-fiction, \{Biographies \& Memoir, {Childrens\textquoteright} Book, History, Teen \& Young Adult\})\\ \cline{2-3} %\hline

& \multicolumn{1}{l}{\textbf{Predicted Genre}:} & (Non-fiction, \{{Childrens\textquoteright} Book, History, Biographies \& Memoir\})\\ %\hline

\hline \hline

\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textbf{\emph{(h)} 9780345291363: Elephant Man; Author: Christine Sparks; Publisher: Ballantine Books}}\\
\hline \hline
& \\ [\dimexpr-\normalbaselineskip+1.5pt]

\multirow{7}{*}{\includegraphics[width=0.08\linewidth]{figs/indistinguish_genre/19.jpg}} & \multirow{5}{*}{\textbf{Blurb}:} &  \\
& & John Merrick had lived for more than twenty years imprisoned in a body that condemned him to a miserable life in the workhouse and to humiliation as a circus   \\
 &  & sideshow freak. But beneath  that tragic exterior, within that enormous and deformed head, thrived the soul of a poet, the heart of a dreamer, the longings of a    \\
 & &  man. Based on the extraordinary motion picture that captured the heart of America.\\
  & & \\
 
\cline{2-3}
% & ${\cal{M}}$ & \{"author":"Christine Sparks","publisher":"Ballantine Books"\}\\ \hline
& \multicolumn{1}{l}{\textbf{Actual Genre}:} & (Non-fiction, \{Biographies \& Memoir, History, Literature, Teen \& Young Adult\})\\ \cline{2-3} %\hline

& \multicolumn{1}{l}{\textbf{Predicted Genre}:} & (Non-fiction, \{History, Literature, Biographies \& Memoir\})\\ \hline



\end{tabular}
\end{adjustbox}


\label{tab:indistinguish_sample}

\end{table*}

==> tables/level_1_kg.tex <==
\begin{table}[]
\centering
\caption{Binary classification (fiction/non-fiction) performance of knowledge graph models on metadata}
\begin{adjustbox}{width=0.40\textwidth} 
\begin{tabular}{l|c|c|c|c}
\hline
\textbf{Model} & \textbf{$\cal{P}$} & \textbf{$\cal{R}$} & \textbf{${\cal{FM}}$} & \textbf{${\cal{A}}$} \\ \hline
TransR & \textbf{81.64}& 69.29 & 74.96 & 68.91 \\ \hline
TransH & 77.42& 81.48 & 79.40& 71.61 \\ \hline
TransD & 78.17& 81.79 & \textbf{79.94} & \textbf{72.44} \\ \hline
ComplEx& 76.72& 79.32 & 78.00& 69.95 \\ \hline
SimplE & 74.75& 81.79 & 78.11 & 69.22 \\ \hline
Analogy& 76.75& 79.48 & 78.09 & 70.05 \\ \hline
DistMult & 74.72& \textbf{82.56} & 78.45 & 69.53 \\ \hline
\end{tabular}
\end{adjustbox}
\label{tab:level_1_kg}
\end{table}

==> tables/level_1_ocr.tex <==
\begin{table}[]
\centering
\caption{Binary classification (fiction/non-fiction) performance of textual models on ocr text}
\begin{adjustbox}{width=0.40\textwidth} 
\begin{tabular}{l|c|c|c|c}
\hline
\textbf{Model} & \textbf{$\cal{P}$} & \textbf{$\cal{R}$} & \textbf{${\cal{FM}}$} & \textbf{${\cal{A}}$} \\ \hline
Distilbert & 91.64& \textbf{94.75} & 93.17 & 90.67 \\ \hline
RoBERTa& 92.27& 90.28 & 91.26 & 88.39 \\ \hline
BERT & 94.22& 91.36 & 92.77 & 90.38 \\ \hline
GPT-2& 75.65& 75.77 & 75.71 & 67.36 \\ \hline
CLIP & 89.68& 93.83 & 91.70 & 88.60\\ \hline
BLIP & 90.74& 84.72 & 87.63 & 83.94 \\ \hline
XLNet& \textbf{94.28}& 92.42 & \textbf{93.34} & \textbf{91.10} \\ \hline
\end{tabular}
\end{adjustbox}
\label{tab:level_1_ocr}
\end{table}

==> tables/misclassification_fiction.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%% Version-1 Uncleaned
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table*}[]
% \centering
% \caption{Fiction genre indistinguishability analysis}


% % \begin{adjustbox}{angle=90, height=0.87\textheight}
% \begin{adjustbox}{width=1\textwidth} 
% \begin{tabular}{cc|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
% \hline
% & Class ID $\downarrow\rightarrow$  & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & 28 & 29 \\

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Sample Count
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \hline \hline
% \multicolumn{31}{c}{(a) \textbf{Sample Count}}\\
% \hline \hline

%  & 1 & 1002 & 539 & 0 & 817 & 23 & 0 & 153 & 0 & 206 & 143 & 0 & 102 & 41 & 38 & 190 & 362 & 38 & 45 & 158 & 52 & 0 & 0 & 16 & 33 & 27 & 0 & 248 & 0 & 304 \\
%  & 2 & 539 & 2024 & 12 & 1279 & 32 & 68 & 308 & 44 & 206 & 319 & 24 & 141 & 129 & 54 & 435 & 716 & 46 & 81 & 204 & 137 & 23 & 102 & 154 & 44 & 71 & 53 & 327 & 39 & 882 \\
%  & 3 & 0 & 12 & 510 & 0 & 28 & 18 & 0 & 0 & 0 & 0 & 0 & 0 & 154 & 109 & 44 & 160 & 0 & 0 & 213 & 30 & 14 & 0 & 0 & 0 & 106 & 0 & 0 & 14 & 69 \\
%  & 4 & 817 & 1279 & 0 & 2575 & 104 & 69 & 291 & 44 & 262 & 387 & 0 & 174 & 273 & 72 & 449 & 997 & 70 & 109 & 484 & 242 & 14 & 51 & 74 & 25 & 83 & 189 & 979 & 19 & 876 \\
%  & 5 & 23 & 32 & 28 & 104 & 643 & 19 & 9 & 0 & 0 & 0 & 0 & 0 & 62 & 32 & 270 & 32 & 0 & 0 & 137 & 0 & 9 & 19 & 69 & 17 & 0 & 19 & 56 & 0 & 299 \\
%  & 6 & 0 & 68 & 18 & 69 & 19 & 473 & 0 & 0 & 0 & 0 & 0 & 0 & 39 & 18 & 54 & 137 & 0 & 0 & 154 & 0 & 0 & 19 & 16 & 18 & 0 & 179 & 16 & 36 & 419 \\
%  & 7 & 153 & 308 & 0 & 291 & 9 & 0 & 646 & 0 & 16 & 62 & 38 & 102 & 24 & 40 & 191 & 306 & 16 & 0 & 133 & 16 & 8 & 0 & 92 & 17 & 0 & 0 & 52 & 32 & 103 \\
%  & 8 & 0 & 44 & 0 & 44 & 0 & 0 & 0 & 408 & 0 & 0 & 77 & 0 & 103 & 0 & 0 & 191 & 0 & 0 & 268 & 44 & 0 & 52 & 0 & 52 & 0 & 0 & 52 & 0 & 0 \\
%  & 9 & 206 & 206 & 0 & 262 & 0 & 0 & 16 & 0 & 713 & 40 & 26 & 0 & 141 & 104 & 40 & 441 & 0 & 0 & 158 & 84 & 0 & 0 & 36 & 48 & 0 & 50 & 76 & 25 & 184 \\
%  & 10 & 143 & 319 & 0 & 387 & 0 & 0 & 62 & 0 & 40 & 638 & 80 & 48 & 130 & 0 & 103 & 371 & 31 & 0 & 20 & 48 & 0 & 0 & 97 & 0 & 36 & 0 & 94 & 8 & 28 \\
%  & 11 & 0 & 24 & 0 & 0 & 0 & 0 & 38 & 77 & 26 & 80 & 1128 & 96 & 254 & 139 & 99 & 614 & 89 & 54 & 256 & 151 & 0 & 9 & 376 & 0 & 153 & 0 & 18 & 66 & 159 \\
%  & 12 & 102 & 141 & 0 & 174 & 0 & 0 & 102 & 0 & 0 & 48 & 96 & 566 & 30 & 200 & 79 & 365 & 257 & 0 & 84 & 21 & 0 & 0 & 9 & 0 & 0 & 0 & 142 & 0 & 76 \\
%  & 13 & 41 & 129 & 154 & 273 & 62 & 39 & 24 & 103 & 141 & 130 & 254 & 30 & 2473 & 138 & 70 & 985 & 108 & 155 & 650 & 382 & 73 & 20 & 574 & 77 & 187 & 65 & 400 & 174 & 506 \\
%  & 14 & 38 & 54 & 109 & 72 & 32 & 18 & 40 & 0 & 104 & 0 & 139 & 200 & 138 & 1169 & 85 & 693 & 226 & 40 & 256 & 287 & 0 & 34 & 97 & 8 & 229 & 26 & 146 & 86 & 339 \\
%  & 15 & 190 & 435 & 44 & 449 & 270 & 54 & 191 & 0 & 40 & 103 & 99 & 79 & 70 & 85 & 1595 & 604 & 25 & 172 & 271 & 38 & 40 & 42 & 100 & 19 & 34 & 40 & 159 & 83 & 454 \\
%  & 16 & 362 & 716 & 160 & 997 & 32 & 137 & 306 & 191 & 441 & 371 & 614 & 365 & 985 & 693 & 604 & 4730 & 378 & 218 & 1044 & 496 & 67 & 216 & 803 & 219 & 277 & 88 & 899 & 425 & 1175 \\
%  & 17 & 158 & 204 & 213 & 484 & 137 & 154 & 133 & 268 & 158 & 20 & 256 & 84 & 650 & 256 & 271 & 1044 & 200 & 214 & 3371 & 258 & 168 & 0 & 379 & 158 & 90 & 236 & 471 & 242 & 1184 \\
%  & 18 & 38 & 46 & 0 & 70 & 0 & 0 & 16 & 0 & 0 & 31 & 89 & 257 & 108 & 226 & 25 & 378 & 752 & 0 & 200 & 29 & 46 & 0 & 117 & 24 & 0 & 8 & 114 & 0 & 144 \\
%  & 19 & 45 & 81 & 0 & 109 & 0 & 0 & 0 & 0 & 0 & 0 & 54 & 0 & 155 & 40 & 172 & 218 & 0 & 598 & 214 & 29 & 0 & 64 & 74 & 16 & 0 & 0 & 85 & 0 & 182 \\
%  & 20 & 52 & 137 & 30 & 242 & 0 & 0 & 16 & 44 & 84 & 48 & 151 & 21 & 382 & 287 & 38 & 496 & 29 & 29 & 258 & 1517 & 0 & 73 & 352 & 18 & 615 & 0 & 171 & 56 & 427 \\
%  & 21 & 0 & 23 & 14 & 14 & 9 & 0 & 8 & 0 & 0 & 0 & 0 & 0 & 73 & 0 & 40 & 67 & 46 & 0 & 168 & 0 & 396 & 23 & 0 & 16 & 0 & 0 & 0 & 14 & 264 \\
%  & 22 & 0 & 102 & 0 & 51 & 19 & 19 & 0 & 52 & 0 & 0 & 9 & 0 & 20 & 34 & 42 & 216 & 0 & 64 & 0 & 73 & 23 & 560 & 0 & 118 & 0 & 63 & 76 & 11 & 379 \\
%  & 23 & 16 & 154 & 0 & 74 & 69 & 16 & 92 & 0 & 36 & 97 & 376 & 9 & 574 & 97 & 100 & 803 & 117 & 74 & 379 & 352 & 0 & 0 & 1778 & 49 & 193 & 12 & 247 & 67 & 423 \\
%  & 24 & 33 & 44 & 0 & 25 & 17 & 18 & 17 & 52 & 48 & 0 & 0 & 0 & 77 & 8 & 19 & 219 & 24 & 16 & 158 & 18 & 16 & 118 & 49 & 580 & 0 & 0 & 92 & 0 & 281 \\
%  & 25 & 27 & 71 & 106 & 83 & 0 & 0 & 0 & 0 & 0 & 36 & 153 & 0 & 187 & 229 & 34 & 277 & 0 & 0 & 90 & 615 & 0 & 0 & 193 & 0 & 799 & 0 & 51 & 45 & 81 \\
%  & 26 & 0 & 53 & 0 & 189 & 19 & 179 & 0 & 0 & 50 & 0 & 0 & 0 & 65 & 26 & 40 & 88 & 8 & 0 & 236 & 0 & 0 & 63 & 12 & 0 & 0 & 657 & 114 & 0 & 366 \\
%  & 27 & 248 & 327 & 0 & 979 & 56 & 16 & 52 & 52 & 76 & 94 & 18 & 142 & 400 & 146 & 159 & 899 & 114 & 85 & 471 & 171 & 0 & 76 & 247 & 92 & 51 & 114 & 1973 & 0 & 766 \\
%  & 28 & 0 & 39 & 14 & 19 & 0 & 36 & 32 & 0 & 25 & 8 & 66 & 0 & 174 & 86 & 83 & 425 & 0 & 0 & 242 & 56 & 14 & 11 & 67 & 0 & 45 & 0 & 0 & 603 & 94 \\
%  & 29 & 304 & 882 & 69 & 876 & 299 & 419 & 103 & 0 & 184 & 28 & 159 & 76 & 506 & 339 & 454 & 1175 & 144 & 182 & 1184 & 427 & 264 & 379 & 423 & 281 & 81 & 366 & 766 & 94 & 3980 \\

 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Cooccurrence
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \hline \hline
% \multicolumn{31}{c}{(b) \textbf{Cooccurrence}}\\
% \hline \hline

%  & 1 & 1.00 & 0.27 & 0.00 & 0.32 & 0.04 & 0.00 & 0.24 & 0.00 & 0.29 & 0.22 & 0.00 & 0.18 & 0.02 & 0.03 & 0.12 & 0.08 & 0.05 & 0.08 & 0.05 & 0.03 & 0.00 & 0.00 & 0.01 & 0.06 & 0.03 & 0.00 & 0.13 & 0.00 & 0.08 \\
%  & 2 & 0.54 & 1.00 & 0.02 & 0.50 & 0.05 & 0.14 & 0.48 & 0.11 & 0.29 & 0.50 & 0.02 & 0.25 & 0.05 & 0.05 & 0.27 & 0.15 & 0.06 & 0.14 & 0.06 & 0.09 & 0.06 & 0.18 & 0.09 & 0.08 & 0.09 & 0.08 & 0.17 & 0.06 & 0.22 \\
%  & 3 & 0.00 & 0.01 & 1.00 & 0.00 & 0.04 & 0.04 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.06 & 0.09 & 0.03 & 0.03 & 0.00 & 0.00 & 0.06 & 0.02 & 0.04 & 0.00 & 0.00 & 0.00 & 0.13 & 0.00 & 0.00 & 0.02 & 0.02 \\
%  & 4 & 0.82 & 0.63 & 0.00 & 1.00 & 0.16 & 0.15 & 0.45 & 0.11 & 0.37 & 0.61 & 0.00 & 0.31 & 0.11 & 0.06 & 0.28 & 0.21 & 0.09 & 0.18 & 0.14 & 0.16 & 0.04 & 0.09 & 0.04 & 0.04 & 0.10 & 0.29 & 0.50 & 0.03 & 0.22 \\
%  & 5 & 0.02 & 0.02 & 0.05 & 0.04 & 1.00 & 0.04 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.03 & 0.03 & 0.17 & 0.01 & 0.00 & 0.00 & 0.04 & 0.00 & 0.02 & 0.03 & 0.04 & 0.03 & 0.00 & 0.03 & 0.03 & 0.00 & 0.08 \\
%  & 6 & 0.00 & 0.03 & 0.04 & 0.03 & 0.03 & 1.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.02 & 0.02 & 0.03 & 0.03 & 0.00 & 0.00 & 0.05 & 0.00 & 0.00 & 0.03 & 0.01 & 0.03 & 0.00 & 0.27 & 0.01 & 0.06 & 0.11 \\
%  & 7 & 0.15 & 0.15 & 0.00 & 0.11 & 0.01 & 0.00 & 1.00 & 0.00 & 0.02 & 0.10 & 0.03 & 0.18 & 0.01 & 0.03 & 0.12 & 0.06 & 0.02 & 0.00 & 0.04 & 0.01 & 0.02 & 0.00 & 0.05 & 0.03 & 0.00 & 0.00 & 0.03 & 0.05 & 0.03 \\
%  & 8 & 0.00 & 0.02 & 0.00 & 0.02 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.07 & 0.00 & 0.04 & 0.00 & 0.00 & 0.04 & 0.00 & 0.00 & 0.08 & 0.03 & 0.00 & 0.09 & 0.00 & 0.09 & 0.00 & 0.00 & 0.03 & 0.00 & 0.00 \\
%  & 9 & 0.21 & 0.10 & 0.00 & 0.10 & 0.00 & 0.00 & 0.02 & 0.00 & 1.00 & 0.06 & 0.02 & 0.00 & 0.06 & 0.09 & 0.03 & 0.09 & 0.00 & 0.00 & 0.05 & 0.06 & 0.00 & 0.00 & 0.02 & 0.08 & 0.00 & 0.08 & 0.04 & 0.04 & 0.05 \\
%  & 10 & 0.14 & 0.16 & 0.00 & 0.15 & 0.00 & 0.00 & 0.10 & 0.00 & 0.06 & 1.00 & 0.07 & 0.08 & 0.05 & 0.00 & 0.06 & 0.08 & 0.04 & 0.00 & 0.01 & 0.03 & 0.00 & 0.00 & 0.05 & 0.00 & 0.05 & 0.00 & 0.05 & 0.01 & 0.01 \\
%  & 11 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.06 & 0.19 & 0.04 & 0.13 & 1.00 & 0.17 & 0.10 & 0.12 & 0.06 & 0.13 & 0.12 & 0.09 & 0.08 & 0.10 & 0.00 & 0.02 & 0.21 & 0.00 & 0.19 & 0.00 & 0.01 & 0.11 & 0.04 \\
%  & 12 & 0.10 & 0.07 & 0.00 & 0.07 & 0.00 & 0.00 & 0.16 & 0.00 & 0.00 & 0.08 & 0.09 & 1.00 & 0.01 & 0.17 & 0.05 & 0.08 & 0.34 & 0.00 & 0.02 & 0.01 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.07 & 0.00 & 0.02 \\
%  & 13 & 0.04 & 0.06 & 0.30 & 0.11 & 0.10 & 0.08 & 0.04 & 0.25 & 0.20 & 0.20 & 0.23 & 0.05 & 1.00 & 0.12 & 0.04 & 0.21 & 0.14 & 0.26 & 0.19 & 0.25 & 0.18 & 0.04 & 0.32 & 0.13 & 0.23 & 0.10 & 0.20 & 0.29 & 0.13 \\
%  & 14 & 0.04 & 0.03 & 0.21 & 0.03 & 0.05 & 0.04 & 0.06 & 0.00 & 0.15 & 0.00 & 0.12 & 0.35 & 0.06 & 1.00 & 0.05 & 0.15 & 0.30 & 0.07 & 0.08 & 0.19 & 0.00 & 0.06 & 0.05 & 0.01 & 0.29 & 0.04 & 0.07 & 0.14 & 0.09 \\
%  & 15 & 0.19 & 0.21 & 0.09 & 0.17 & 0.42 & 0.11 & 0.30 & 0.00 & 0.06 & 0.16 & 0.09 & 0.14 & 0.03 & 0.07 & 1.00 & 0.13 & 0.03 & 0.29 & 0.08 & 0.03 & 0.10 & 0.08 & 0.06 & 0.03 & 0.04 & 0.06 & 0.08 & 0.14 & 0.11 \\
%  & 16 & 0.36 & 0.35 & 0.31 & 0.39 & 0.05 & 0.29 & 0.47 & 0.47 & 0.62 & 0.58 & 0.54 & 0.64 & 0.40 & 0.59 & 0.38 & 1.00 & 0.50 & 0.36 & 0.31 & 0.33 & 0.17 & 0.39 & 0.45 & 0.38 & 0.35 & 0.13 & 0.46 & 0.70 & 0.30 \\
%  & 17 & 0.16 & 0.10 & 0.42 & 0.19 & 0.21 & 0.33 & 0.21 & 0.66 & 0.22 & 0.03 & 0.23 & 0.15 & 0.26 & 0.22 & 0.17 & 0.22 & 0.27 & 0.36 & 1.00 & 0.17 & 0.42 & 0.00 & 0.21 & 0.27 & 0.11 & 0.36 & 0.24 & 0.40 & 0.30 \\
%  & 18 & 0.04 & 0.02 & 0.00 & 0.03 & 0.00 & 0.00 & 0.02 & 0.00 & 0.00 & 0.05 & 0.08 & 0.45 & 0.04 & 0.19 & 0.02 & 0.08 & 1.00 & 0.00 & 0.06 & 0.02 & 0.12 & 0.00 & 0.07 & 0.04 & 0.00 & 0.01 & 0.06 & 0.00 & 0.04 \\
%  & 19 & 0.04 & 0.04 & 0.00 & 0.04 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.05 & 0.00 & 0.06 & 0.03 & 0.11 & 0.05 & 0.00 & 1.00 & 0.06 & 0.02 & 0.00 & 0.11 & 0.04 & 0.03 & 0.00 & 0.00 & 0.04 & 0.00 & 0.05 \\
%  & 20 & 0.05 & 0.07 & 0.06 & 0.09 & 0.00 & 0.00 & 0.02 & 0.11 & 0.12 & 0.08 & 0.13 & 0.04 & 0.15 & 0.25 & 0.02 & 0.10 & 0.04 & 0.05 & 0.08 & 1.00 & 0.00 & 0.13 & 0.20 & 0.03 & 0.77 & 0.00 & 0.09 & 0.09 & 0.11 \\
%  & 21 & 0.00 & 0.01 & 0.03 & 0.01 & 0.01 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.03 & 0.00 & 0.03 & 0.01 & 0.06 & 0.00 & 0.05 & 0.00 & 1.00 & 0.04 & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 & 0.02 & 0.07 \\
%  & 22 & 0.00 & 0.05 & 0.00 & 0.02 & 0.03 & 0.04 & 0.00 & 0.13 & 0.00 & 0.00 & 0.01 & 0.00 & 0.01 & 0.03 & 0.03 & 0.05 & 0.00 & 0.11 & 0.00 & 0.05 & 0.06 & 1.00 & 0.00 & 0.20 & 0.00 & 0.10 & 0.04 & 0.02 & 0.10 \\
%  & 23 & 0.02 & 0.08 & 0.00 & 0.03 & 0.11 & 0.03 & 0.14 & 0.00 & 0.05 & 0.15 & 0.33 & 0.02 & 0.23 & 0.08 & 0.06 & 0.17 & 0.16 & 0.12 & 0.11 & 0.23 & 0.00 & 0.00 & 1.00 & 0.08 & 0.24 & 0.02 & 0.13 & 0.11 & 0.11 \\
%  & 24 & 0.03 & 0.02 & 0.00 & 0.01 & 0.03 & 0.04 & 0.03 & 0.13 & 0.07 & 0.00 & 0.00 & 0.00 & 0.03 & 0.01 & 0.01 & 0.05 & 0.03 & 0.03 & 0.05 & 0.01 & 0.04 & 0.21 & 0.03 & 1.00 & 0.00 & 0.00 & 0.05 & 0.00 & 0.07 \\
%  & 25 & 0.03 & 0.04 & 0.21 & 0.03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.06 & 0.14 & 0.00 & 0.08 & 0.20 & 0.02 & 0.06 & 0.00 & 0.00 & 0.03 & 0.41 & 0.00 & 0.00 & 0.11 & 0.00 & 1.00 & 0.00 & 0.03 & 0.07 & 0.02 \\
%  & 26 & 0.00 & 0.03 & 0.00 & 0.07 & 0.03 & 0.38 & 0.00 & 0.00 & 0.07 & 0.00 & 0.00 & 0.00 & 0.03 & 0.02 & 0.03 & 0.02 & 0.01 & 0.00 & 0.07 & 0.00 & 0.00 & 0.11 & 0.01 & 0.00 & 0.00 & 1.00 & 0.06 & 0.00 & 0.09 \\
%  & 27 & 0.25 & 0.16 & 0.00 & 0.38 & 0.09 & 0.03 & 0.08 & 0.13 & 0.11 & 0.15 & 0.02 & 0.25 & 0.16 & 0.12 & 0.10 & 0.19 & 0.15 & 0.14 & 0.14 & 0.11 & 0.00 & 0.14 & 0.14 & 0.16 & 0.06 & 0.17 & 1.00 & 0.00 & 0.19 \\
%  & 28 & 0.00 & 0.02 & 0.03 & 0.01 & 0.00 & 0.08 & 0.05 & 0.00 & 0.04 & 0.01 & 0.06 & 0.00 & 0.07 & 0.07 & 0.05 & 0.09 & 0.00 & 0.00 & 0.07 & 0.04 & 0.04 & 0.02 & 0.04 & 0.00 & 0.06 & 0.00 & 0.00 & 1.00 & 0.02 \\
%  & 29 & 0.30 & 0.44 & 0.14 & 0.34 & 0.47 & 0.89 & 0.16 & 0.00 & 0.26 & 0.04 & 0.14 & 0.13 & 0.20 & 0.29 & 0.28 & 0.25 & 0.19 & 0.30 & 0.35 & 0.28 & 0.67 & 0.68 & 0.24 & 0.48 & 0.10 & 0.56 & 0.39 & 0.16 & 1.00 \\


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Misprediction
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \hline \hline
% \multicolumn{31}{c}{(c) \textbf{Misprediction}}\\
% \hline \hline


%  \multirow{30}{*}{\rotatebox{90}{\underline{Predicted Class ID $\downarrow$}}} & 1 & 0.00 & 0.04 & 0.00 & 0.00 & 0.01 & 0.00 & 0.03 & 0.00 & 0.01 & 0.03 & 0.00 & 0.02 & 0.02 & 0.01 & 0.04 & 0.01 & 0.01 & 0.01 & 0.02 & 0.02 & 0.00 & 0.00 & 0.02 & 0.00 & 0.00 & 0.01 & 0.06 & 0.00 & 0.02 \\
%  & 2 & 0.18 & 0.00 & 0.02 & 0.03 & 0.13 & 0.00 & 0.09 & 0.00 & 0.04 & 0.12 & 0.03 & 0.04 & 0.06 & 0.07 & 0.09 & 0.06 & 0.01 & 0.04 & 0.07 & 0.06 & 0.09 & 0.04 & 0.07 & 0.05 & 0.06 & 0.06 & 0.08 & 0.03 & 0.04 \\
%  & 3 & 0.01 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\
%  & 4 & 0.64 & 0.19 & 0.02 & 0.00 & 0.06 & 0.00 & 0.09 & 0.00 & 0.03 & 0.18 & 0.01 & 0.04 & 0.05 & 0.03 & 0.08 & 0.06 & 0.01 & 0.01 & 0.08 & 0.07 & 0.02 & 0.00 & 0.05 & 0.02 & 0.02 & 0.07 & 0.13 & 0.01 & 0.06 \\
%  & 5 & 0.00 & 0.01 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.01 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.01 & 0.00 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.01 \\
%  & 6 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.01 & 0.02 & 0.03 & 0.00 & 0.00 & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 \\
%  & 7 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
%  & 8 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
%  & 9 & 0.02 & 0.01 & 0.00 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.01 & 0.03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.02 & 0.01 & 0.02 & 0.00 & 0.02 & 0.00 & 0.00 & 0.01 & 0.02 & 0.01 & 0.01 \\
%  & 10 & 0.03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.02 & 0.01 & 0.02 & 0.01 & 0.01 & 0.00 & 0.00 & 0.04 & 0.00 & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 & 0.03 & 0.00 & 0.00 \\
%  & 11 & 0.02 & 0.03 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.02 & 0.01 & 0.03 & 0.00 & 0.02 & 0.02 & 0.03 & 0.03 & 0.02 & 0.02 & 0.00 & 0.04 & 0.06 & 0.00 & 0.02 & 0.03 & 0.00 & 0.01 & 0.00 & 0.03 & 0.00 & 0.01 \\
%  & 12 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\
%  & 13 & 0.03 & 0.06 & 0.03 & 0.05 & 0.09 & 0.00 & 0.00 & 0.05 & 0.04 & 0.00 & 0.18 & 0.00 & 0.00 & 0.09 & 0.05 & 0.07 & 0.00 & 0.08 & 0.13 & 0.14 & 0.08 & 0.00 & 0.09 & 0.05 & 0.03 & 0.05 & 0.08 & 0.08 & 0.08 \\
%  & 14 & 0.02 & 0.02 & 0.04 & 0.01 & 0.03 & 0.00 & 0.01 & 0.00 & 0.00 & 0.01 & 0.04 & 0.02 & 0.01 & 0.00 & 0.02 & 0.02 & 0.03 & 0.00 & 0.03 & 0.02 & 0.07 & 0.00 & 0.03 & 0.01 & 0.01 & 0.04 & 0.03 & 0.02 & 0.02 \\
%  & 15 & 0.01 & 0.03 & 0.00 & 0.02 & 0.14 & 0.00 & 0.05 & 0.00 & 0.00 & 0.03 & 0.03 & 0.02 & 0.02 & 0.03 & 0.00 & 0.03 & 0.02 & 0.02 & 0.04 & 0.01 & 0.10 & 0.02 & 0.03 & 0.03 & 0.00 & 0.03 & 0.03 & 0.00 & 0.03 \\
%  & 16 & 0.16 & 0.11 & 0.10 & 0.10 & 0.16 & 0.00 & 0.08 & 0.07 & 0.08 & 0.21 & 0.23 & 0.05 & 0.15 & 0.51 & 0.19 & 0.00 & 0.04 & 0.13 & 0.17 & 0.17 & 0.15 & 0.08 & 0.17 & 0.23 & 0.08 & 0.06 & 0.26 & 0.26 & 0.10 \\
%  & 17 & 0.07 & 0.05 & 0.03 & 0.04 & 0.09 & 0.03 & 0.03 & 0.05 & 0.01 & 0.04 & 0.11 & 0.02 & 0.03 & 0.11 & 0.03 & 0.04 & 0.00 & 0.07 & 0.00 & 0.04 & 0.12 & 0.00 & 0.02 & 0.04 & 0.02 & 0.08 & 0.03 & 0.10 & 0.05 \\
%  & 18 & 0.00 & 0.01 & 0.02 & 0.00 & 0.01 & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 & 0.04 & 0.00 & 0.01 & 0.01 & 0.00 & 0.01 & 0.00 & 0.00 & 0.01 & 0.01 & 0.05 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.01 \\
%  & 19 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 \\
%  & 20 & 0.02 & 0.03 & 0.06 & 0.02 & 0.03 & 0.00 & 0.01 & 0.00 & 0.04 & 0.03 & 0.04 & 0.00 & 0.01 & 0.06 & 0.01 & 0.03 & 0.00 & 0.01 & 0.05 & 0.00 & 0.00 & 0.03 & 0.02 & 0.09 & 0.19 & 0.02 & 0.02 & 0.02 & 0.03 \\
%  & 21 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
%  & 22 & 0.00 & 0.00 & 0.00 & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.05 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.02 & 0.00 & 0.01 \\
%  & 23 & 0.02 & 0.04 & 0.00 & 0.03 & 0.03 & 0.00 & 0.00 & 0.00 & 0.03 & 0.03 & 0.15 & 0.00 & 0.07 & 0.07 & 0.06 & 0.05 & 0.02 & 0.05 & 0.07 & 0.11 & 0.00 & 0.00 & 0.00 & 0.09 & 0.01 & 0.01 & 0.06 & 0.02 & 0.04 \\
%  & 24 & 0.01 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.01 & 0.01 & 0.00 & 0.00 & 0.02 & 0.01 & 0.00 & 0.04 & 0.00 & 0.00 & 0.01 & 0.00 & 0.02 & 0.01 & 0.02 \\
%  & 25 & 0.00 & 0.00 & 0.07 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
%  & 26 & 0.01 & 0.01 & 0.00 & 0.01 & 0.03 & 0.03 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.01 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 \\
%  & 27 & 0.09 & 0.08 & 0.00 & 0.12 & 0.04 & 0.02 & 0.03 & 0.00 & 0.00 & 0.03 & 0.05 & 0.00 & 0.05 & 0.04 & 0.05 & 0.07 & 0.00 & 0.01 & 0.10 & 0.08 & 0.00 & 0.04 & 0.09 & 0.04 & 0.00 & 0.00 & 0.00 & 0.01 & 0.06 \\
%  & 28 & 0.01 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.03 & 0.01 & 0.00 & 0.00 & 0.01 & 0.02 & 0.02 & 0.00 & 0.02 & 0.00 & 0.00 & 0.02 & 0.02 & 0.00 & 0.00 & 0.01 \\
%  & 29 & 0.13 & 0.16 & 0.04 & 0.07 & 0.38 & 0.17 & 0.03 & 0.00 & 0.04 & 0.03 & 0.07 & 0.02 & 0.07 & 0.13 & 0.10 & 0.07 & 0.01 & 0.02 & 0.22 & 0.12 & 0.79 & 0.14 & 0.08 & 0.25 & 0.04 & 0.30 & 0.14 & 0.00 & 0.00 \\
%  & 30 & 0.01 & 0.00 & 0.00 & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.01 & 0.01 & 0.01 & 0.01 & 0.00 & 0.01 & 0.01 & 0.01 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.01 & 0.00 & 0.01 \\
% \hline
% \end{tabular}
% \end{adjustbox}

% \label{tab:misclassification_fiction}
% \end{table*}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Version-2 cleaned
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table*}[]
\centering
\caption{Fiction genre indistinguishability analysis}


% \begin{adjustbox}{angle=90, height=0.87\textheight}
\begin{adjustbox}{width=1\textwidth} 
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\hline
& Class ID $\downarrow\rightarrow$  & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & 28 & 29 \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Sample Count
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline \hline
\rowcolor[HTML]{D9D9D9}
\multicolumn{31}{c}{(a) \textbf{Sample Count}}\\
\hline \hline

 \multirow{29}{*}{\rotatebox{90}{Actual Class ID $\downarrow$}} & 1 & 1002 & 539 & 0 & 817 & 23 & 0 & 153 & 0 & 206 & 143 & 0 & 102 & 41 & 38 & 190 & 362 & 38 & 45 & 158 & 52 & 0 & 0 & 16 & 33 & 27 & 0 & 248 & 0 & 304 \\
 & 2 & 539 & 2024 & 12 & 1279 & 32 & 68 & 308 & 44 & 206 & 319 & 24 & 141 & 129 & 54 & 435 & 716 & 46 & 81 & 204 & 137 & 23 & 102 & 154 & 44 & 71 & 53 & 327 & 39 & 882 \\
 & 3 & 0 & 12 & 510 & 0 & 28 & 18 & 0 & 0 & 0 & 0 & 0 & 0 & 154 & 109 & 44 & 160 & 0 & 0 & 213 & 30 & 14 & 0 & 0 & 0 & 106 & 0 & 0 & 14 & 69 \\
 & 4 & 817 & 1279 & 0 & 2575 & 104 & 69 & 291 & 44 & 262 & 387 & 0 & 174 & 273 & 72 & 449 & 997 & 70 & 109 & 484 & 242 & 14 & 51 & 74 & 25 & 83 & 189 & 979 & 19 & 876 \\
 & 5 & 23 & 32 & 28 & 104 & 643 & 19 & 9 & 0 & 0 & 0 & 0 & 0 & 62 & 32 & 270 & 32 & 0 & 0 & 137 & 0 & 9 & 19 & 69 & 17 & 0 & 19 & 56 & 0 & 299 \\
 & 6 & 0 & 68 & 18 & 69 & 19 & 473 & 0 & 0 & 0 & 0 & 0 & 0 & 39 & 18 & 54 & 137 & 0 & 0 & 154 & 0 & 0 & 19 & 16 & 18 & 0 & 179 & 16 & 36 & 419 \\
 & 7 & 153 & 308 & 0 & 291 & 9 & 0 & 646 & 0 & 16 & 62 & 38 & 102 & 24 & 40 & 191 & 306 & 16 & 0 & 133 & 16 & 8 & 0 & 92 & 17 & 0 & 0 & 52 & 32 & 103 \\
 & 8 & 0 & 44 & 0 & 44 & 0 & 0 & 0 & 408 & 0 & 0 & 77 & 0 & 103 & 0 & 0 & 191 & 0 & 0 & 268 & 44 & 0 & 52 & 0 & 52 & 0 & 0 & 52 & 0 & 0 \\
 & 9 & 206 & 206 & 0 & 262 & 0 & 0 & 16 & 0 & 713 & 40 & 26 & 0 & 141 & 104 & 40 & 441 & 0 & 0 & 158 & 84 & 0 & 0 & 36 & 48 & 0 & 50 & 76 & 25 & 184 \\
 & 10 & 143 & 319 & 0 & 387 & 0 & 0 & 62 & 0 & 40 & 638 & 80 & 48 & 130 & 0 & 103 & 371 & 31 & 0 & 20 & 48 & 0 & 0 & 97 & 0 & 36 & 0 & 94 & 8 & 28 \\
 & 11 & 0 & 24 & 0 & 0 & 0 & 0 & 38 & 77 & 26 & 80 & 1128 & 96 & 254 & 139 & 99 & 614 & 89 & 54 & 256 & 151 & 0 & 9 & 376 & 0 & 153 & 0 & 18 & 66 & 159 \\
 & 12 & 102 & 141 & 0 & 174 & 0 & 0 & 102 & 0 & 0 & 48 & 96 & 566 & 30 & 200 & 79 & 365 & 257 & 0 & 84 & 21 & 0 & 0 & 9 & 0 & 0 & 0 & 142 & 0 & 76 \\
 & 13 & 41 & 129 & 154 & 273 & 62 & 39 & 24 & 103 & 141 & 130 & 254 & 30 & 2473 & 138 & 70 & 985 & 108 & 155 & 650 & 382 & 73 & 20 & 574 & 77 & 187 & 65 & 400 & 174 & 506 \\
 & 14 & 38 & 54 & 109 & 72 & 32 & 18 & 40 & 0 & 104 & 0 & 139 & 200 & 138 & 1169 & 85 & 693 & 226 & 40 & 256 & 287 & 0 & 34 & 97 & 8 & 229 & 26 & 146 & 86 & 339 \\
 & 15 & 190 & 435 & 44 & 449 & 270 & 54 & 191 & 0 & 40 & 103 & 99 & 79 & 70 & 85 & 1595 & 604 & 25 & 172 & 271 & 38 & 40 & 42 & 100 & 19 & 34 & 40 & 159 & 83 & 454 \\
 & 16 & 362 & 716 & 160 & 997 & 32 & 137 & 306 & 191 & 441 & 371 & 614 & 365 & 985 & 693 & 604 & 4730 & 378 & 218 & 1044 & 496 & 67 & 216 & 803 & 219 & 277 & 88 & 899 & 425 & 1175 \\
 & 17 & 158 & 204 & 213 & 484 & 137 & 154 & 133 & 268 & 158 & 20 & 256 & 84 & 650 & 256 & 271 & 1044 & 200 & 214 & 3371 & 258 & 168 & 0 & 379 & 158 & 90 & 236 & 471 & 242 & 1184 \\
 & 18 & 38 & 46 & 0 & 70 & 0 & 0 & 16 & 0 & 0 & 31 & 89 & 257 & 108 & 226 & 25 & 378 & 752 & 0 & 200 & 29 & 46 & 0 & 117 & 24 & 0 & 8 & 114 & 0 & 144 \\
 & 19 & 45 & 81 & 0 & 109 & 0 & 0 & 0 & 0 & 0 & 0 & 54 & 0 & 155 & 40 & 172 & 218 & 0 & 598 & 214 & 29 & 0 & 64 & 74 & 16 & 0 & 0 & 85 & 0 & 182 \\
 & 20 & 52 & 137 & 30 & 242 & 0 & 0 & 16 & 44 & 84 & 48 & 151 & 21 & 382 & 287 & 38 & 496 & 29 & 29 & 258 & 1517 & 0 & 73 & 352 & 18 & 615 & 0 & 171 & 56 & 427 \\
 & 21 & 0 & 23 & 14 & 14 & 9 & 0 & 8 & 0 & 0 & 0 & 0 & 0 & 73 & 0 & 40 & 67 & 46 & 0 & 168 & 0 & \textbf{396} & 23 & 0 & 16 & 0 & 0 & 0 & 14 & \textbf{264} \\
 & 22 & 0 & 102 & 0 & 51 & 19 & 19 & 0 & 52 & 0 & 0 & 9 & 0 & 20 & 34 & 42 & 216 & 0 & 64 & 0 & 73 & 23 & 560 & 0 & 118 & 0 & 63 & 76 & 11 & 379 \\
 & 23 & 16 & 154 & 0 & 74 & 69 & 16 & 92 & 0 & 36 & 97 & 376 & 9 & 574 & 97 & 100 & 803 & 117 & 74 & 379 & 352 & 0 & 0 & 1778 & 49 & 193 & 12 & 247 & 67 & 423 \\
 & 24 & 33 & 44 & 0 & 25 & 17 & 18 & 17 & 52 & 48 & 0 & 0 & 0 & 77 & 8 & 19 & 219 & 24 & 16 & 158 & 18 & 16 & 118 & 49 & 580 & 0 & 0 & 92 & 0 & 281 \\
 & 25 & 27 & 71 & 106 & 83 & 0 & 0 & 0 & 0 & 0 & 36 & 153 & 0 & 187 & 229 & 34 & 277 & 0 & 0 & 90 & 615 & 0 & 0 & 193 & 0 & 799 & 0 & 51 & 45 & 81 \\
 & 26 & 0 & 53 & 0 & 189 & 19 & 179 & 0 & 0 & 50 & 0 & 0 & 0 & 65 & 26 & 40 & 88 & 8 & 0 & 236 & 0 & 0 & 63 & 12 & 0 & 0 & 657 & 114 & 0 & 366 \\
 & 27 & 248 & 327 & 0 & 979 & 56 & 16 & 52 & 52 & 76 & 94 & 18 & 142 & 400 & 146 & 159 & 899 & 114 & 85 & 471 & 171 & 0 & 76 & 247 & 92 & 51 & 114 & 1973 & 0 & 766 \\
 & 28 & 0 & 39 & 14 & 19 & 0 & 36 & 32 & 0 & 25 & 8 & 66 & 0 & 174 & 86 & 83 & 425 & 0 & 0 & 242 & 56 & 14 & 11 & 67 & 0 & 45 & 0 & 0 & 603 & 94 \\
 & 29 & 304 & 882 & 69 & 876 & 299 & 419 & 103 & 0 & 184 & 28 & 159 & 76 & 506 & 339 & 454 & 1175 & 144 & 182 & 1184 & 427 & \textbf{264} & 379 & 423 & 281 & 81 & 366 & 766 & 94 & \textbf{3980} \\

 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Cooccurrence
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline \hline
\rowcolor[HTML]{D9D9D9}
\multicolumn{31}{c}{(b) \textbf{Cooccurrence}}\\
\hline \hline

 \multirow{29}{*}{\rotatebox{90}{Actual Class ID $\downarrow$}} & 1 & 1 & 0.27 & 0 & 0.32 & 0.04 & 0 & 0.24 & 0 & 0.29 & 0.22 & 0 & 0.18 & 0.02 & 0.03 & 0.12 & 0.08 & 0.05 & 0.08 & 0.05 & 0.03 & 0 & 0 & 0.01 & 0.06 & 0.03 & 0 & 0.13 & 0 & 0.08 \\
 & 2 & 0.54 & 1 & 0.02 & 0.50 & 0.05 & 0.14 & 0.48 & 0.11 & 0.29 & 0.50 & 0.02 & 0.25 & 0.05 & 0.05 & 0.27 & 0.15 & 0.06 & 0.14 & 0.06 & 0.09 & 0.06 & 0.18 & 0.09 & 0.08 & 0.09 & 0.08 & 0.17 & 0.06 & 0.22 \\
 & 3 & 0 & 0.01 & 1 & 0 & 0.04 & 0.04 & 0 & 0 & 0 & 0 & 0 & 0 & 0.06 & 0.09 & 0.03 & 0.03 & 0 & 0 & 0.06 & 0.02 & 0.04 & 0 & 0 & 0 & 0.13 & 0 & 0 & 0.02 & 0.02 \\
 & 4 & 0.82 & 0.63 & 0 & 1 & 0.16 & 0.15 & 0.45 & 0.11 & 0.37 & 0.61 & 0 & 0.31 & 0.11 & 0.06 & 0.28 & 0.21 & 0.09 & 0.18 & 0.14 & 0.16 & 0.04 & 0.09 & 0.04 & 0.04 & 0.10 & 0.29 & 0.50 & 0.03 & 0.22 \\
 & 5 & 0.02 & 0.02 & 0.05 & 0.04 & 1 & 0.04 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0.03 & 0.03 & 0.17 & 0.01 & 0 & 0 & 0.04 & 0 & 0.02 & 0.03 & 0.04 & 0.03 & 0 & 0.03 & 0.03 & 0 & 0.08 \\
 & 6 & 0 & 0.03 & 0.04 & 0.03 & 0.03 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0.02 & 0.02 & 0.03 & 0.03 & 0 & 0 & 0.05 & 0 & 0 & 0.03 & 0.01 & 0.03 & 0 & 0.27 & 0.01 & 0.06 & 0.11 \\
 & 7 & 0.15 & 0.15 & 0 & 0.11 & 0.01 & 0 & 1 & 0 & 0.02 & 0.10 & 0.03 & 0.18 & 0.01 & 0.03 & 0.12 & 0.06 & 0.02 & 0 & 0.04 & 0.01 & 0.02 & 0 & 0.05 & 0.03 & 0 & 0 & 0.03 & 0.05 & 0.03 \\
 & 8 & 0 & 0.02 & 0 & 0.02 & 0 & 0 & 0 & 1 & 0 & 0 & 0.07 & 0 & 0.04 & 0 & 0 & 0.04 & 0 & 0 & 0.08 & 0.03 & 0 & 0.09 & 0 & 0.09 & 0 & 0 & 0.03 & 0 & 0 \\
 & 9 & 0.21 & 0.10 & 0 & 0.10 & 0 & 0 & 0.02 & 0 & 1 & 0.06 & 0.02 & 0 & 0.06 & 0.09 & 0.03 & 0.09 & 0 & 0 & 0.05 & 0.06 & 0 & 0 & 0.02 & 0.08 & 0 & 0.08 & 0.04 & 0.04 & 0.05 \\
 & 10 & 0.14 & 0.16 & 0 & 0.15 & 0 & 0 & 0.10 & 0 & 0.06 & 1 & 0.07 & 0.08 & 0.05 & 0 & 0.06 & 0.08 & 0.04 & 0 & 0.01 & 0.03 & 0 & 0 & 0.05 & 0 & 0.05 & 0 & 0.05 & 0.01 & 0.01 \\
 & 11 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0.06 & 0.19 & 0.04 & 0.13 & 1 & 0.17 & 0.10 & 0.12 & 0.06 & 0.13 & 0.12 & 0.09 & 0.08 & 0.10 & 0 & 0.02 & 0.21 & 0 & 0.19 & 0 & 0.01 & 0.11 & 0.04 \\
 & 12 & 0.10 & 0.07 & 0 & 0.07 & 0 & 0 & 0.16 & 0 & 0 & 0.08 & 0.09 & 1 & 0.01 & 0.17 & 0.05 & 0.08 & 0.34 & 0 & 0.02 & 0.01 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0.07 & 0 & 0.02 \\
 & 13 & 0.04 & 0.06 & 0.30 & 0.11 & 0.10 & 0.08 & 0.04 & 0.25 & 0.20 & 0.20 & 0.23 & 0.05 & 1 & 0.12 & 0.04 & 0.21 & 0.14 & 0.26 & 0.19 & 0.25 & 0.18 & 0.04 & 0.32 & 0.13 & 0.23 & 0.10 & 0.20 & 0.29 & 0.13 \\
 & 14 & 0.04 & 0.03 & 0.21 & 0.03 & 0.05 & 0.04 & 0.06 & 0 & 0.15 & 0 & 0.12 & 0.35 & 0.06 & 1 & 0.05 & 0.15 & 0.30 & 0.07 & 0.08 & 0.19 & 0 & 0.06 & 0.05 & 0.01 & 0.29 & 0.04 & 0.07 & 0.14 & 0.09 \\
 & 15 & 0.19 & 0.21 & 0.09 & 0.17 & 0.42 & 0.11 & 0.30 & 0 & 0.06 & 0.16 & 0.09 & 0.14 & 0.03 & 0.07 & 1 & 0.13 & 0.03 & 0.29 & 0.08 & 0.03 & 0.10 & 0.08 & 0.06 & 0.03 & 0.04 & 0.06 & 0.08 & 0.14 & 0.11 \\
 & 16 & 0.36 & 0.35 & 0.31 & 0.39 & 0.05 & 0.29 & 0.47 & 0.47 & 0.62 & 0.58 & 0.54 & 0.64 & 0.40 & 0.59 & 0.38 & 1 & 0.50 & 0.36 & 0.31 & 0.33 & 0.17 & 0.39 & 0.45 & 0.38 & 0.35 & 0.13 & 0.46 & 0.70 & 0.30 \\
 & 17 & 0.16 & 0.10 & 0.42 & 0.19 & 0.21 & 0.33 & 0.21 & 0.66 & 0.22 & 0.03 & 0.23 & 0.15 & 0.26 & 0.22 & 0.17 & 0.22 & 0.27 & 0.36 & 1 & 0.17 & 0.42 & 0 & 0.21 & 0.27 & 0.11 & 0.36 & 0.24 & 0.40 & 0.30 \\
 & 18 & 0.04 & 0.02 & 0 & 0.03 & 0 & 0 & 0.02 & 0 & 0 & 0.05 & 0.08 & 0.45 & 0.04 & 0.19 & 0.02 & 0.08 & 1 & 0 & 0.06 & 0.02 & 0.12 & 0 & 0.07 & 0.04 & 0 & 0.01 & 0.06 & 0 & 0.04 \\
 & 19 & 0.04 & 0.04 & 0 & 0.04 & 0 & 0 & 0 & 0 & 0 & 0 & 0.05 & 0 & 0.06 & 0.03 & 0.11 & 0.05 & 0 & 1 & 0.06 & 0.02 & 0 & 0.11 & 0.04 & 0.03 & 0 & 0 & 0.04 & 0 & 0.05 \\
 & 20 & 0.05 & 0.07 & 0.06 & 0.09 & 0 & 0 & 0.02 & 0.11 & 0.12 & 0.08 & 0.13 & 0.04 & 0.15 & 0.25 & 0.02 & 0.10 & 0.04 & 0.05 & 0.08 & 1 & 0 & 0.13 & 0.20 & 0.03 & 0.77 & 0 & 0.09 & 0.09 & 0.11 \\
 & 21 & 0 & 0.01 & 0.03 & 0.01 & 0.01 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0.03 & 0 & 0.03 & 0.01 & 0.06 & 0 & 0.05 & 0 & 1 & 0.04 & 0 & 0.03 & 0 & 0 & 0 & 0.02 & 0.07 \\
 & 22 & 0 & 0.05 & 0 & 0.02 & 0.03 & 0.04 & 0 & 0.13 & 0 & 0 & 0.01 & 0 & 0.01 & 0.03 & 0.03 & 0.05 & 0 & 0.11 & 0 & 0.05 & 0.06 & 1 & 0 & 0.20 & 0 & 0.10 & 0.04 & 0.02 & 0.10 \\
 & 23 & 0.02 & 0.08 & 0 & 0.03 & 0.11 & 0.03 & 0.14 & 0 & 0.05 & 0.15 & 0.33 & 0.02 & 0.23 & 0.08 & 0.06 & 0.17 & 0.16 & 0.12 & 0.11 & 0.23 & 0 & 0 & 1 & 0.08 & 0.24 & 0.02 & 0.13 & 0.11 & 0.11 \\
 & 24 & 0.03 & 0.02 & 0 & 0.01 & 0.03 & 0.04 & 0.03 & 0.13 & 0.07 & 0 & 0 & 0 & 0.03 & 0.01 & 0.01 & 0.05 & 0.03 & 0.03 & 0.05 & 0.01 & 0.04 & 0.21 & 0.03 & 1 & 0 & 0 & 0.05 & 0 & 0.07 \\
 & 25 & 0.03 & 0.04 & 0.21 & 0.03 & 0 & 0 & 0 & 0 & 0 & 0.06 & 0.14 & 0 & 0.08 & 0.20 & 0.02 & 0.06 & 0 & 0 & 0.03 & 0.41 & 0 & 0 & 0.11 & 0 & 1 & 0 & 0.03 & 0.07 & 0.02 \\
 & 26 & 0 & 0.03 & 0 & 0.07 & 0.03 & 0.38 & 0 & 0 & 0.07 & 0 & 0 & 0 & 0.03 & 0.02 & 0.03 & 0.02 & 0.01 & 0 & 0.07 & 0 & 0 & 0.11 & 0.01 & 0 & 0 & 1 & 0.06 & 0 & 0.09 \\
 & 27 & 0.25 & 0.16 & 0 & 0.38 & 0.09 & 0.03 & 0.08 & 0.13 & 0.11 & 0.15 & 0.02 & 0.25 & 0.16 & 0.12 & 0.10 & 0.19 & 0.15 & 0.14 & 0.14 & 0.11 & 0 & 0.14 & 0.14 & 0.16 & 0.06 & 0.17 & 1 & 0 & 0.19 \\
 & 28 & 0 & 0.02 & 0.03 & 0.01 & 0 & 0.08 & 0.05 & 0 & 0.04 & 0.01 & 0.06 & 0 & 0.07 & 0.07 & 0.05 & 0.09 & 0 & 0 & 0.07 & 0.04 & 0.04 & 0.02 & 0.04 & 0 & 0.06 & 0 & 0 & 1 & 0.02 \\
 & 29 & 0.30 & 0.44 & 0.14 & 0.34 & 0.47 & 0.89 & 0.16 & 0 & 0.26 & 0.04 & 0.14 & 0.13 & 0.20 & 0.29 & 0.28 & 0.25 & 0.19 & 0.30 & 0.35 & 0.28 & \textbf{0.67} & 0.68 & 0.24 & 0.48 & 0.10 & 0.56 & 0.39 & 0.16 & 1 \\


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Misprediction
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline \hline
\rowcolor[HTML]{D9D9D9}
\multicolumn{31}{c}{(c) \textbf{Misprediction}}\\
\hline \hline


 \multirow{30}{*}{\rotatebox{90}{Predicted Class ID $\downarrow$}} & 1 & 0 & 0.04 & 0 & 0 & 0.01 & 0 & 0.03 & 0 & 0.01 & 0.03 & 0 & 0.02 & 0.02 & 0.01 & 0.04 & 0.01 & 0.01 & 0.01 & 0.02 & 0.02 & 0 & 0 & 0.02 & 0 & 0 & 0.01 & 0.06 & 0 & 0.02 \\
 & 2 & 0.18 & 0 & 0.02 & 0.03 & 0.13 & 0 & 0.09 & 0 & 0.04 & 0.12 & 0.03 & 0.04 & 0.06 & 0.07 & 0.09 & 0.06 & 0.01 & 0.04 & 0.07 & 0.06 & 0.09 & 0.04 & 0.07 & 0.05 & 0.06 & 0.06 & 0.08 & 0.03 & 0.04 \\
 & 3 & 0.01 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0.01 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0.01 & 0 & 0.01 & 0 & 0 & 0 & 0 \\
 & 4 & 0.64 & 0.19 & 0.02 & 0 & 0.06 & 0 & 0.09 & 0 & 0.03 & 0.18 & 0.01 & 0.04 & 0.05 & 0.03 & 0.08 & 0.06 & 0.01 & 0.01 & 0.08 & 0.07 & 0.02 & 0 & 0.05 & 0.02 & 0.02 & 0.07 & 0.13 & 0.01 & 0.06 \\
 & 5 & 0 & 0.01 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0.01 & 0 & 0 & 0.01 & 0 & 0 & 0.01 & 0 & 0.02 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0.01 \\
 & 6 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0.01 & 0.02 & 0.03 & 0 & 0 & 0 & 0.03 & 0 & 0 & 0 \\
 & 7 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0 & 0.02 & 0 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 & 8 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 & 9 & 0.02 & 0.01 & 0 & 0.01 & 0.01 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0.01 & 0.03 & 0.01 & 0 & 0 & 0 & 0.02 & 0.01 & 0.02 & 0 & 0.02 & 0 & 0 & 0.01 & 0.02 & 0.01 & 0.01 \\
 & 10 & 0.03 & 0.01 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0.01 & 0 & 0.02 & 0.01 & 0.02 & 0.01 & 0.01 & 0 & 0 & 0.04 & 0 & 0 & 0.03 & 0 & 0 & 0 & 0.03 & 0 & 0 \\
 & 11 & 0.02 & 0.03 & 0 & 0.01 & 0 & 0 & 0 & 0.02 & 0.01 & 0.03 & 0 & 0.02 & 0.02 & 0.03 & 0.03 & 0.02 & 0.02 & 0 & 0.04 & 0.06 & 0 & 0.02 & 0.03 & 0 & 0.01 & 0 & 0.03 & 0 & 0.01 \\
 & 12 & 0 & 0 & 0 & 0 & 0 & 0 & 0.03 & 0 & 0 & 0 & 0 & 0 & 0 & 0.02 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0 \\
 & 13 & 0.03 & 0.06 & 0.03 & 0.05 & 0.09 & 0 & 0 & 0.05 & 0.04 & 0 & 0.18 & 0 & 0 & 0.09 & 0.05 & 0.07 & 0 & 0.08 & 0.13 & 0.14 & 0.08 & 0 & 0.09 & 0.05 & 0.03 & 0.05 & 0.08 & 0.08 & 0.08 \\
 & 14 & 0.02 & 0.02 & 0.04 & 0.01 & 0.03 & 0 & 0.01 & 0 & 0 & 0.01 & 0.04 & 0.02 & 0.01 & 0 & 0.02 & 0.02 & 0.03 & 0 & 0.03 & 0.02 & 0.07 & 0 & 0.03 & 0.01 & 0.01 & 0.04 & 0.03 & 0.02 & 0.02 \\
 & 15 & 0.01 & 0.03 & 0 & 0.02 & 0.14 & 0 & 0.05 & 0 & 0 & 0.03 & 0.03 & 0.02 & 0.02 & 0.03 & 0 & 0.03 & 0.02 & 0.02 & 0.04 & 0.01 & 0.10 & 0.02 & 0.03 & 0.03 & 0 & 0.03 & 0.03 & 0 & 0.03 \\
 & 16 & 0.16 & 0.11 & 0.10 & 0.10 & 0.16 & 0 & 0.08 & 0.07 & 0.08 & 0.21 & 0.23 & 0.05 & 0.15 & 0.51 & 0.19 & 0 & 0.04 & 0.13 & 0.17 & 0.17 & 0.15 & 0.08 & 0.17 & 0.23 & 0.08 & 0.06 & 0.26 & 0.26 & 0.10 \\
 & 17 & 0.07 & 0.05 & 0.03 & 0.04 & 0.09 & 0.03 & 0.03 & 0.05 & 0.01 & 0.04 & 0.11 & 0.02 & 0.03 & 0.11 & 0.03 & 0.04 & 0 & 0.07 & 0 & 0.04 & 0.12 & 0 & 0.02 & 0.04 & 0.02 & 0.08 & 0.03 & 0.10 & 0.05 \\
 & 18 & 0 & 0.01 & 0.02 & 0 & 0.01 & 0 & 0.03 & 0 & 0 & 0 & 0.04 & 0 & 0.01 & 0.01 & 0 & 0.01 & 0 & 0 & 0.01 & 0.01 & 0.05 & 0.01 & 0.01 & 0 & 0 & 0 & 0 & 0.01 & 0.01 \\
 & 19 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0 \\
 & 20 & 0.02 & 0.03 & 0.06 & 0.02 & 0.03 & 0 & 0.01 & 0 & 0.04 & 0.03 & 0.04 & 0 & 0.01 & 0.06 & 0.01 & 0.03 & 0 & 0.01 & 0.05 & 0 & 0 & 0.03 & 0.02 & 0.09 & 0.19 & 0.02 & 0.02 & 0.02 & 0.03 \\
 & 21 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0 \\
 & 22 & 0 & 0 & 0 & 0 & 0.03 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0.05 & 0 & 0 & 0 & 0 & 0.01 & 0.02 & 0 & 0.01 \\
 & 23 & 0.02 & 0.04 & 0 & 0.03 & 0.03 & 0 & 0 & 0 & 0.03 & 0.03 & 0.15 & 0 & 0.07 & 0.07 & 0.06 & 0.05 & 0.02 & 0.05 & 0.07 & 0.11 & 0 & 0 & 0 & 0.09 & 0.01 & 0.01 & 0.06 & 0.02 & 0.04 \\
 & 24 & 0.01 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0.01 & 0.01 & 0 & 0 & 0.02 & 0.01 & 0 & 0.04 & 0 & 0 & 0.01 & 0 & 0.02 & 0.01 & 0.02 \\
 & 25 & 0 & 0 & 0.07 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
 & 26 & 0.01 & 0.01 & 0 & 0.01 & 0.03 & 0.03 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0.01 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0.01 \\
 & 27 & 0.09 & 0.08 & 0 & 0.12 & 0.04 & 0.02 & 0.03 & 0 & 0 & 0.03 & 0.05 & 0 & 0.05 & 0.04 & 0.05 & 0.07 & 0 & 0.01 & 0.10 & 0.08 & 0 & 0.04 & 0.09 & 0.04 & 0 & 0 & 0 & 0.01 & 0.06 \\
 & 28 & 0.01 & 0 & 0 & 0 & 0.01 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0 & 0.03 & 0.01 & 0 & 0 & 0.01 & 0.02 & 0.02 & 0 & 0.02 & 0 & 0 & 0.02 & 0.02 & 0 & 0 & 0.01 \\
 & 29 & 0.13 & 0.16 & 0.04 & 0.07 & 0.38 & 0.17 & 0.03 & 0 & 0.04 & 0.03 & 0.07 & 0.02 & 0.07 & 0.13 & 0.10 & 0.07 & 0.01 & 0.02 & 0.22 & 0.12 & \textbf{0.79} & 0.14 & 0.08 & 0.25 & 0.04 & 0.30 & 0.14 & 0 & 0 \\
 & 30 & 0.01 & 0 & 0 & 0 & 0.03 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0.01 & 0.01 & 0.01 & 0.01 & 0 & 0.01 & 0.01 & 0.01 & 0.02 & 0 & 0 & 0 & 0 & 0.01 & 0.01 & 0 & 0.01 \\
\hline
\end{tabular}
\end{adjustbox}

\label{tab:misclassification_fiction}
\end{table*}

==> tables/misclassification_non_fiction.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%% Version-1 Uncleaned
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table*}[]
% \centering
% \caption{Non-fiction genre indistinguishability analysis}


% % \begin{adjustbox}{angle=90, height=0.87\textheight}
% \begin{adjustbox}{width=1\textwidth} 
% \begin{tabular}{cc|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
% \hline
% & Class ID $\downarrow\rightarrow$  & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & 28 & 30 \\

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Sample Count
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \hline \hline
% \multicolumn{31}{c}{(a) \textbf{Sample Count}}\\
% \hline \hline


%  & 1 & 748 & 169 & 0 & 222 & 41 & 0 & 12 & 0 & 306 & 14 & 0 & 12 & 89 & 52 & 97 & 44 & 14 & 10 & 0 & 16 & 0 & 95 & 0 & 369 & 14 & 0 & 65 & 37 & 157 \\
%  & 2 & 169 & 1444 & 9 & 331 & 203 & 42 & 0 & 143 & 53 & 34 & 103 & 12 & 512 & 237 & 165 & 109 & 26 & 57 & 58 & 58 & 270 & 408 & 125 & 236 & 14 & 8 & 162 & 28 & 259 \\
%  & 3 & 0 & 9 & 614 & 0 & 46 & 197 & 0 & 0 & 0 & 24 & 0 & 0 & 197 & 303 & 38 & 9 & 0 & 0 & 0 & 34 & 44 & 84 & 0 & 58 & 227 & 0 & 8 & 0 & 107 \\
%  & 4 & 222 & 331 & 0 & 878 & 41 & 0 & 8 & 28 & 84 & 170 & 0 & 31 & 214 & 140 & 82 & 52 & 37 & 46 & 0 & 9 & 0 & 152 & 0 & 340 & 61 & 9 & 315 & 0 & 109 \\
%  & 5 & 41 & 203 & 46 & 41 & 806 & 0 & 0 & 17 & 19 & 10 & 47 & 17 & 308 & 274 & 298 & 50 & 0 & 25 & 24 & 16 & 8 & 216 & 11 & 176 & 19 & 0 & 19 & 16 & 187 \\
%  & 6 & 0 & 42 & 197 & 0 & 0 & 483 & 0 & 0 & 11 & 0 & 0 & 0 & 165 & 183 & 11 & 0 & 8 & 12 & 0 & 0 & 0 & 69 & 0 & 201 & 28 & 9 & 0 & 0 & 73 \\
%  & 7 & 12 & 0 & 0 & 8 & 0 & 0 & 494 & 0 & 72 & 0 & 9 & 183 & 38 & 26 & 26 & 38 & 41 & 9 & 0 & 11 & 0 & 185 & 12 & 29 & 89 & 0 & 8 & 104 & 111 \\
%  & 8 & 0 & 143 & 0 & 28 & 17 & 0 & 0 & 439 & 45 & 0 & 110 & 8 & 52 & 44 & 8 & 19 & 0 & 34 & 0 & 32 & 0 & 290 & 0 & 0 & 47 & 8 & 0 & 0 & 12 \\
%  & 9 & 306 & 53 & 0 & 84 & 19 & 11 & 72 & 45 & 846 & 0 & 0 & 66 & 197 & 132 & 37 & 39 & 11 & 0 & 76 & 17 & 9 & 174 & 0 & 361 & 9 & 55 & 41 & 122 & 196 \\
%  & 10 & 14 & 34 & 24 & 170 & 10 & 0 & 0 & 0 & 0 & 889 & 119 & 142 & 16 & 521 & 33 & 25 & 149 & 84 & 0 & 193 & 0 & 222 & 225 & 54 & 506 & 9 & 80 & 0 & 57 \\
%  & 11 & 0 & 103 & 0 & 0 & 47 & 0 & 9 & 110 & 0 & 119 & 896 & 0 & 210 & 398 & 85 & 216 & 12 & 68 & 47 & 71 & 33 & 223 & 282 & 39 & 133 & 12 & 0 & 9 & 204 \\
%  & 12 & 12 & 12 & 0 & 31 & 17 & 0 & 183 & 8 & 66 & 142 & 0 & 949 & 17 & 381 & 0 & 11 & 456 & 0 & 0 & 92 & 0 & 400 & 11 & 221 & 506 & 16 & 0 & 0 & 84 \\
%  & 13 & 89 & 512 & 197 & 214 & 308 & 165 & 38 & 52 & 197 & 16 & 210 & 17 & 3297 & 1016 & 250 & 556 & 128 & 258 & 383 & 249 & 412 & 478 & 198 & 590 & 9 & 84 & 266 & 369 & 1198 \\
%  & 14 & 52 & 237 & 303 & 140 & 274 & 183 & 26 & 44 & 132 & 521 & 398 & 381 & 1016 & 3417 & 295 & 594 & 353 & 254 & 103 & 532 & 241 & 632 & 369 & 597 & 783 & 24 & 255 & 92 & 581 \\
%  & 15 & 97 & 165 & 38 & 82 & 298 & 11 & 26 & 8 & 37 & 33 & 85 & 0 & 250 & 295 & 1112 & 97 & 0 & 37 & 39 & 12 & 104 & 149 & 11 & 77 & 33 & 52 & 40 & 147 & 405 \\
%  & 16 & 44 & 109 & 9 & 52 & 50 & 0 & 38 & 19 & 39 & 25 & 216 & 11 & 556 & 594 & 97 & 1448 & 34 & 236 & 93 & 126 & 102 & 207 & 265 & 66 & 17 & 0 & 96 & 204 & 575 \\
%  & 17 & 0 & 58 & 0 & 0 & 24 & 0 & 0 & 0 & 76 & 0 & 47 & 0 & 383 & 103 & 39 & 93 & 44 & 41 & 744 & 55 & 126 & 103 & 87 & 58 & 9 & 81 & 0 & 221 & 383 \\
%  & 18 & 14 & 26 & 0 & 37 & 0 & 8 & 41 & 0 & 11 & 149 & 12 & 456 & 128 & 353 & 0 & 34 & 886 & 0 & 44 & 143 & 9 & 241 & 20 & 318 & 361 & 0 & 0 & 0 & 179 \\
%  & 19 & 10 & 57 & 0 & 46 & 25 & 12 & 9 & 34 & 0 & 84 & 68 & 0 & 258 & 254 & 37 & 236 & 0 & 762 & 41 & 52 & 0 & 315 & 0 & 32 & 27 & 0 & 25 & 37 & 289 \\
%  & 20 & 16 & 58 & 34 & 9 & 16 & 0 & 11 & 32 & 17 & 193 & 71 & 92 & 249 & 532 & 12 & 126 & 143 & 52 & 55 & 1122 & 0 & 135 & 205 & 93 & 416 & 12 & 0 & 36 & 147 \\
%  & 21 & 0 & 270 & 44 & 0 & 8 & 0 & 0 & 0 & 9 & 0 & 33 & 0 & 412 & 241 & 104 & 102 & 9 & 0 & 126 & 0 & 735 & 104 & 42 & 42 & 0 & 11 & 8 & 67 & 278 \\
%  & 22 & 95 & 408 & 84 & 152 & 216 & 69 & 185 & 290 & 174 & 222 & 223 & 400 & 478 & 632 & 149 & 207 & 241 & 315 & 103 & 135 & 104 & 2495 & 171 & 327 & 462 & 129 & 149 & 72 & 107 \\
%  & 23 & 0 & 125 & 0 & 0 & 11 & 0 & 12 & 0 & 0 & 225 & 282 & 11 & 198 & 369 & 11 & 265 & 20 & 0 & 87 & 205 & 42 & 171 & 877 & 70 & 273 & 12 & 0 & 43 & 162 \\
%  & 24 & 369 & 236 & 58 & 340 & 176 & 201 & 29 & 0 & 361 & 54 & 39 & 221 & 590 & 597 & 77 & 66 & 318 & 32 & 58 & 93 & 42 & 327 & 70 & 1809 & 148 & 0 & 188 & 41 & 207 \\
%  & 25 & 14 & 14 & 227 & 61 & 19 & 28 & 89 & 47 & 9 & 506 & 133 & 506 & 9 & 783 & 33 & 17 & 361 & 27 & 9 & 416 & 0 & 462 & 273 & 148 & 1519 & 25 & 16 & 9 & 63 \\
%  & 26 & 0 & 8 & 0 & 9 & 0 & 9 & 0 & 8 & 55 & 9 & 12 & 16 & 84 & 24 & 52 & 0 & 0 & 0 & 81 & 12 & 11 & 129 & 12 & 0 & 25 & 424 & 0 & 69 & 185 \\
%  & 27 & 65 & 162 & 8 & 315 & 19 & 0 & 8 & 0 & 41 & 80 & 0 & 0 & 266 & 255 & 40 & 96 & 0 & 25 & 0 & 0 & 8 & 149 & 0 & 188 & 16 & 0 & 659 & 0 & 151 \\
%  & 28 & 37 & 28 & 0 & 0 & 16 & 0 & 104 & 0 & 122 & 0 & 9 & 0 & 369 & 92 & 147 & 204 & 0 & 37 & 221 & 36 & 67 & 72 & 43 & 41 & 9 & 69 & 0 & 888 & 543 \\
%  & 30 & 157 & 259 & 107 & 109 & 187 & 73 & 111 & 12 & 196 & 57 & 204 & 84 & 1198 & 581 & 405 & 575 & 179 & 289 & 383 & 147 & 278 & 107 & 162 & 207 & 63 & 185 & 151 & 543 & 2802 \\

 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Cooccurrence
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \hline \hline
% \multicolumn{31}{c}{(b) \textbf{Cooccurrence}}\\
% \hline \hline


%  & 1 & 1.00 & 0.12 & 0.00 & 0.25 & 0.05 & 0.00 & 0.02 & 0.00 & 0.36 & 0.02 & 0.00 & 0.01 & 0.03 & 0.02 & 0.09 & 0.03 & 0.02 & 0.01 & 0.00 & 0.01 & 0.00 & 0.04 & 0.00 & 0.20 & 0.01 & 0.00 & 0.10 & 0.04 & 0.06 \\
%  & 2 & 0.23 & 1.00 & 0.01 & 0.38 & 0.25 & 0.09 & 0.00 & 0.33 & 0.06 & 0.04 & 0.11 & 0.01 & 0.16 & 0.07 & 0.15 & 0.08 & 0.03 & 0.07 & 0.08 & 0.05 & 0.37 & 0.16 & 0.14 & 0.13 & 0.01 & 0.02 & 0.25 & 0.03 & 0.09 \\
%  & 3 & 0.00 & 0.01 & 1.00 & 0.00 & 0.06 & 0.41 & 0.00 & 0.00 & 0.00 & 0.03 & 0.00 & 0.00 & 0.06 & 0.09 & 0.03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.03 & 0.06 & 0.03 & 0.00 & 0.03 & 0.15 & 0.00 & 0.01 & 0.00 & 0.04 \\
%  & 4 & 0.30 & 0.23 & 0.00 & 1.00 & 0.05 & 0.00 & 0.02 & 0.06 & 0.10 & 0.19 & 0.00 & 0.03 & 0.06 & 0.04 & 0.07 & 0.04 & 0.04 & 0.06 & 0.00 & 0.01 & 0.00 & 0.06 & 0.00 & 0.19 & 0.04 & 0.02 & 0.48 & 0.00 & 0.04 \\
%  & 5 & 0.05 & 0.14 & 0.07 & 0.05 & 1.00 & 0.00 & 0.00 & 0.04 & 0.02 & 0.01 & 0.05 & 0.02 & 0.09 & 0.08 & 0.27 & 0.03 & 0.00 & 0.03 & 0.03 & 0.01 & 0.01 & 0.09 & 0.01 & 0.10 & 0.01 & 0.00 & 0.03 & 0.02 & 0.07 \\
%  & 6 & 0.00 & 0.03 & 0.32 & 0.00 & 0.00 & 1.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.05 & 0.05 & 0.01 & 0.00 & 0.01 & 0.02 & 0.00 & 0.00 & 0.00 & 0.03 & 0.00 & 0.11 & 0.02 & 0.02 & 0.00 & 0.00 & 0.03 \\
%  & 7 & 0.02 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 1.00 & 0.00 & 0.09 & 0.00 & 0.01 & 0.19 & 0.01 & 0.01 & 0.02 & 0.03 & 0.05 & 0.01 & 0.00 & 0.01 & 0.00 & 0.07 & 0.01 & 0.02 & 0.06 & 0.00 & 0.01 & 0.12 & 0.04 \\
%  & 8 & 0.00 & 0.10 & 0.00 & 0.03 & 0.02 & 0.00 & 0.00 & 1.00 & 0.05 & 0.00 & 0.12 & 0.01 & 0.02 & 0.01 & 0.01 & 0.01 & 0.00 & 0.04 & 0.00 & 0.03 & 0.00 & 0.12 & 0.00 & 0.00 & 0.03 & 0.02 & 0.00 & 0.00 & 0.00 \\
%  & 9 & 0.41 & 0.04 & 0.00 & 0.10 & 0.02 & 0.02 & 0.15 & 0.10 & 1.00 & 0.00 & 0.00 & 0.07 & 0.06 & 0.04 & 0.03 & 0.03 & 0.01 & 0.00 & 0.10 & 0.02 & 0.01 & 0.07 & 0.00 & 0.20 & 0.01 & 0.13 & 0.06 & 0.14 & 0.07 \\
%  & 10 & 0.02 & 0.02 & 0.04 & 0.19 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.13 & 0.15 & 0.00 & 0.15 & 0.03 & 0.02 & 0.17 & 0.11 & 0.00 & 0.17 & 0.00 & 0.09 & 0.26 & 0.03 & 0.33 & 0.02 & 0.12 & 0.00 & 0.02 \\
%  & 11 & 0.00 & 0.07 & 0.00 & 0.00 & 0.06 & 0.00 & 0.02 & 0.25 & 0.00 & 0.13 & 1.00 & 0.00 & 0.06 & 0.12 & 0.08 & 0.15 & 0.01 & 0.09 & 0.06 & 0.06 & 0.04 & 0.09 & 0.32 & 0.02 & 0.09 & 0.03 & 0.00 & 0.01 & 0.07 \\
%  & 12 & 0.02 & 0.01 & 0.00 & 0.04 & 0.02 & 0.00 & 0.37 & 0.02 & 0.08 & 0.16 & 0.00 & 1.00 & 0.01 & 0.11 & 0.00 & 0.01 & 0.51 & 0.00 & 0.00 & 0.08 & 0.00 & 0.16 & 0.01 & 0.12 & 0.33 & 0.04 & 0.00 & 0.00 & 0.03 \\
%  & 13 & 0.12 & 0.35 & 0.32 & 0.24 & 0.38 & 0.34 & 0.08 & 0.12 & 0.23 & 0.02 & 0.23 & 0.02 & 1.00 & 0.30 & 0.22 & 0.38 & 0.14 & 0.34 & 0.51 & 0.22 & 0.56 & 0.19 & 0.23 & 0.33 & 0.01 & 0.20 & 0.40 & 0.42 & 0.43 \\
%  & 14 & 0.07 & 0.16 & 0.49 & 0.16 & 0.34 & 0.38 & 0.05 & 0.10 & 0.16 & 0.59 & 0.44 & 0.40 & 0.31 & 1.00 & 0.27 & 0.41 & 0.40 & 0.33 & 0.14 & 0.47 & 0.33 & 0.25 & 0.42 & 0.33 & 0.52 & 0.06 & 0.39 & 0.10 & 0.21 \\
%  & 15 & 0.13 & 0.11 & 0.06 & 0.09 & 0.37 & 0.02 & 0.05 & 0.02 & 0.04 & 0.04 & 0.09 & 0.00 & 0.08 & 0.09 & 1.00 & 0.07 & 0.00 & 0.05 & 0.05 & 0.01 & 0.14 & 0.06 & 0.01 & 0.04 & 0.02 & 0.12 & 0.06 & 0.17 & 0.14 \\
%  & 16 & 0.06 & 0.08 & 0.01 & 0.06 & 0.06 & 0.00 & 0.08 & 0.04 & 0.05 & 0.03 & 0.24 & 0.01 & 0.17 & 0.17 & 0.09 & 1.00 & 0.04 & 0.31 & 0.13 & 0.11 & 0.14 & 0.08 & 0.30 & 0.04 & 0.01 & 0.00 & 0.15 & 0.23 & 0.21 \\
%  & 17 & 0.00 & 0.04 & 0.00 & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 & 0.09 & 0.00 & 0.05 & 0.00 & 0.12 & 0.03 & 0.04 & 0.06 & 0.05 & 0.05 & 1.00 & 0.05 & 0.17 & 0.04 & 0.10 & 0.03 & 0.01 & 0.19 & 0.00 & 0.25 & 0.14 \\
%  & 18 & 0.02 & 0.02 & 0.00 & 0.04 & 0.00 & 0.02 & 0.08 & 0.00 & 0.01 & 0.17 & 0.01 & 0.48 & 0.04 & 0.10 & 0.00 & 0.02 & 1.00 & 0.00 & 0.06 & 0.13 & 0.01 & 0.10 & 0.02 & 0.18 & 0.24 & 0.00 & 0.00 & 0.00 & 0.06 \\
%  & 19 & 0.01 & 0.04 & 0.00 & 0.05 & 0.03 & 0.02 & 0.02 & 0.08 & 0.00 & 0.09 & 0.08 & 0.00 & 0.08 & 0.07 & 0.03 & 0.16 & 0.00 & 1.00 & 0.06 & 0.05 & 0.00 & 0.13 & 0.00 & 0.02 & 0.02 & 0.00 & 0.04 & 0.04 & 0.10 \\
%  & 20 & 0.02 & 0.04 & 0.06 & 0.01 & 0.02 & 0.00 & 0.02 & 0.07 & 0.02 & 0.22 & 0.08 & 0.10 & 0.08 & 0.16 & 0.01 & 0.09 & 0.16 & 0.07 & 0.07 & 1.00 & 0.00 & 0.05 & 0.23 & 0.05 & 0.27 & 0.03 & 0.00 & 0.04 & 0.05 \\
%  & 21 & 0.00 & 0.19 & 0.07 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.04 & 0.00 & 0.12 & 0.07 & 0.09 & 0.07 & 0.01 & 0.00 & 0.17 & 0.00 & 1.00 & 0.04 & 0.05 & 0.02 & 0.00 & 0.03 & 0.01 & 0.08 & 0.10 \\
%  & 22 & 0.13 & 0.28 & 0.14 & 0.17 & 0.27 & 0.14 & 0.37 & 0.66 & 0.21 & 0.25 & 0.25 & 0.42 & 0.14 & 0.18 & 0.13 & 0.14 & 0.27 & 0.41 & 0.14 & 0.12 & 0.14 & 1.00 & 0.19 & 0.18 & 0.30 & 0.30 & 0.23 & 0.08 & 0.04 \\
%  & 23 & 0.00 & 0.09 & 0.00 & 0.00 & 0.01 & 0.00 & 0.02 & 0.00 & 0.00 & 0.25 & 0.31 & 0.01 & 0.06 & 0.11 & 0.01 & 0.18 & 0.02 & 0.00 & 0.12 & 0.18 & 0.06 & 0.07 & 1.00 & 0.04 & 0.18 & 0.03 & 0.00 & 0.05 & 0.06 \\
%  & 24 & 0.49 & 0.16 & 0.09 & 0.39 & 0.22 & 0.42 & 0.06 & 0.00 & 0.43 & 0.06 & 0.04 & 0.23 & 0.18 & 0.17 & 0.07 & 0.05 & 0.36 & 0.04 & 0.08 & 0.08 & 0.06 & 0.13 & 0.08 & 1.00 & 0.10 & 0.00 & 0.29 & 0.05 & 0.07 \\
%  & 25 & 0.02 & 0.01 & 0.37 & 0.07 & 0.02 & 0.06 & 0.18 & 0.11 & 0.01 & 0.57 & 0.15 & 0.53 & 0.00 & 0.23 & 0.03 & 0.01 & 0.41 & 0.04 & 0.01 & 0.37 & 0.00 & 0.19 & 0.31 & 0.08 & 1.00 & 0.06 & 0.02 & 0.01 & 0.02 \\
%  & 26 & 0.00 & 0.01 & 0.00 & 0.01 & 0.00 & 0.02 & 0.00 & 0.02 & 0.07 & 0.01 & 0.01 & 0.02 & 0.03 & 0.01 & 0.05 & 0.00 & 0.00 & 0.00 & 0.11 & 0.01 & 0.01 & 0.05 & 0.01 & 0.00 & 0.02 & 1.00 & 0.00 & 0.08 & 0.07 \\
%  & 27 & 0.09 & 0.11 & 0.01 & 0.36 & 0.02 & 0.00 & 0.02 & 0.00 & 0.05 & 0.09 & 0.00 & 0.00 & 0.08 & 0.07 & 0.04 & 0.07 & 0.00 & 0.03 & 0.00 & 0.00 & 0.01 & 0.06 & 0.00 & 0.10 & 0.01 & 0.00 & 1.00 & 0.00 & 0.05 \\
%  & 28 & 0.05 & 0.02 & 0.00 & 0.00 & 0.02 & 0.00 & 0.21 & 0.00 & 0.14 & 0.00 & 0.01 & 0.00 & 0.11 & 0.03 & 0.13 & 0.14 & 0.00 & 0.05 & 0.30 & 0.03 & 0.09 & 0.03 & 0.05 & 0.02 & 0.01 & 0.16 & 0.00 & 1.00 & 0.19 \\
%  & 30 & 0.21 & 0.18 & 0.17 & 0.12 & 0.23 & 0.15 & 0.22 & 0.03 & 0.23 & 0.06 & 0.23 & 0.09 & 0.36 & 0.17 & 0.36 & 0.40 & 0.20 & 0.38 & 0.51 & 0.13 & 0.38 & 0.04 & 0.18 & 0.11 & 0.04 & 0.44 & 0.23 & 0.61 & 1.00 \\

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Misprediction
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \hline \hline
% \multicolumn{31}{c}{(c) \textbf{Misprediction}}\\
% \hline \hline

%  \multirow{30}{*}{\rotatebox{90}{\underline{Predicted Class ID $\downarrow$}}}
%  & 1 & 0.00 & 0.03 & 0.01 & 0.03 & 0.01 & 0.02 & 0.00 & 0.00 & 0.05 & 0.00 & 0.00 & 0.00 & 0.01 & 0.01 & 0.01 & 0.02 & 0.00 & 0.00 & 0.01 & 0.01 & 0.01 & 0.01 & 0.00 & 0.04 & 0.00 & 0.00 & 0.06 & 0.00 & 0.00 \\
%  & 2 & 0.03 & 0.00 & 0.03 & 0.06 & 0.03 & 0.00 & 0.02 & 0.03 & 0.00 & 0.02 & 0.01 & 0.00 & 0.04 & 0.01 & 0.01 & 0.03 & 0.00 & 0.01 & 0.02 & 0.01 & 0.09 & 0.02 & 0.00 & 0.04 & 0.00 & 0.00 & 0.10 & 0.02 & 0.05 \\
%  & 3 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.03 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.02 & 0.00 & 0.02 & 0.00 & 0.00 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 \\
%  & 4 & 0.03 & 0.03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.04 & 0.00 & 0.00 & 0.01 & 0.01 & 0.02 & 0.01 & 0.01 & 0.00 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.04 & 0.01 & 0.00 & 0.17 & 0.01 & 0.01 \\
%  & 5 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.04 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.04 & 0.00 & 0.00 \\
%  & 6 & 0.00 & 0.01 & 0.06 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.01 \\
%  & 7 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.01 & 0.01 & 0.00 & 0.00 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.01 \\
%  & 8 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\
%  & 9 & 0.07 & 0.02 & 0.00 & 0.04 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.01 & 0.02 & 0.02 & 0.02 & 0.00 & 0.00 & 0.00 & 0.01 & 0.02 & 0.00 & 0.00 & 0.02 & 0.01 & 0.00 & 0.05 & 0.03 & 0.02 \\
%  & 10 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.02 & 0.00 & 0.03 & 0.01 & 0.01 & 0.01 & 0.00 & 0.00 & 0.04 & 0.01 & 0.00 & 0.01 & 0.00 & 0.06 & 0.00 & 0.03 & 0.01 & 0.01 \\
%  & 11 & 0.02 & 0.01 & 0.00 & 0.00 & 0.01 & 0.00 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.01 & 0.01 & 0.01 & 0.03 & 0.04 & 0.00 & 0.00 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.02 & 0.00 & 0.01 & 0.02 & 0.03 \\
%  & 12 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.09 & 0.00 & 0.00 & 0.02 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.02 & 0.00 & 0.02 & 0.00 & 0.02 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\
%  & 13 & 0.03 & 0.06 & 0.16 & 0.09 & 0.10 & 0.03 & 0.02 & 0.00 & 0.03 & 0.00 & 0.09 & 0.00 & 0.00 & 0.06 & 0.09 & 0.16 & 0.04 & 0.03 & 0.23 & 0.04 & 0.11 & 0.02 & 0.01 & 0.04 & 0.01 & 0.03 & 0.43 & 0.24 & 0.16 \\
%  & 14 & 0.00 & 0.06 & 0.08 & 0.00 & 0.05 & 0.00 & 0.00 & 0.07 & 0.01 & 0.10 & 0.05 & 0.04 & 0.00 & 0.00 & 0.07 & 0.09 & 0.07 & 0.03 & 0.07 & 0.15 & 0.11 & 0.02 & 0.02 & 0.07 & 0.09 & 0.02 & 0.25 & 0.07 & 0.05 \\
%  & 15 & 0.03 & 0.01 & 0.00 & 0.02 & 0.05 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.02 & 0.00 & 0.01 & 0.02 & 0.00 & 0.04 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.05 & 0.05 & 0.02 \\
%  & 16 & 0.02 & 0.01 & 0.01 & 0.01 & 0.03 & 0.00 & 0.02 & 0.02 & 0.00 & 0.02 & 0.03 & 0.01 & 0.04 & 0.04 & 0.00 & 0.00 & 0.02 & 0.09 & 0.04 & 0.04 & 0.01 & 0.01 & 0.00 & 0.01 & 0.01 & 0.02 & 0.10 & 0.14 & 0.11 \\
%  & 17 & 0.01 & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.03 & 0.00 & 0.02 & 0.02 & 0.00 & 0.00 & 0.03 & 0.01 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.01 & 0.00 & 0.02 & 0.03 & 0.07 & 0.04 \\
%  & 18 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.04 & 0.00 & 0.00 & 0.02 & 0.00 & 0.00 & 0.00 & 0.01 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.02 & 0.00 & 0.00 & 0.00 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 \\
%  & 19 & 0.00 & 0.01 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.06 & 0.00 & 0.01 & 0.01 & 0.00 & 0.00 & 0.01 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.02 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.01 & 0.01 \\
%  & 20 & 0.01 & 0.04 & 0.00 & 0.02 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0.00 & 0.03 & 0.05 & 0.01 & 0.00 & 0.00 & 0.01 & 0.01 & 0.00 & 0.01 & 0.03 & 0.00 & 0.04 & 0.02 & 0.03 \\
%  & 21 & 0.00 & 0.01 & 0.07 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.04 & 0.02 \\
%  & 22 & 0.03 & 0.01 & 0.02 & 0.04 & 0.03 & 0.04 & 0.06 & 0.24 & 0.04 & 0.07 & 0.00 & 0.05 & 0.03 & 0.04 & 0.06 & 0.02 & 0.01 & 0.00 & 0.00 & 0.04 & 0.00 & 0.00 & 0.00 & 0.03 & 0.02 & 0.03 & 0.08 & 0.02 & 0.01 \\
%  & 23 & 0.02 & 0.00 & 0.00 & 0.00 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.01 & 0.01 & 0.02 & 0.01 & 0.00 & 0.01 & 0.04 & 0.00 & 0.00 & 0.00 & 0.01 & 0.01 & 0.02 & 0.00 & 0.02 & 0.03 \\
%  & 24 & 0.07 & 0.04 & 0.01 & 0.08 & 0.03 & 0.03 & 0.04 & 0.00 & 0.06 & 0.03 & 0.01 & 0.03 & 0.02 & 0.03 & 0.03 & 0.03 & 0.08 & 0.00 & 0.01 & 0.02 & 0.01 & 0.01 & 0.00 & 0.00 & 0.03 & 0.00 & 0.08 & 0.00 & 0.00 \\
%  & 25 & 0.01 & 0.01 & 0.02 & 0.00 & 0.02 & 0.00 & 0.04 & 0.04 & 0.01 & 0.05 & 0.01 & 0.06 & 0.01 & 0.05 & 0.02 & 0.02 & 0.07 & 0.00 & 0.01 & 0.09 & 0.02 & 0.02 & 0.02 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.01 \\
%  & 26 & 0.01 & 0.01 & 0.00 & 0.01 & 0.01 & 0.02 & 0.00 & 0.00 & 0.01 & 0.00 & 0.01 & 0.01 & 0.01 & 0.01 & 0.03 & 0.00 & 0.00 & 0.02 & 0.00 & 0.02 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.02 & 0.01 \\
%  & 27 & 0.00 & 0.01 & 0.00 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.03 & 0.00 & 0.00 & 0.01 & 0.01 & 0.02 & 0.00 & 0.00 & 0.01 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.00 & 0.00 & 0.01 & 0.02 \\
%  & 28 & 0.00 & 0.00 & 0.01 & 0.00 & 0.01 & 0.04 & 0.00 & 0.00 & 0.01 & 0.00 & 0.01 & 0.00 & 0.01 & 0.02 & 0.02 & 0.01 & 0.00 & 0.00 & 0.05 & 0.02 & 0.03 & 0.01 & 0.00 & 0.02 & 0.01 & 0.00 & 0.00 & 0.00 & 0.01 \\
%  & 29 & 0.00 & 0.01 & 0.00 & 0.02 & 0.01 & 0.00 & 0.02 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.01 & 0.01 & 0.01 & 0.00 & 0.00 & 0.01 & 0.02 & 0.00 & 0.01 & 0.00 & 0.01 & 0.00 & 0.00 & 0.00 & 0.00 & 0.02 \\
%  & 30 & 0.06 & 0.05 & 0.10 & 0.06 & 0.01 & 0.00 & 0.00 & 0.00 & 0.01 & 0.04 & 0.12 & 0.03 & 0.10 & 0.07 & 0.09 & 0.14 & 0.12 & 0.07 & 0.17 & 0.08 & 0.13 & 0.03 & 0.03 & 0.05 & 0.04 & 0.07 & 0.23 & 0.23 & 0.00 \\
%  \hline
% \end{tabular}
% \end{adjustbox}
% \label{tab:misclassification_non_fiction}
% \end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Version-2 cleaned
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[]
\centering
\caption{Non-fiction genre indistinguishability analysis}


% \begin{adjustbox}{angle=90, height=0.87\textheight}
\begin{adjustbox}{width=1\textwidth} 
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\hline
& Class ID $\downarrow\rightarrow$  & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & 28 & 30 \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Sample Count
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline \hline
\rowcolor[HTML]{D9D9D9}
\multicolumn{31}{c}{(a) \textbf{Sample Count}}\\
\hline \hline


\multirow{29}{*}{\rotatebox{90}{Actual Class ID $\downarrow$}} & 1 & 748 & 169 & 0 & 222 & 41 & 0 & 12 & 0 & 306 & 14 & 0 & 12 & 89 & 52 & 97 & 44 & 14 & 10 & 0 & 16 & 0 & 95 & 0 & 369 & 14 & 0 & 65 & 37 & 157 \\
 & 2 & 169 & 1444 & 9 & 331 & 203 & 42 & 0 & 143 & 53 & 34 & 103 & 12 & 512 & 237 & 165 & 109 & 26 & 57 & 58 & 58 & 270 & 408 & 125 & 236 & 14 & 8 & 162 & 28 & 259 \\
 & 3 & 0 & 9 & 614 & 0 & 46 & 197 & 0 & 0 & 0 & 24 & 0 & 0 & 197 & 303 & 38 & 9 & 0 & 0 & 0 & 34 & 44 & 84 & 0 & 58 & 227 & 0 & 8 & 0 & 107 \\
 & 4 & 222 & 331 & 0 & 878 & 41 & 0 & 8 & 28 & 84 & 170 & 0 & 31 & 214 & 140 & 82 & 52 & 37 & 46 & 0 & 9 & 0 & 152 & 0 & 340 & 61 & 9 & 315 & 0 & 109 \\
 & 5 & 41 & 203 & 46 & 41 & 806 & 0 & 0 & 17 & 19 & 10 & 47 & 17 & 308 & 274 & 298 & 50 & 0 & 25 & 24 & 16 & 8 & 216 & 11 & 176 & 19 & 0 & 19 & 16 & 187 \\
 & 6 & 0 & 42 & 197 & 0 & 0 & 483 & 0 & 0 & 11 & 0 & 0 & 0 & 165 & 183 & 11 & 0 & 8 & 12 & 0 & 0 & 0 & 69 & 0 & 201 & 28 & 9 & 0 & 0 & 73 \\
 & 7 & 12 & 0 & 0 & 8 & 0 & 0 & 494 & 0 & 72 & 0 & 9 & 183 & 38 & 26 & 26 & 38 & 41 & 9 & 0 & 11 & 0 & 185 & 12 & 29 & 89 & 0 & 8 & 104 & 111 \\
 & 8 & 0 & 143 & 0 & 28 & 17 & 0 & 0 & 439 & 45 & 0 & 110 & 8 & 52 & 44 & 8 & 19 & 0 & 34 & 0 & 32 & 0 & 290 & 0 & 0 & 47 & 8 & 0 & 0 & 12 \\
 & 9 & 306 & 53 & 0 & 84 & 19 & 11 & 72 & 45 & 846 & 0 & 0 & 66 & 197 & 132 & 37 & 39 & 11 & 0 & 76 & 17 & 9 & 174 & 0 & 361 & 9 & 55 & 41 & 122 & 196 \\
 & 10 & 14 & 34 & 24 & 170 & 10 & 0 & 0 & 0 & 0 & 889 & 119 & 142 & 16 & 521 & 33 & 25 & 149 & 84 & 0 & 193 & 0 & 222 & 225 & 54 & 506 & 9 & 80 & 0 & 57 \\
 & 11 & 0 & 103 & 0 & 0 & 47 & 0 & 9 & 110 & 0 & 119 & 896 & 0 & 210 & 398 & 85 & 216 & 12 & 68 & 47 & 71 & 33 & 223 & 282 & 39 & 133 & 12 & 0 & 9 & 204 \\
 & 12 & 12 & 12 & 0 & 31 & 17 & 0 & 183 & 8 & 66 & 142 & 0 & 949 & 17 & 381 & 0 & 11 & 456 & 0 & 0 & 92 & 0 & 400 & 11 & 221 & 506 & 16 & 0 & 0 & 84 \\
 & 13 & 89 & 512 & 197 & 214 & 308 & 165 & 38 & 52 & 197 & 16 & 210 & 17 & \textbf{3297} & 1016 & 250 & 556 & 128 & 258 & 383 & 249 & 412 & 478 & 198 & 590 & 9 & 84 & \textbf{266} & 369 & 1198 \\
 & 14 & 52 & 237 & 303 & 140 & 274 & 183 & 26 & 44 & 132 & 521 & 398 & 381 & 1016 & 3417 & 295 & 594 & 353 & 254 & 103 & 532 & 241 & 632 & 369 & 597 & 783 & 24 & 255 & 92 & 581 \\
 & 15 & 97 & 165 & 38 & 82 & 298 & 11 & 26 & 8 & 37 & 33 & 85 & 0 & 250 & 295 & 1112 & 97 & 0 & 37 & 39 & 12 & 104 & 149 & 11 & 77 & 33 & 52 & 40 & 147 & 405 \\
 & 16 & 44 & 109 & 9 & 52 & 50 & 0 & 38 & 19 & 39 & 25 & 216 & 11 & 556 & 594 & 97 & 1448 & 34 & 236 & 93 & 126 & 102 & 207 & 265 & 66 & 17 & 0 & 96 & 204 & 575 \\
 & 17 & 0 & 58 & 0 & 0 & 24 & 0 & 0 & 0 & 76 & 0 & 47 & 0 & 383 & 103 & 39 & 93 & 44 & 41 & 744 & 55 & 126 & 103 & 87 & 58 & 9 & 81 & 0 & 221 & 383 \\
 & 18 & 14 & 26 & 0 & 37 & 0 & 8 & 41 & 0 & 11 & 149 & 12 & 456 & 128 & 353 & 0 & 34 & 886 & 0 & 44 & 143 & 9 & 241 & 20 & 318 & 361 & 0 & 0 & 0 & 179 \\
 & 19 & 10 & 57 & 0 & 46 & 25 & 12 & 9 & 34 & 0 & 84 & 68 & 0 & 258 & 254 & 37 & 236 & 0 & 762 & 41 & 52 & 0 & 315 & 0 & 32 & 27 & 0 & 25 & 37 & 289 \\
 & 20 & 16 & 58 & 34 & 9 & 16 & 0 & 11 & 32 & 17 & 193 & 71 & 92 & 249 & 532 & 12 & 126 & 143 & 52 & 55 & 1122 & 0 & 135 & 205 & 93 & 416 & 12 & 0 & 36 & 147 \\
 & 21 & 0 & 270 & 44 & 0 & 8 & 0 & 0 & 0 & 9 & 0 & 33 & 0 & 412 & 241 & 104 & 102 & 9 & 0 & 126 & 0 & 735 & 104 & 42 & 42 & 0 & 11 & 8 & 67 & 278 \\
 & 22 & 95 & 408 & 84 & 152 & 216 & 69 & 185 & 290 & 174 & 222 & 223 & 400 & 478 & 632 & 149 & 207 & 241 & 315 & 103 & 135 & 104 & 2495 & 171 & 327 & 462 & 129 & 149 & 72 & 107 \\
 & 23 & 0 & 125 & 0 & 0 & 11 & 0 & 12 & 0 & 0 & 225 & 282 & 11 & 198 & 369 & 11 & 265 & 20 & 0 & 87 & 205 & 42 & 171 & 877 & 70 & 273 & 12 & 0 & 43 & 162 \\
 & 24 & 369 & 236 & 58 & 340 & 176 & 201 & 29 & 0 & 361 & 54 & 39 & 221 & 590 & 597 & 77 & 66 & 318 & 32 & 58 & 93 & 42 & 327 & 70 & 1809 & 148 & 0 & 188 & 41 & 207 \\
 & 25 & 14 & 14 & 227 & 61 & 19 & 28 & 89 & 47 & 9 & 506 & 133 & 506 & 9 & 783 & 33 & 17 & 361 & 27 & 9 & 416 & 0 & 462 & 273 & 148 & 1519 & 25 & 16 & 9 & 63 \\
 & 26 & 0 & 8 & 0 & 9 & 0 & 9 & 0 & 8 & 55 & 9 & 12 & 16 & 84 & 24 & 52 & 0 & 0 & 0 & 81 & 12 & 11 & 129 & 12 & 0 & 25 & 424 & 0 & 69 & 185 \\
 & 27 & 65 & 162 & 8 & 315 & 19 & 0 & 8 & 0 & 41 & 80 & 0 & 0 & \textbf{266} & 255 & 40 & 96 & 0 & 25 & 0 & 0 & 8 & 149 & 0 & 188 & 16 & 0 & \textbf{659} & 0 & 151 \\
 & 28 & 37 & 28 & 0 & 0 & 16 & 0 & 104 & 0 & 122 & 0 & 9 & 0 & 369 & 92 & 147 & 204 & 0 & 37 & 221 & 36 & 67 & 72 & 43 & 41 & 9 & 69 & 0 & 888 & 543 \\
 & 30 & 157 & 259 & 107 & 109 & 187 & 73 & 111 & 12 & 196 & 57 & 204 & 84 & 1198 & 581 & 405 & 575 & 179 & 289 & 383 & 147 & 278 & 107 & 162 & 207 & 63 & 185 & 151 & 543 & 2802 \\

 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Cooccurrence
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline \hline
\rowcolor[HTML]{D9D9D9}
\multicolumn{31}{c}{(b) \textbf{Cooccurrence}}\\
\hline \hline


 \multirow{29}{*}{\rotatebox{90}{Actual Class ID $\downarrow$}} & 1 & 1 & 0.12 & 0 & 0.25 & 0.05 & 0 & 0.02 & 0 & 0.36 & 0.02 & 0 & 0.01 & 0.03 & 0.02 & 0.09 & 0.03 & 0.02 & 0.01 & 0 & 0.01 & 0 & 0.04 & 0 & 0.20 & 0.01 & 0 & 0.10 & 0.04 & 0.06 \\
 & 2 & 0.23 & 1 & 0.01 & 0.38 & 0.25 & 0.09 & 0 & 0.33 & 0.06 & 0.04 & 0.11 & 0.01 & 0.16 & 0.07 & 0.15 & 0.08 & 0.03 & 0.07 & 0.08 & 0.05 & 0.37 & 0.16 & 0.14 & 0.13 & 0.01 & 0.02 & 0.25 & 0.03 & 0.09 \\
 & 3 & 0 & 0.01 & 1 & 0 & 0.06 & 0.41 & 0 & 0 & 0 & 0.03 & 0 & 0 & 0.06 & 0.09 & 0.03 & 0.01 & 0 & 0 & 0 & 0.03 & 0.06 & 0.03 & 0 & 0.03 & 0.15 & 0 & 0.01 & 0 & 0.04 \\
 & 4 & 0.30 & 0.23 & 0 & 1 & 0.05 & 0 & 0.02 & 0.06 & 0.10 & 0.19 & 0 & 0.03 & 0.06 & 0.04 & 0.07 & 0.04 & 0.04 & 0.06 & 0 & 0.01 & 0 & 0.06 & 0 & 0.19 & 0.04 & 0.02 & 0.48 & 0 & 0.04 \\
 & 5 & 0.05 & 0.14 & 0.07 & 0.05 & 1 & 0 & 0 & 0.04 & 0.02 & 0.01 & 0.05 & 0.02 & 0.09 & 0.08 & 0.27 & 0.03 & 0 & 0.03 & 0.03 & 0.01 & 0.01 & 0.09 & 0.01 & 0.10 & 0.01 & 0 & 0.03 & 0.02 & 0.07 \\
 & 6 & 0 & 0.03 & 0.32 & 0 & 0 & 1 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0.05 & 0.05 & 0.01 & 0 & 0.01 & 0.02 & 0 & 0 & 0 & 0.03 & 0 & 0.11 & 0.02 & 0.02 & 0 & 0 & 0.03 \\
 & 7 & 0.02 & 0 & 0 & 0.01 & 0 & 0 & 1 & 0 & 0.09 & 0 & 0.01 & 0.19 & 0.01 & 0.01 & 0.02 & 0.03 & 0.05 & 0.01 & 0 & 0.01 & 0 & 0.07 & 0.01 & 0.02 & 0.06 & 0 & 0.01 & 0.12 & 0.04 \\
 & 8 & 0 & 0.10 & 0 & 0.03 & 0.02 & 0 & 0 & 1 & 0.05 & 0 & 0.12 & 0.01 & 0.02 & 0.01 & 0.01 & 0.01 & 0 & 0.04 & 0 & 0.03 & 0 & 0.12 & 0 & 0 & 0.03 & 0.02 & 0 & 0 & 0 \\
 & 9 & 0.41 & 0.04 & 0 & 0.10 & 0.02 & 0.02 & 0.15 & 0.10 & 1 & 0 & 0 & 0.07 & 0.06 & 0.04 & 0.03 & 0.03 & 0.01 & 0 & 0.10 & 0.02 & 0.01 & 0.07 & 0 & 0.20 & 0.01 & 0.13 & 0.06 & 0.14 & 0.07 \\
 & 10 & 0.02 & 0.02 & 0.04 & 0.19 & 0.01 & 0 & 0 & 0 & 0 & 1 & 0.13 & 0.15 & 0 & 0.15 & 0.03 & 0.02 & 0.17 & 0.11 & 0 & 0.17 & 0 & 0.09 & 0.26 & 0.03 & 0.33 & 0.02 & 0.12 & 0 & 0.02 \\
 & 11 & 0 & 0.07 & 0 & 0 & 0.06 & 0 & 0.02 & 0.25 & 0 & 0.13 & 1 & 0 & 0.06 & 0.12 & 0.08 & 0.15 & 0.01 & 0.09 & 0.06 & 0.06 & 0.04 & 0.09 & 0.32 & 0.02 & 0.09 & 0.03 & 0 & 0.01 & 0.07 \\
 & 12 & 0.02 & 0.01 & 0 & 0.04 & 0.02 & 0 & 0.37 & 0.02 & 0.08 & 0.16 & 0 & 1 & 0.01 & 0.11 & 0 & 0.01 & 0.51 & 0 & 0 & 0.08 & 0 & 0.16 & 0.01 & 0.12 & 0.33 & 0.04 & 0 & 0 & 0.03 \\
 & 13 & 0.12 & 0.35 & 0.32 & 0.24 & 0.38 & 0.34 & 0.08 & 0.12 & 0.23 & 0.02 & 0.23 & 0.02 & 1 & 0.30 & 0.22 & 0.38 & 0.14 & 0.34 & 0.51 & 0.22 & 0.56 & 0.19 & 0.23 & 0.33 & 0.01 & 0.20 & \textbf{0.40} & 0.42 & 0.43 \\
 & 14 & 0.07 & 0.16 & 0.49 & 0.16 & 0.34 & 0.38 & 0.05 & 0.10 & 0.16 & 0.59 & 0.44 & 0.40 & 0.31 & 1 & 0.27 & 0.41 & 0.40 & 0.33 & 0.14 & 0.47 & 0.33 & 0.25 & 0.42 & 0.33 & 0.52 & 0.06 & 0.39 & 0.10 & 0.21 \\
 & 15 & 0.13 & 0.11 & 0.06 & 0.09 & 0.37 & 0.02 & 0.05 & 0.02 & 0.04 & 0.04 & 0.09 & 0 & 0.08 & 0.09 & 1 & 0.07 & 0 & 0.05 & 0.05 & 0.01 & 0.14 & 0.06 & 0.01 & 0.04 & 0.02 & 0.12 & 0.06 & 0.17 & 0.14 \\
 & 16 & 0.06 & 0.08 & 0.01 & 0.06 & 0.06 & 0 & 0.08 & 0.04 & 0.05 & 0.03 & 0.24 & 0.01 & 0.17 & 0.17 & 0.09 & 1 & 0.04 & 0.31 & 0.13 & 0.11 & 0.14 & 0.08 & 0.30 & 0.04 & 0.01 & 0 & 0.15 & 0.23 & 0.21 \\
 & 17 & 0 & 0.04 & 0 & 0 & 0.03 & 0 & 0 & 0 & 0.09 & 0 & 0.05 & 0 & 0.12 & 0.03 & 0.04 & 0.06 & 0.05 & 0.05 & 1 & 0.05 & 0.17 & 0.04 & 0.10 & 0.03 & 0.01 & 0.19 & 0 & 0.25 & 0.14 \\
 & 18 & 0.02 & 0.02 & 0 & 0.04 & 0 & 0.02 & 0.08 & 0 & 0.01 & 0.17 & 0.01 & 0.48 & 0.04 & 0.10 & 0 & 0.02 & 1 & 0 & 0.06 & 0.13 & 0.01 & 0.10 & 0.02 & 0.18 & 0.24 & 0 & 0 & 0 & 0.06 \\
 & 19 & 0.01 & 0.04 & 0 & 0.05 & 0.03 & 0.02 & 0.02 & 0.08 & 0 & 0.09 & 0.08 & 0 & 0.08 & 0.07 & 0.03 & 0.16 & 0 & 1 & 0.06 & 0.05 & 0 & 0.13 & 0 & 0.02 & 0.02 & 0 & 0.04 & 0.04 & 0.10 \\
 & 20 & 0.02 & 0.04 & 0.06 & 0.01 & 0.02 & 0 & 0.02 & 0.07 & 0.02 & 0.22 & 0.08 & 0.10 & 0.08 & 0.16 & 0.01 & 0.09 & 0.16 & 0.07 & 0.07 & 1 & 0 & 0.05 & 0.23 & 0.05 & 0.27 & 0.03 & 0 & 0.04 & 0.05 \\
 & 21 & 0 & 0.19 & 0.07 & 0 & 0.01 & 0 & 0 & 0 & 0.01 & 0 & 0.04 & 0 & 0.12 & 0.07 & 0.09 & 0.07 & 0.01 & 0 & 0.17 & 0 & 1 & 0.04 & 0.05 & 0.02 & 0 & 0.03 & 0.01 & 0.08 & 0.10 \\
 & 22 & 0.13 & 0.28 & 0.14 & 0.17 & 0.27 & 0.14 & 0.37 & 0.66 & 0.21 & 0.25 & 0.25 & 0.42 & 0.14 & 0.18 & 0.13 & 0.14 & 0.27 & 0.41 & 0.14 & 0.12 & 0.14 & 1 & 0.19 & 0.18 & 0.30 & 0.30 & 0.23 & 0.08 & 0.04 \\
 & 23 & 0 & 0.09 & 0 & 0 & 0.01 & 0 & 0.02 & 0 & 0 & 0.25 & 0.31 & 0.01 & 0.06 & 0.11 & 0.01 & 0.18 & 0.02 & 0 & 0.12 & 0.18 & 0.06 & 0.07 & 1 & 0.04 & 0.18 & 0.03 & 0 & 0.05 & 0.06 \\
 & 24 & 0.49 & 0.16 & 0.09 & 0.39 & 0.22 & 0.42 & 0.06 & 0 & 0.43 & 0.06 & 0.04 & 0.23 & 0.18 & 0.17 & 0.07 & 0.05 & 0.36 & 0.04 & 0.08 & 0.08 & 0.06 & 0.13 & 0.08 & 1 & 0.10 & 0 & 0.29 & 0.05 & 0.07 \\
 & 25 & 0.02 & 0.01 & 0.37 & 0.07 & 0.02 & 0.06 & 0.18 & 0.11 & 0.01 & 0.57 & 0.15 & 0.53 & 0 & 0.23 & 0.03 & 0.01 & 0.41 & 0.04 & 0.01 & 0.37 & 0 & 0.19 & 0.31 & 0.08 & 1 & 0.06 & 0.02 & 0.01 & 0.02 \\
 & 26 & 0 & 0.01 & 0 & 0.01 & 0 & 0.02 & 0 & 0.02 & 0.07 & 0.01 & 0.01 & 0.02 & 0.03 & 0.01 & 0.05 & 0 & 0 & 0 & 0.11 & 0.01 & 0.01 & 0.05 & 0.01 & 0 & 0.02 & 1 & 0 & 0.08 & 0.07 \\
 & 27 & 0.09 & 0.11 & 0.01 & 0.36 & 0.02 & 0 & 0.02 & 0 & 0.05 & 0.09 & 0 & 0 & 0.08 & 0.07 & 0.04 & 0.07 & 0 & 0.03 & 0 & 0 & 0.01 & 0.06 & 0 & 0.10 & 0.01 & 0 & 1 & 0 & 0.05 \\
 & 28 & 0.05 & 0.02 & 0 & 0 & 0.02 & 0 & 0.21 & 0 & 0.14 & 0 & 0.01 & 0 & 0.11 & 0.03 & 0.13 & 0.14 & 0 & 0.05 & 0.30 & 0.03 & 0.09 & 0.03 & 0.05 & 0.02 & 0.01 & 0.16 & 0 & 1 & 0.19 \\
 & 30 & 0.21 & 0.18 & 0.17 & 0.12 & 0.23 & 0.15 & 0.22 & 0.03 & 0.23 & 0.06 & 0.23 & 0.09 & 0.36 & 0.17 & 0.36 & 0.40 & 0.20 & 0.38 & 0.51 & 0.13 & 0.38 & 0.04 & 0.18 & 0.11 & 0.04 & 0.44 & 0.23 & 0.61 & 1 \\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Misprediction
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hline \hline
\rowcolor[HTML]{D9D9D9}
\multicolumn{31}{c}{(c) \textbf{Misprediction}}\\
\hline \hline

 \multirow{30}{*}{\rotatebox{90}{Predicted Class ID $\downarrow$}}
 & 1 & 0 & 0.03 & 0.01 & 0.03 & 0.01 & 0.02 & 0 & 0 & 0.05 & 0 & 0 & 0 & 0.01 & 0.01 & 0.01 & 0.02 & 0 & 0 & 0.01 & 0.01 & 0.01 & 0.01 & 0 & 0.04 & 0 & 0 & 0.06 & 0 & 0 \\
 & 2 & 0.03 & 0 & 0.03 & 0.06 & 0.03 & 0 & 0.02 & 0.03 & 0 & 0.02 & 0.01 & 0 & 0.04 & 0.01 & 0.01 & 0.03 & 0 & 0.01 & 0.02 & 0.01 & 0.09 & 0.02 & 0 & 0.04 & 0 & 0 & 0.10 & 0.02 & 0.05 \\
 & 3 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0.03 & 0 & 0.01 & 0 & 0 & 0 & 0.02 & 0 & 0.02 & 0 & 0 & 0.02 & 0 & 0 & 0 & 0 \\
 & 4 & 0.03 & 0.03 & 0 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0.04 & 0 & 0 & 0.01 & 0.01 & 0.02 & 0.01 & 0.01 & 0 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.04 & 0.01 & 0 & 0.17 & 0.01 & 0.01 \\
 & 5 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0.04 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0.04 & 0 & 0 \\
 & 6 & 0 & 0.01 & 0.06 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0.01 & 0 & 0 & 0 & 0.01 \\
 & 7 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0.01 & 0.01 & 0 & 0 & 0.01 & 0.01 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0.01 \\
 & 8 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0 \\
 & 9 & 0.07 & 0.02 & 0 & 0.04 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0.01 & 0.02 & 0.02 & 0.02 & 0 & 0 & 0 & 0.01 & 0.02 & 0 & 0 & 0.02 & 0.01 & 0 & 0.05 & 0.03 & 0.02 \\
 & 10 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.02 & 0 & 0.03 & 0.01 & 0.01 & 0.01 & 0 & 0 & 0.04 & 0.01 & 0 & 0.01 & 0 & 0.06 & 0 & 0.03 & 0.01 & 0.01 \\
 & 11 & 0.02 & 0.01 & 0 & 0 & 0.01 & 0 & 0.02 & 0 & 0 & 0 & 0 & 0.01 & 0.01 & 0.01 & 0.01 & 0.03 & 0.04 & 0 & 0 & 0.01 & 0.01 & 0 & 0 & 0 & 0.02 & 0 & 0.01 & 0.02 & 0.03 \\
 & 12 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0.09 & 0 & 0 & 0.02 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0.02 & 0 & 0.02 & 0 & 0.02 & 0.01 & 0 & 0 & 0 & 0 \\
 & 13 & 0.03 & 0.06 & 0.16 & 0.09 & 0.10 & 0.03 & 0.02 & 0 & 0.03 & 0 & 0.09 & 0 & 0 & 0.06 & 0.09 & 0.16 & 0.04 & 0.03 & 0.23 & 0.04 & 0.11 & 0.02 & 0.01 & 0.04 & 0.01 & 0.03 & \textbf{0.43} & 0.24 & 0.16 \\
 & 14 & 0 & 0.06 & 0.08 & 0 & 0.05 & 0 & 0 & 0.07 & 0.01 & 0.10 & 0.05 & 0.04 & 0 & 0 & 0.07 & 0.09 & 0.07 & 0.03 & 0.07 & 0.15 & 0.11 & 0.02 & 0.02 & 0.07 & 0.09 & 0.02 & 0.25 & 0.07 & 0.05 \\
 & 15 & 0.03 & 0.01 & 0 & 0.02 & 0.05 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0.01 & 0 & 0 & 0.02 & 0 & 0.01 & 0.02 & 0 & 0.04 & 0 & 0 & 0.01 & 0 & 0 & 0.05 & 0.05 & 0.02 \\
 & 16 & 0.02 & 0.01 & 0.01 & 0.01 & 0.03 & 0 & 0.02 & 0.02 & 0 & 0.02 & 0.03 & 0.01 & 0.04 & 0.04 & 0 & 0 & 0.02 & 0.09 & 0.04 & 0.04 & 0.01 & 0.01 & 0 & 0.01 & 0.01 & 0.02 & 0.10 & 0.14 & 0.11 \\
 & 17 & 0.01 & 0 & 0.03 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0.03 & 0 & 0.02 & 0.02 & 0 & 0 & 0.03 & 0.01 & 0 & 0 & 0 & 0.01 & 0 & 0.01 & 0 & 0.02 & 0.03 & 0.07 & 0.04 \\
 & 18 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0.04 & 0 & 0 & 0.02 & 0 & 0 & 0 & 0.01 & 0.02 & 0 & 0 & 0 & 0 & 0.02 & 0 & 0 & 0 & 0.01 & 0.01 & 0 & 0 & 0 & 0 \\
 & 19 & 0 & 0.01 & 0 & 0.01 & 0 & 0 & 0 & 0.06 & 0 & 0.01 & 0.01 & 0 & 0 & 0.01 & 0 & 0.01 & 0 & 0 & 0 & 0.02 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0.01 & 0.01 & 0.01 \\
 & 20 & 0.01 & 0.04 & 0 & 0.02 & 0.02 & 0 & 0 & 0 & 0 & 0.01 & 0.01 & 0.01 & 0.03 & 0.01 & 0 & 0.03 & 0.05 & 0.01 & 0 & 0 & 0.01 & 0.01 & 0 & 0.01 & 0.03 & 0 & 0.04 & 0.02 & 0.03 \\
 & 21 & 0 & 0.01 & 0.07 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0.03 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0.04 & 0.02 \\
 & 22 & 0.03 & 0.01 & 0.02 & 0.04 & 0.03 & 0.04 & 0.06 & 0.24 & 0.04 & 0.07 & 0 & 0.05 & 0.03 & 0.04 & 0.06 & 0.02 & 0.01 & 0 & 0 & 0.04 & 0 & 0 & 0 & 0.03 & 0.02 & 0.03 & 0.08 & 0.02 & 0.01 \\
 & 23 & 0.02 & 0 & 0 & 0 & 0.02 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0.01 & 0.01 & 0.02 & 0.01 & 0 & 0.01 & 0.04 & 0 & 0 & 0 & 0.01 & 0.01 & 0.02 & 0 & 0.02 & 0.03 \\
 & 24 & 0.07 & 0.04 & 0.01 & 0.08 & 0.03 & 0.03 & 0.04 & 0 & 0.06 & 0.03 & 0.01 & 0.03 & 0.02 & 0.03 & 0.03 & 0.03 & 0.08 & 0 & 0.01 & 0.02 & 0.01 & 0.01 & 0 & 0 & 0.03 & 0 & 0.08 & 0 & 0 \\
 & 25 & 0.01 & 0.01 & 0.02 & 0 & 0.02 & 0 & 0.04 & 0.04 & 0.01 & 0.05 & 0.01 & 0.06 & 0.01 & 0.05 & 0.02 & 0.02 & 0.07 & 0 & 0.01 & 0.09 & 0.02 & 0.02 & 0.02 & 0 & 0 & 0 & 0.01 & 0 & 0.01 \\
 & 26 & 0.01 & 0.01 & 0 & 0.01 & 0.01 & 0.02 & 0 & 0 & 0.01 & 0 & 0.01 & 0.01 & 0.01 & 0.01 & 0.03 & 0 & 0 & 0.02 & 0 & 0.02 & 0.01 & 0.01 & 0 & 0 & 0 & 0 & 0.01 & 0.02 & 0.01 \\
 & 27 & 0 & 0.01 & 0 & 0.02 & 0 & 0 & 0 & 0 & 0 & 0.03 & 0 & 0 & 0.01 & 0.01 & 0.02 & 0 & 0 & 0.01 & 0.01 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0 & 0 & 0.01 & 0.02 \\
 & 28 & 0 & 0 & 0.01 & 0 & 0.01 & 0.04 & 0 & 0 & 0.01 & 0 & 0.01 & 0 & 0.01 & 0.02 & 0.02 & 0.01 & 0 & 0 & 0.05 & 0.02 & 0.03 & 0.01 & 0 & 0.02 & 0.01 & 0 & 0 & 0 & 0.01 \\
 & 29 & 0 & 0.01 & 0 & 0.02 & 0.01 & 0 & 0.02 & 0 & 0 & 0 & 0 & 0 & 0.01 & 0.01 & 0.01 & 0.01 & 0 & 0 & 0.01 & 0.02 & 0 & 0.01 & 0 & 0.01 & 0 & 0 & 0 & 0 & 0.02 \\
 & 30 & 0.06 & 0.05 & 0.10 & 0.06 & 0.01 & 0 & 0 & 0 & 0.01 & 0.04 & 0.12 & 0.03 & 0.10 & 0.07 & 0.09 & 0.14 & 0.12 & 0.07 & 0.17 & 0.08 & 0.13 & 0.03 & 0.03 & 0.05 & 0.04 & 0.07 & 0.23 & 0.23 & 0 \\
 \hline
\end{tabular}
\end{adjustbox}
\label{tab:misclassification_non_fiction}
\end{table*}

==> tables/misprediction_sample.tex <==


\begin{table}[!hbt]
\centering
\caption{Misprediction due to insufficient information on samples}
\begin{adjustbox}{width=0.5\textwidth}
% \begin{adjustbox}{angle=90, height=1\textheight}
% \footnotesize
\begin{tabular}{c|ll}%p{0.9\textwidth}}
% \multicolumn{3}{c}{(a) Samples for heatmap analysis}\\
\hline \hline
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \\[\dimexpr -\normalbaselineskip+1.5pt]

% \rowcolor[HTML]{D9D9D9}
% \multicolumn{3}{c}{\textbf{\emph{(a)} 9780062506139: The Archaic Revival : Speculations on Psychedelic Mushrooms, the Amazon, Virtual Reality, UFOs, Evolut}}\\
% \hline \hline
% & \\ [\dimexpr-\normalbaselineskip+1.5pt]

% \multirow{3}{*}{\includegraphics[width=0.04\linewidth, height=0.05\linewidth]{figs/misprediction_sample/5.jpg}} & ${\cal{T}} $ & Cited by theL.A. Weeklyas "the culture's foremost spokesman for the psychedelic experience," Terrence McKenna is an underground legend as a brilliant raconteur, adventurer \& \\
% & &  expert on the experiential use of mind-altering plants. In these essays, interviews \& narrative adventures, McKenna takes us on a mesmerizing journey deep into the Amazon as\\
% & &     well as into the hidden recesses of the human psyche \& the outer limits of our culture, giving us startling visions of the past \& future.\\ \cline{2-3}
% & ${\cal{M}}$ & \{"author":"Terence Mckenna","publisher":"HarperSanFrancisco"\}\\ \hline
% \multicolumn{2}{c|}{Actaul Genre} & Non-fiction: History, Humanities, Mythology \& Religion \& Spirituality, Science \& Math \& Mathematics\\ \hline
% \multicolumn{2}{c|}{Predicted Genre} & Non-fiction: Travel, Biographies \& Memoir\\

% \hline \hline

% \rowcolor[HTML]{D9D9D9}
% \multicolumn{3}{c}{\textbf{\emph{(b)} 9780345338495: Black Mountain Breakdown}}\\
% \hline \hline
% & \\ [\dimexpr-\normalbaselineskip+1.5pt]


% \multirow{3}{*}{\includegraphics[width=0.04\linewidth, height=0.05\linewidth]{figs/misprediction_sample/6.jpg}} & ${\cal{T}} $ & Crystal Spangler lives in rural Appalachia. She's the apple of her mother's eye -- not yet beautiful, but she will be. She's the most popular girl at Black Rock High. She makes\\
% & &  cheerleader, gets good grades, and is elected beauty queen. Crystal discovers God, goes to college, and falls in love. When she comes home, she's disheveled and confused. Crystal \\
% & & becomes a wealthy politician's wife. But there's something calling her, drawing her back to where it all began, in the shadow of Black Mountain . . .From the Paperback edition.\\ 
% & & to battle the forces of evil. \\ \cline{2-3}

% & ${\cal{M}}$ & \{"author":"Lee Smith","publisher":"Ballantine Books"\}\\ \hline
% \multicolumn{2}{c|}{Actaul Genre} & Fiction: History, Literature\\ \hline
% \multicolumn{2}{c|}{Predicted Genre} & Fiction: Mythology \& Religion \& Spirituality, Romance\\



\hline \hline
\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textbf{{\emph{(a)}} 9780760705902: The awakening; Author: Kate Chopin; Publisher: Barnes \& Noble Books}}\\
\hline \hline
& \\ [\dimexpr-\normalbaselineskip+1.5pt]

\multirow{6}{*}{\includegraphics[width=0.15\linewidth]{figs/less_info_misprediction/58649539.jpg}} & \multirow{2}{*}{\textbf{Blurb}:} & \multirow{2}{*}{The Awakening}\\ %\cline{2-3}
& & \\ \cline{2-3}
% & ${\cal{M}}$ & \{"author":"Kate Chopin","publisher":"Barnes \& Noble Books"\}\\ \hline
& \multirow{2}{*}{\textbf{Actual Genre}:} & \multirow{2}{*}{(Fiction, \{History, Humanities, Literature, Teen \& Young Adult\})}\\ %\cline{2-3}
& & \\ \cline{2-3}
& \multirow{2}{*}{\textbf{Predicted Genre}:} & \multirow{2}{*}{(Fiction, \{Arts \& Photography, Environment \& Plant, Literature\})}\\
& & \\ 



\hline \hline
\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textbf{{\emph{(b)}} 9780826400475: Pedagogy of the oppressed; Author: Paulo Freire; Publisher: Continuum}}\\
\hline \hline
& \\ [\dimexpr-\normalbaselineskip+1.5pt]

\multirow{6}{*}{\includegraphics[width=0.15\linewidth]{figs/misprediction_sample/7.jpg}} & \multirow{2}{*}{\textbf{Blurb}:} & \multirow{2}{*}{TSIGNED COPY BY THE AUTHOR} \\ 
& & \\
\cline{2-3}

%& ${\cal{M}}$ & \{"author":"Paulo Freire","publisher":"Continuum"\}\\ \hline
& \multirow{2}{*}{\textbf{Actual Genre}:} & \multirow{2}{*}{(Non-fiction, \{Humanities\})}\\ 
& & \\
\cline{2-3}
& \multirow{2}{*}{\textbf{Predicted Genre}:} & \multirow{2}{*}{(Non-fiction, \{Science \& Math \& Mathematics\})} \\
& & \\


\hline \hline
\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textbf{{\emph{(c)}} 9788420478722: LA Caverna De Las Ideas; Author: Jose Carlos Somoza; Publisher: Alfaguara}}\\
\hline \hline

\multirow{6}{*}{\includegraphics[width=0.15\linewidth]{figs/less_info_misprediction/848607.jpg}} & \multirow{2}{*}{\textbf{Blurb}:} & \multirow{2}{*}{Book by Jose Carlos Somoza} \\
& &  \\ \cline{2-3}

% & ${\cal{M}}$ & \{"author":"Jose Carlos Somoza","publisher":"Aguilar"\}\\
% \hline

& \multirow{2}{*}{\textbf{Actual Genre}:} & \multirow{2}{*}{(Fiction, \{History, Humanities, Literature, Mystery \& Thriller \& Suspense \& Horror\})}\\
& &  \\ \cline{2-3}
& \multirow{2}{*}{\textbf{Predicted Genre}:} & \multirow{2}{*}{(Fiction, \{Arts \& Photography, Literature, Reference \& Language, Sci-Fi\})} \\
& &  \\


\hline \hline
\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textbf{{\emph{(d)}} 9781571740601: Gooberz; Author: Linda Goodman; Publisher: Hampton Roads Publishing Company}}\\
\hline \hline


\multirow{6}{*}{\includegraphics[width=0.15\linewidth]{figs/less_info_misprediction/213153.jpg}} & \multirow{2}{*}{\textbf{Blurb}:} & \multirow{2}{*}{Paperback} \\
& & \\
\cline{2-3}
% & ${\cal{M}}$ & \{"author":"Linda Goodman","publisher":"Hampton Roads Publishing Company"\}\\
% \hline
& \multirow{2}{*}{\textbf{Actual Genre}:} & \multirow{2}{*}{(Fiction, \{Literature, Mythology \& Religion \& Spirituality\})}\\
& & \\
\cline{2-3}
& \multirow{2}{*}{\textbf{Predicted Genre}:} & \multirow{2}{*}{(Fiction, \{Arts \& Photography, Literature, Sci-Fi\})}\\
& & \\


\hline

% \multicolumn{3}{r}{${\cal{I}}$: Coverpage Image, ${\cal{T}}$: Description Text, ${\cal{M}}$: Metadata}
\end{tabular}
\end{adjustbox}


\label{tab:misprediction_sample}

\end{table}

==> tables/model_limitation.tex <==


\begin{table*}[!hbt]
\centering
\caption{Misprediction due to Level-1 classification}
\begin{adjustbox}{width=0.95\textwidth}
% \begin{adjustbox}{angle=90, height=1\textheight}
% \footnotesize
\begin{tabular}{c|ll}%p{0.9\textwidth}}
% \multicolumn{3}{c}{(a) Samples for heatmap analysis}\\


\hline \hline
\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textbf{{\emph{(a)}} 9780312266820: Dead Egotistical Morons: A Paul Turner Mystery; Author: Mark Richard Zubro; Publisher: St. Martin's Press}}\\
\hline \hline

\multirow{11}{*}{\includegraphics[width=0.1\linewidth]{figs/misprediction_sample/4.jpg}} & \multirow{8}{*}{\textbf{Blurb}:} & Boys4U is the world's most popular singing group - at least among teenaged girls - and they have closed out their sold-out world tour with a series of shows \\
& &   in Chicago's brand new arena. The premier group of the inexplicably popular "boy band" trend, they've just finished their very last concert of the tour. While  \\
& & hundreds of tour members, well-wishers, executives, and various hangers on wait to celebrate another wildly successful tour, the lead singer is found murdered  \\
& &   - shot in the back of the head at close range - in the shower all times, the only other people back there were the other members of the band, and  none of the \\
& &   dozens of people in the next room report having heard a shot. While the international press is engaged of the backstage dressing area. To make matters more    \\
& & distressing, the crime itself was almost impossible - there was tight security on the shower area at in an unprecedented feeding frenzy over the sensationalistic \\
& & murder, Chicago Police Detectives Paul Turner and his partner Buck Fenwick have pulled the unenviable task of investigating the murder But even the initial \\
& &  appearances are deceiving and as they dig deeper into the case, they uncover more disturbing truths beneath the wholesome façade of Boys4U. Now they have \\
& &  untangle an increasingly complex web if they are to stop a determined killer before more victims are claimed. \\
\cline{2-3}

% & ${\cal{M}}$ & \{"author":"Mark Richard Zubro","publisher":"St. Martin's Press"\}\\ \hline

& \multicolumn{1}{l}{\textbf{Actaul Genre}:} & (Fiction, \{Fashion \& Lifestyle, Mystery \& Thriller \& Suspense \& Horror\})\\ \cline{2-3} %\hline
& \multicolumn{1}{l}{\textbf{Predicted Genre}:} & (Non-fiction, \{Arts \& Photography\}) \\



\hline \hline
\rowcolor[HTML]{D9D9D9}
\multicolumn{3}{c}{\textbf{{\emph{(b)}} 9780312979256: Mafia Marriage; Author: Rosalie Bonanno; Publisher: St. Martin's Paperbacks}}\\
\hline \hline

\multirow{9}{*}{\includegraphics[width=0.08\linewidth]{figs/misprediction_sample/16.jpg}} & \multirow{6}{*}{\textbf{Blurb}:} & An Unforgettable Look Inside the Godfather's Own HouseShe Was A Profaci. He Was A BonannoRosalie Profaci was a Mafia princess. Salvatore "Bill" \\
& &   Bonanno, oldest son of   Mafia Don Joe Bonanno, the real-life model for The Godfather, was organized crime's crown prince. And Bill, deeply involved in his \\
& &   father's "business" of mob schemes thought  pretty Rosalie knew what it meant to be a "Mafia wife." But the convent-raised, deeply devout Rosalie, whose \\
& &   innocence was protected by her doting father, had no idea...Their  Marriage United Two Mafia Dynasties...Mafia Marriage is Rosalie Bonanno's intimate \\
& &  account of life inside the secretive world of the Mafia. Naming names and providing shocking details, she writes about the wild spending sprees, the \\
& &   mysterious absences of her husband, the other women in his-their running from the law, the abductions, and shootings. Above all, Rosalie reveals the passion\\
& &  that kept her virtually a prisoner to love...and her heartbreaking journey of discovering the truth and trying to break free. \\

\cline{2-3}

% & ${\cal{M}}$ & \{"author":"Rosalie Bonanno","publisher":"St. Martin's Paperbacks"\}\\ \hline

& \multicolumn{1}{l}{\textbf{Actaul Genre}:} & (Non-fiction, \{Biographies \& Memoir, Mystery \& Thriller \& Suspense \& Horror\})\\ \cline{2-3} %\hline
& \multicolumn{1}{l}{\textbf{Predicted Genre}:} & (Fiction, \{History, Romance, Teen \& Young Adult\}) \\



\hline


% \multicolumn{3}{r}{${\cal{I}}$: Coverpage Image, ${\cal{T}}$: Description Text, ${\cal{M}}$: Metadata}
\end{tabular}
\end{adjustbox}


\label{tab:model_limitation}

\end{table*}

==> tables/module_ablation.tex <==





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Version-1
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!htb]
\centering
\caption{Module ablation study}
% \begin{adjustbox}{angle=90, height=\textheight}
\begin{adjustbox}{width=0.91\textwidth} 
% \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\begin{tabular}{c | cc | c cccc cccc | c cccc cccc}
\hline
% \multirow{3}{*}{\textbf{Model}}  & \multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Level-1}}} & \multicolumn{18}{c}{\textbf{Level-2}} \\ \cline{4-21} 

% & \multicolumn{2}{c|}{}& \multicolumn{9}{c|}{\textbf{Fiction}}& \multicolumn{9}{c}{\textbf{Non-fiction}} \\ \cline{2-21} 
\multirow{2}{*}{\textbf{Model}}  & \multicolumn{2}{c|}{\textbf{Level-1}} & \multicolumn{9}{c|}{\textbf{Level-2: Fiction}}& \multicolumn{9}{c}{\textbf{Level-2: Non-fiction}} \\ 
\cline{2-21}
& $\cal{F}\uparrow$ & 
 ${\cal{A}}\uparrow$ & 
 ${\cal{F}}_{\mu}\uparrow$ & 
 ${\cal{BA}}_{\mu}\uparrow$ & 
 ${\cal{F}}_{m}\uparrow$ & 
 ${\cal{BA}}_{m}\uparrow$ &
 ${\cal{F}}_{w}\uparrow$ &
 ${\cal{BA}}_{w}\uparrow$ & 
 ${\cal{F}}_{s}\uparrow$ & 
 ${\cal{BA}}_{s}\uparrow$
 & $\cal{HL}\downarrow$ & 
 ${\cal{F}}_{\mu}\uparrow$ & 
 ${\cal{BA}}_{\mu}\uparrow$ & 
 ${\cal{F}}_{m}\uparrow$ & 
 ${\cal{BA}}_{m}\uparrow$ &
 ${\cal{F}}_{w}\uparrow$ &
 ${\cal{BA}}_{w}\uparrow$ & 
 ${\cal{F}}_{s}\uparrow$ & 
 ${\cal{BA}}_{s}\uparrow$ & 
 ${\cal{HL}}\downarrow$ \\

\hline \hline 
$MM_{F}$ & -  & - & 64.28 & 80.47  & 62.38 & 78.53 & 62.64 & 77.91 & 62.12 & 80.34 & 0.0799 & 72.30 & 82.78 & 69.11 & 81.25 & 70.51 & 81.37 & 71.11 & 83.91 & 0.0629 \\ \hline 

% \rowcolor{lightgray}
% Improvement & - & - & 15.04 & 8.29 & 18.14 & 10.63 & 16.79 & 9.32 & 15.07 & 7.82 & 39.29\% & 11.44 & 8.28 & 15.16 & 9.67 & 13.2 & 8.85 & 9.32 & 6.62 & 43.08\% \\ 

 $\psi_M$  & \textbf{98.51} & \textbf{98.36} & {76.65} & {87.47} & {78.15} & {87.87} & {76.62} & {85.22} & {74.27} & {86.88} & {0.0553} & {78.46} & {87.00} & {79.39} & {86.74} & {78.40} & {85.83} & {73.23} & {85.90} & {0.0457}\\ \hline 


% \rowcolor{lightgray}
% Improvement & 0.00 & 0.00 & 2.67 & 1.29 & 2.37 & 1.29 & 2.81 & 2.01 & 2.92 & 1.28 & 12.29\% & 5.28 & 4.06 & 4.88 & 4.18 & 5.31 & 4.39 & 7.20 & 4.63 & 21.66\% \\ 


IMAGINE &\textbf{98.51} & \textbf{98.36} & \textbf{79.32} & \textbf{88.76} & \textbf{80.52} & \textbf{89.16} & \textbf{79.43} & \textbf{87.23} & \textbf{77.19} & \textbf{88.16} & \textbf{0.0485} & \textbf{83.74} & \textbf{91.06} & \textbf{84.27} & \textbf{90.92} & \textbf{83.71} & \textbf{90.22} & \textbf{80.43} & \textbf{90.53} & \textbf{0.0358}\\ \hline
% \multicolumn{22}{r}{$UM_v$: , $UM_d$: , $MM_{vd}$: , $MM_{vdc}$: , $MM_{vdm}$: , $MM_{vdcm}$: }


% \hline
% \multicolumn{21}{r}{$^\ast$Improvement of IMaGINe over the \textbf{second-best} results}
\end{tabular}
\end{adjustbox}
\label{tab:module_ablation}
\end{table*}

==> tables/settings_table.tex <==
\begin{table}[!hbt]
\centering

\caption{Experimental settings details}
\begin{adjustbox}{width=0.4\textwidth} 
\begin{tabular}{c|l}
% \hline
% \multicolumn{2}{c}{System settings} \\ \hline

% Operating system & Ubuntu 20.04.4 LTS \\
% Processor & Intel(R) Xeon(R) W-1270 (3.40GHz, 16 cores) \\
% Ram & 128 GB \\
% GPU & NVIDIA RTX A5000 (24GB) \\
% Environment & Python 3.10.14, PyTorch 2.1.0 \\

\hline
\multicolumn{2}{c}{Knowledge graph embedding settings} \\
\hline

Tool & OpenKE Toolkit \\
No. of epochs & 500 \\
Batch size & 100 \\
Learning rate & $10^{-3}$ \\
Optimizer & Adam \\

\hline
\multicolumn{2}{c}{Level-1 and Level-2 classification settings} \\
\hline

No. of epochs (Level-1 classification) & 50 \\
No. of epochs (Level-2 classification) & 100 \\
Batch size & 16 \\
Learning rate & $10^{-5}$ \\
Weight decay & $10^{-2}$ \\
Exponential decay rates & $\beta_1$ = 0.9, $\beta_2$ = 0.999 \\
Zero-denominator avoidance parameter & $10^{-8}$ \\
Optimizer & AdamW \\
Patience & 5 \\

\hline
\multicolumn{2}{c}{Classifier selector settings} \\
\hline

No. of epochs & 100 \\
Batch size & 16 \\
Learning rate & $10^{-3}$ \\
Weight decay & $10^{-2}$ \\
Exponential decay rates & $\beta_1$ = 0.9, $\beta_2$ = 0.999 \\
Zero-denominator avoidance parameter & $10^{-8}$ \\
Optimizer & AdamW \\
Patience & 5 \\
\hline
\end{tabular}
\label{tab:settings}
\end{adjustbox}
\end{table}

==> tables/stat.tex <==
% \begin{table}[]
%  \centering
%  \caption{Statistical analysis}
%  %\vspace{1em} % Adjust the vertical space here
%  \begin{adjustbox}{width=0.47\textwidth}
%  \begin{tabular}{c|p{2.95cm}|c|c|c|c|c}
% \hline
%    \textbf{Input} & 
   
%    & \textbf{Minimum} & \textbf{Maximum} & \textbf{Mean} & \textbf{Median} & \textbf{Standard deviation}\\ \hline
%     \multirow{4}{*}{\rotatebox{0}{\textbf{Cover page images}}} & Image area before augmentation & \multirow{2}{*}{20460} & \multirow{2}{*}{16301712} & \multirow{2}{*}{176507.93} & \multirow{2}{*}{125000} & \multirow{2}{*}{104410.22}\\
%     \cline{2-7}
%    & Image area after augmentation & \multirow{2}{*}{20460} & \multirow{2}{*}{16301712} & \multirow{2}{*}{143180.11} & \multirow{2}{*}{125000} & \multirow{2}{*}{97393.49}\\ \cline{2-7}
%     \hline
  

%    \multirow{9}{*}{\rotatebox{0}{\textbf{Description}}} & No. of samples before augmentation & \multirow{2}{*}{0} & \multirow{2}{*}{1580} & \multirow{2}{*}{108.217} & \multirow{2}{*}{87} & \multirow{2}{*}{90.925}\\ \cline{2-7}
%    & No. of samples after augmentation (Without preprocessing) & \multirow{4}{*}{0} & \multirow{4}{*}{1580} & \multirow{4}{*}{97.368} & \multirow{4}{*}{85} & \multirow{4}{*}{33.023}\\ \cline{2-7}
%    & No. of samples after augmentation (With preprocessing) & \multirow{3}{*}{21} & \multirow{3}{*}{949} & \multirow{3}{*}{69.483} & \multirow{3}{*}{61} & \multirow{3}{*}{20.394}\\ \cline{2-7}
%    \hline
%    \multirow{2}{*}{\rotatebox{0}{\textbf{OCR text}}} & No. of samples before and after augmentation & \multirow{2}{*}{1} & \multirow{2}{*}{862} & \multirow{2}{*}{21.327} & \multirow{2}{*}{15} & \multirow{2}{*}{33.390}\\
   

%    \hline

%    \multirow{4}{*}{\rotatebox{0}{\textbf{Metadata}}} & No. of books written by an author & \multirow{2}{*}{1} & \multirow{2}{*}{632} & \multirow{2}{*}{9.89} & \multirow{2}{*}{5.5} & \multirow{2}{*}{19.82}\\ \cline{2-7}
%    & No. of books published by a publisher & \multirow{2}{*}{1} & \multirow{2}{*}{7536} & \multirow{2}{*}{60.75} & \multirow{2}{*}{50.5} & \multirow{2}{*}{125.74}\\ \cline{2-7}
%    \hline
%  \end{tabular}
% \end{adjustbox}
%  \end{table}



\begin{table}[]
 \centering
 \caption{Statistical analysis}
 %\vspace{1em} % Adjust the vertical space here
 \begin{adjustbox}{width=0.5\textwidth}
 \begin{tabular}{c|c|c|c|c|c|c}
\hline
   \textbf{Input} & 
   
& \textbf{Min} & \textbf{Max} & \textbf{Mean ($\mu$)} & \textbf{Median} & \textbf{SD ($\sigma$)}\\ \hline

& Image area before & \multirow{2}{*}{20460} & \multirow{2}{*}{16301712} & \multirow{2}{*}{176507.93} & \multirow{2}{*}{125000} & \multirow{2}{*}{104410.22}\\
    

\textbf{Cover page} & augmentation & & & & & \\
\cline{2-7}
\textbf{images} & Image area after & \multirow{2}{*}{20460} & \multirow{2}{*}{16301712} & \multirow{2}{*}{143180.11} & \multirow{2}{*}{125000} & \multirow{2}{*}{97393.49}\\ 
& augmentation & & & & & \\
\hline
  

& No. of samples before & \multirow{2}{*}{0} & \multirow{2}{*}{1580} & \multirow{2}{*}{108.22} & \multirow{2}{*}{87} & \multirow{2}{*}{90.93}\\ 
   
\textbf{Description} & augmentation & & & & & \\
\cline{2-7}

& No. of samples after & \multirow{2}{*}{0} & \multirow{2}{*}{1580} & \multirow{2}{*}{97.37} & \multirow{2}{*}{85} & \multirow{2}{*}{33.02}\\ 

& augmentation & & & & & \\
\hline

 & No. of samples  & \multirow{3}{*}{1} & \multirow{3}{*}{862} & \multirow{3}{*}{21.33} & \multirow{3}{*}{15} & \multirow{3}{*}{33.39}\\

\textbf{OCR text} & before and after & & & & & \\

& augmentation & & & & & \\
   
\hline

& No. of books  & \multirow{2}{*}{1} & \multirow{2}{*}{632} & \multirow{2}{*}{9.89} & \multirow{2}{*}{5.5} & \multirow{2}{*}{19.82}\\ 

\textbf{Metadata} & written by an author & & & & & \\

\cline{2-7}
& No. of books  & \multirow{2}{*}{1} & \multirow{2}{*}{7536} & \multirow{2}{*}{60.75} & \multirow{2}{*}{50.5} & \multirow{2}{*}{125.74}\\ 
   
& published by a publisher & & & & & \\

\hline

   \multicolumn{7}{r}{SD: Standard Deviation}
 \end{tabular}
\end{adjustbox}
 \end{table}





==> tables/symbol_table.tex <==
\begin{table}[]
    \centering
    \caption{Symbol table}
    \begin{tabular}{c|c}
    \hline
      Symbol   & Meaning \\ \hline
      $\cal{P}$ & Precision \\ \hline
      $\cal{R}$ & Recall \\ \hline
      ${\cal{A}}$ & Accuracy \\ \hline
       ${\cal{F}}$  & F-measure \\ \hline
       ${\cal{F}}_{\mu}$ & Micro F-measure \\ \hline
       ${\cal{BA}}_{\mu}$ & Micro balanced accuracy \\ \hline
       ${\cal{F}}_{m}$ & Macro F-measure \\ \hline
       ${\cal{BA}}_{m}$ & Macro balanced accuracy \\ \hline
       ${\cal{F}}_{w}$ & Weighted F-measure \\ \hline
       ${\cal{BA}}_{w}$ & Weighted balanced accuracy \\ \hline
       ${\cal{F}}_{s}$ & Samples F-measure \\ \hline
       ${\cal{BA}}_{s}$ & Samples balanced accuracy \\ \hline
       ${\cal{HL}}$ & Hamming loss \\ \hline
       ${\cal{S}}p$ & Specificity \\ \hline
    \end{tabular}
    \label{tab:symbol}
\end{table}
